Towards Diverse Behaviors: A Benchmark for Imitation Learning with Human Demonstrations

Imitation learning with human data has demonstrated remarkable success in teaching robots in a wide range of skills. However, the inherent diversity in human behavior leads to the emergence of multi-modal data distributions, thereby presenting a formidable challenge for existing imitation learning algorithms. Quantifying a model's capacity to capture and replicate this diversity effectively is still an open problem. In this work, we introduce simulation benchmark environments and the corresponding Datasets with Diverse human Demonstrations for Imitation Learning (D3IL), designed explicitly to evaluate a model's ability to learn multi-modal behavior. Our environments are designed to involve multiple sub-tasks that need to be solved, consider manipulation of multiple objects which increases the diversity of the behavior and can only be solved by policies that rely on closed loop sensory feedback. Other available datasets are missing at least one of these challenging properties. To address the challenge of diversity quantification, we introduce tractable metrics that provide valuable insights into a model's ability to acquire and reproduce diverse behaviors. These metrics offer a practical means to assess the robustness and versatility of imitation learning algorithms. Furthermore, we conduct a thorough evaluation of state-of-the-art methods on the proposed task suite. This evaluation serves as a benchmark for assessing their capability to learn diverse behaviors. Our findings shed light on the effectiveness of these methods in tackling the intricate problem of capturing and generalizing multi-modal human behaviors, offering a valuable reference for the design of future imitation learning algorithms.

==> results/figures/ddpm_steps_ablation.tex <==
\begin{figure*}[htbp]
        \centering
 %        \subfigure[Obstacle Avoidance]{
            \begin{minipage}[t!]{0.48\textwidth}
                \centering 
                \includegraphics[width=0.48\textwidth]{figures/obstacle_avoidance/oa_beso_ablation_success.pdf}
                \includegraphics[width=0.48\textwidth]{figures/obstacle_avoidance/oa_beso_ablation_entropy.pdf}

                \subcaption[]{Diffusion Policy Ablation}
            \end{minipage}

            % \hfill

            % \begin{minipage}[t!]{0.48\textwidth}
            %     \centering 
            %     \includegraphics[width=0.48\textwidth]{figures/obstacle_avoidance/oa_ddpm_ablation_success.pdf}
            %     \includegraphics[width=0.48\textwidth]{figures/obstacle_avoidance/oa_ddpm_ablation_entropy.pdf}

            %     \subcaption[]{Diffusion Policy Ablation}
            % \end{minipage}
            
        \caption[ ]
        {\small \textbf{Environments.} We created 5 tasks in this paper, including one toy task Obstacle Avoidance and 4 robot manipulation tasks. For each task, we collected a large amount of human demonstrations with diverse behaviors. }
        \label{fig:ddpm_steps_ablation}
\end{figure*}

==> results/figures/stacking_demo.tex <==
\begin{figure*}[htbp]
        \centering
        % \subfigure[Obstacle Avoidance]{
            \begin{minipage}[t!]{0.48\textwidth}
                \centering 
                \includegraphics[width=0.48\textwidth]{figures/stacking/1.png}
                \includegraphics[width=0.48\textwidth]{figures/stacking/2.png}

                \subcaption[]{Diffusion Policy Ablation}
            \end{minipage}
        % }

        \caption[ ]
        {\small \textbf{Multi-modal Behaviors}}
        \label{fig:environments}
\end{figure*}


==> results/tables/ba_sort.tex <==
\begin{table}[hbtp]
\centering
 \caption{Performance of IL methods in the Sorting task with varying number of blocks}\label{sorting_table}
 % \caption{Sorting tasks benchmark}\label{sorting_table}
\resizebox{\textwidth}{!}{  

\begin{tabular}{l|cc|cc|cc}
	\toprule 
            & \multicolumn{2}{c|}{Sorting-2 (T4) } & \multicolumn{2}{c|}{Sorting-4 (T4)} & \multicolumn{2}{c}{Sorting-6 (T4)} \\
            
        \midrule

         Methods & Success Rate & Entropy & Success Rate & Entropy & Success Rate & Entropy \\

	\midrule

        BC-MLP  & 
        $0.444 \scriptstyle{\pm 0.069}$ & $0.0 \scriptstyle{\pm 0.0}$ & 
        $0.058 \scriptstyle{\pm 0.048}$ & $0.0 \scriptstyle{\pm 0.0}$ & 
        $0.016 \scriptstyle{\pm 0.014}$ & $0.0 \scriptstyle{\pm 0.0}$ \\
        % -------------------------------------------------------------- %
        % BC-GMM  & 
        % 0 & 0 & 
        % 0 & 0 & 
        % 0 & 0 \\
        % -------------------------------------------------------------- %
        VAE-State & 
        $0.451 \scriptstyle{\pm 0.059}$ & $0.106 \scriptstyle{\pm 0.051}$ & 
        $0.079 \scriptstyle{\pm 0.042}$ & $0.090 \scriptstyle{\pm 0.032}$ & 
        $\mathbf{0.030 \scriptstyle{\pm 0.016}}$ & $\mathbf{0.086 \scriptstyle{\pm 0.017}}$\\
        % -------------------------------------------------------------- %
        BeT-MLP & 
        $0.317 \scriptstyle{\pm 0.070}$ & $0.309 \scriptstyle{\pm 0.059}$ & 
        $0.003 \scriptstyle{\pm 0.001}$ & $0.021 \scriptstyle{\pm 0.052}$ & 
        $0.0 \scriptstyle{\pm 0.0}$ & $0.0 \scriptstyle{\pm 0.0}$\\
        % -------------------------------------------------------------- %
        IBC & 
        $0.459 \scriptstyle{\pm 0.033}$ & $\mathbf{0.370 \scriptstyle{\pm 0.071}}$ & 
        $\mathbf{0.080 \scriptstyle{\pm 0.016}}$ & $\mathbf{0.097 \scriptstyle{\pm 0.026}}$ & 
        $0.007 \scriptstyle{\pm 0.005}$ & $0.024 \scriptstyle{\pm 0.028}$\\
        % -------------------------------------------------------------- %
        DDPM-MLP & 
        $\mathbf{0.460 \scriptstyle{\pm 0.039}}$ & $0.327 \scriptstyle{\pm 0.037}$ & 
        $0.032 \scriptstyle{\pm 0.009}$ & $0.071 \scriptstyle{\pm 0.025}$ & 
        $0.0 \scriptstyle{\pm 0.0}$ & $0.0 \scriptstyle{\pm 0.0}$\\
        % -------------------------------------------------------------- %
        % \midrule

        %  history=5 $\rightarrow$ $\pi(a_t|s_{t-h+1:t})$ & Success Rate & Entropy & Success Rate & Entropy & Success Rate & Entropy \\

	\midrule

        BC-GPT  & 
        $0.800 \scriptstyle{\pm 0.040}$ & $0.0 \scriptstyle{\pm 0.0}$ & 
        $0.075 \scriptstyle{\pm 0.063}$ & $0.0 \scriptstyle{\pm 0.0}$ & 
        $0.007 \scriptstyle{\pm 0.003}$ & $0.0 \scriptstyle{\pm 0.0}$ \\
        % -------------------------------------------------------------- %
        % LSTM-GMM & 
        % 0 & 0 & 
        % 0 & 0 & 
        % 0 & 0\\
        % -------------------------------------------------------------- %
        BeT & 
        $0.680 \scriptstyle{\pm 0.060}$ & $\mathbf{0.473 \scriptstyle{\pm 0.049}}$ & 
        $0.018 \scriptstyle{\pm 0.010}$ & $0.059 \scriptstyle{\pm 0.035}$ & 
        $0.0 \scriptstyle{\pm 0.0}$ & $0.0 \scriptstyle{\pm 0.0}$\\
        % -------------------------------------------------------------- %
        DDPM-GPT & 
        $\mathbf{0.854 \scriptstyle{\pm 0.013}}$ & $0.431 \scriptstyle{\pm 0.060}$ & 
        $\mathbf{0.337 \scriptstyle{\pm 0.084}}$ & $\mathbf{0.372 \scriptstyle{\pm 0.068}}$ & 
        $0.005 \scriptstyle{\pm 0.003}$ & $0.031 \scriptstyle{\pm 0.029}$\\
        % -------------------------------------------------------------- %
        BESO  & 
        $0.784 \scriptstyle{\pm 0.026}$ & $0.387 \scriptstyle{\pm 0.038}$ & 
        $0.188 \scriptstyle{\pm 0.042}$ & $0.232 \scriptstyle{\pm 0.040}$ & 
        $\mathbf{0.020 \scriptstyle{\pm 0.002}}$ & $\mathbf{0.055 \scriptstyle{\pm 0.031}}$ \\

        \midrule
        VAE-ACT &
        $0.858 \scriptstyle{\pm 0.073}$ & $0.012 \scriptstyle{\pm 0.018}$ & 
        $\mathbf{0.565 \scriptstyle{\pm 0.108}}$ & $0.114 \scriptstyle{\pm 0.020}$ & 
        $0.021 \scriptstyle{\pm 0.019}$ & $0.057 \scriptstyle{\pm 0.040}$
        \\
        \midrule
        DDPM-ACT &
        $\mathbf{0.882 \scriptstyle{\pm 0.023}}$ & $0.347 \scriptstyle{\pm 0.048}$ & 
        $0.300 \scriptstyle{\pm 0.060}$ & $0.300 \scriptstyle{\pm 0.051}$ & 
        $0.0 \scriptstyle{\pm 0.0}$ & $0.0 \scriptstyle{\pm 0.0}$ 
        \\
	\bottomrule
\end{tabular}

}

\vskip -0.15in
\end{table}





% \begin{table}[hbtp]
% \centering
%  \caption{Results on Aligning (T2) and Stacking-X (T4) for \st{proprioceptive} and \im{image-based} state representation.}\label{table:ba_sort}
% \resizebox{\textwidth}{!}{  

% \begin{tabular}{l|cc|cc|cc}
% 	\toprule 
%             & \multicolumn{2}{c|}{Aligning (T2)} & \multicolumn{2}{c|}{Sorting-2 (T4)} & \multicolumn{2}{c}{Sorting-3 (T4)} \\
            
%         % \midrule

%           & Success Rate & Entropy & Success Rate & Entropy & Success Rate & Entropy \\

% 	\midrule

%         BC-MLP  & 
%         $0.708 \scriptstyle{\pm 0.052}$ / $0.148 \scriptstyle{\pm 0.045}$ & $0.0 \scriptstyle{\pm 0.0}$ / $0.0 \scriptstyle{\pm 0.0}$ & 
%         $0.058 \scriptstyle{\pm 0.048}$ / $0.666 \scriptstyle{\pm 0.080}$ & $0.0 \scriptstyle{\pm 0.0}$ / $0.0 \scriptstyle{\pm 0.0}$ & 
%         $0.016 \scriptstyle{\pm 0.014}$ / $0.636 \scriptstyle{\pm 0.026}$ & $0.0 \scriptstyle{\pm 0.0}$ / $0.0 \scriptstyle{\pm 0.0}$ \\
%         % -------------------------------------------------------------- %
%         % BC-GMM  & 
%         % 0 & 0 & 
%         % 0 & 0 & 
%         % 0 & 0 \\
%         % -------------------------------------------------------------- %
%         CVAE-State & 
%         $0.579 \scriptstyle{\pm 0.138}$ / $0.121 \scriptstyle{\pm 0.035}$  & $0.030 \scriptstyle{\pm 0.053}$ / $0.013 \scriptstyle{\pm 0.019}$  & 
%         $0.079 \scriptstyle{\pm 0.042}$ / $0.653 \scriptstyle{\pm 0.061}$ & $0.090 \scriptstyle{\pm 0.032}$ / $0.165 \scriptstyle{\pm 0.010}$ & 
%         $0.030 \scriptstyle{\pm 0.016}$ / $0.570 \scriptstyle{\pm 0.023}$ & $0.086 \scriptstyle{\pm 0.017}$ / $0.236 \scriptstyle{\pm 0.013}$\\
%         % -------------------------------------------------------------- %
%         BeT-MLP & 
%         $0.507 \scriptstyle{\pm 0.081}$ / $0.203 \scriptstyle{\pm 0.035}$ & $0.485 \scriptstyle{\pm 0.092}$ / $0.053 \scriptstyle{\pm 0.028}$ & 
%         $0.003 \scriptstyle{\pm 0.001}$ / $0.671 \scriptstyle{\pm 0.014}$& $0.021 \scriptstyle{\pm 0.052}$ / $0.296 \scriptstyle{\pm 0.033}$& 
%         $0.0 \scriptstyle{\pm 0.0}$ / $0.616 \scriptstyle{\pm 0.035}$& $0.0 \scriptstyle{\pm 0.0}$ / $0.365 \scriptstyle{\pm 0.022}$\\
%         % -------------------------------------------------------------- %
%         IBC & 
%         $0.638 \scriptstyle{\pm 0.027}$  / $0.179 \scriptstyle{\pm 0.028}$ & $0.300 \scriptstyle{\pm 0.048}$ / $0.071 \scriptstyle{\pm 0.052}$ & 
%         $0.080 \scriptstyle{\pm 0.016}$ / $0.707 \scriptstyle{\pm 0.031}$& $0.097 \scriptstyle{\pm 0.026}$ / $0.236 \scriptstyle{\pm 0.027}$& 
%         $0.007 \scriptstyle{\pm 0.005}$ / $0.664 \scriptstyle{\pm 0.039}$& $0.024 \scriptstyle{\pm 0.028}$ / $0.328 \scriptstyle{\pm 0.026}$\\
%         % -------------------------------------------------------------- %
%         DDPM-MLP & 
%         $\mathbf{0.763 \scriptstyle{\pm 0.039}}$ / $0.233 \scriptstyle{\pm 0.029}$ & $\mathbf{0.712 \scriptstyle{\pm 0.064}}$ / $0.060 \scriptstyle{\pm 0.033}$& 
%         $0.032 \scriptstyle{\pm 0.009}$ / $0.763 \scriptstyle{\pm 0.028}$& $0.071 \scriptstyle{\pm 0.025}$ / $0.237 \scriptstyle{\pm 0.028}$& 
%         $0.0 \scriptstyle{\pm 0.0}$ / $0.748 \scriptstyle{\pm 0.026}$ & $0.0 \scriptstyle{\pm 0.0}$ / $0.359 \scriptstyle{\pm 0.025}$\\
%         % -------------------------------------------------------------- %
%         % \midrulet
%  %          & Success & Entropy & Success & Entropy & Success & Entropy \\
% 	% \midrule

%         BC-GPT  & 
%         $0.833 \scriptstyle{\pm 0.043}$ / $0.084 \scriptstyle{\pm 0.015}$ & $0.0 \scriptstyle{\pm 0.0}$ / $0.0 \scriptstyle{\pm 0.0}$& 
%         $0.075 \scriptstyle{\pm 0.063}$ / $0.654 \scriptstyle{\pm 0.048}$ & $0.0 \scriptstyle{\pm 0.0}$ / $0.0 \scriptstyle{\pm 0.0}$& 
%         $0.011 \scriptstyle{\pm 0.008}$ / $0.590 \scriptstyle{\pm 0.017}$ & $0.0 \scriptstyle{\pm 0.0}$ / $0.0 \scriptstyle{\pm 0.0}$\\
%         % -------------------------------------------------------------- %
%         % LSTM-GMM & 
%         % 0 & 0 & 
%         % 0 & 0 & 
%         % 0 & 0\\
%         % -------------------------------------------------------------- %
%         BeT & 
%         $0.645 \scriptstyle{\pm 0.069}$ / $0.154 \scriptstyle{\pm 0.067}$ & $0.536 \scriptstyle{\pm 0.105}$ / $0.023 \scriptstyle{\pm 0.012}$& 
%         $0.018 \scriptstyle{\pm 0.010}$ / $0.676 \scriptstyle{\pm 0.035}$ & $0.059 \scriptstyle{\pm 0.035}$ / $0.305 \scriptstyle{\pm 0.029}$& 
%         $0.0 \scriptstyle{\pm 0.0}$ / $0.617 \scriptstyle{\pm 0.033}$ & $0.0 \scriptstyle{\pm 0.0}$ / $0.380 \scriptstyle{\pm 0.019}$\\
%         % -------------------------------------------------------------- %
%         DDPM-GPT & 
%         $0.839 \scriptstyle{\pm 0.020}$ / $0.316 \scriptstyle{\pm 0.026}$ & $0.664 \scriptstyle{\pm 0.075}$ / $0.089 \scriptstyle{\pm 0.021}$& 
%         $0.337 \scriptstyle{\pm 0.084}$ / $0.770 \scriptstyle{\pm 0.022}$ & $\mathbf{0.372 \scriptstyle{\pm 0.068}}$ / $0.270 \scriptstyle{\pm 0.033}$ & 
%         $0.008 \scriptstyle{\pm 0.006}$ / $0.710 \scriptstyle{\pm 0.029}$ & $0.031 \scriptstyle{\pm 0.028}$ / $0.314 \scriptstyle{\pm 0.042}$\\
%         % -------------------------------------------------------------- %
%         BESO  & 
%         $0.861 \scriptstyle{\pm 0.016}$ / $0.359 \scriptstyle{\pm 0.031}$ & $0.711 \scriptstyle{\pm 0.030}$ / $0.151 \scriptstyle{\pm 0.051}$ & 
%         $0.188 \scriptstyle{\pm 0.042}$ & $0.232 \scriptstyle{\pm 0.040}$ & 
%         $0.0 \scriptstyle{\pm 0.0}$ & $0.0 \scriptstyle{\pm 0.0}$ \\

%         % \midrule
%         VAE-ACT &
%         $\mathbf{0.891 \scriptstyle{\pm 0.022}}$ / $0.166 \scriptstyle{\pm 0.017}$ & $0.025 \scriptstyle{\pm 0.012}$ / $0.021 \scriptstyle{\pm 0.011}$ & 
%         $\mathbf{0.565 \scriptstyle{\pm 0.108}}$ / $0.717 \scriptstyle{\pm 0.038}$ & $0.114 \scriptstyle{\pm 0.020}$ / $0.217 \scriptstyle{\pm 0.024}$& 
%         $0.033 \scriptstyle{\pm 0.022}$ / $0.604 \scriptstyle{\pm 0.017}$ & $0.062 \scriptstyle{\pm 0.024}$ / $0.276 \scriptstyle{\pm 0.007}$
%         \\
%         % \midrule
%         DDPM-ACT &
%         $0.849 \scriptstyle{\pm 0.023}$ / $0.278 \scriptstyle{\pm 0.071}$& $\mathbf{0.749 \scriptstyle{\pm 0.041}}$ / $0.139 \scriptstyle{\pm 0.054}$& 
%         $0.300 \scriptstyle{\pm 0.060}$ & $0.300 \scriptstyle{\pm 0.051}$ & 
%         $0.001 \scriptstyle{\pm 0}$ & $0.0 \scriptstyle{\pm 0.0}$ 
%         \\
% 	\bottomrule
% \end{tabular}

% }

% \vskip -0.15in
% \end{table}


==> results/tables/bet_num_bins.tex <==
\begin{table}[hbtp]
\centering
 \caption{Ablation study of action clusters on Avoiding and Aligning}\label{bet_num_bins}
 
\resizebox{\textwidth}{!}{  

\begin{tabular}{lc|cc|cc}
	\toprule 
            & & \multicolumn{2}{c|}{Avoiding} & \multicolumn{2}{c}{Aligning} \\
            
        \midrule

         & action clusters & Success Rate & Entropy & Success Rate & Entropy \\

	\midrule

        BeT & 8 & $0.670 \scriptstyle{\pm 0.054}$ & $0.804 \scriptstyle{\pm 0.066}$ & $0.601            \scriptstyle{\pm 0.057}$ & $0.498 \scriptstyle{\pm 0.074}$ \\
        
                 & 16 & $0.754 \scriptstyle{\pm 0.038}$ & $0.782 \scriptstyle{\pm 0.043}$ & $0.656 \scriptstyle{\pm 0.021}$ & $0.463 \scriptstyle{\pm 0.080}$ \\
                 
                 & 32 & $0.749 \scriptstyle{\pm 0.046}$ & $0.804 \scriptstyle{\pm 0.045}$ & $0.709 \scriptstyle{\pm 0.032}$ & $0.547 \scriptstyle{\pm 0.070}$ \\
                 
                 & 64 & $0.747 \scriptstyle{\pm 0.030}$ & $0.844 \scriptstyle{\pm 0.035}$ & 
                     $0.645 \scriptstyle{\pm 0.069}$ & $0.536 \scriptstyle{\pm 0.105}$ \\
        
	\bottomrule
\end{tabular}

}
\vskip -0.15in
\end{table}



==> results/tables/diffusion_steps.tex <==
\begin{table}[hbtp]
\centering
 \caption{Ablation study of diffusion steps on Avoiding and Aligning}\label{diffusion_steps}
 
\resizebox{\textwidth}{!}{  

\begin{tabular}{lc|cc|cc}
	\toprule 
            & & \multicolumn{2}{c|}{Avoiding} & \multicolumn{2}{c}{Aligning} \\
            
        \midrule

         & diffusion steps & Success Rate & Entropy & Success Rate & Entropy \\

	\midrule

        DDPM-GPT & 4 & $0.951 \scriptstyle{\pm 0.021}$ & $0.847 \scriptstyle{\pm 0.026}$ & $0.879 \scriptstyle{\pm 0.017}$ & $0.525 \scriptstyle{\pm 0.088}$ \\
                 & 8 & $0.927 \scriptstyle{\pm 0.022}$ & $0.898 \scriptstyle{\pm 0.018}$ & $0.839 \scriptstyle{\pm 0.015}$ & $0.658 \scriptstyle{\pm 0.074}$ \\
                 & 16 & $0.917 \scriptstyle{\pm 0.015}$ & $0.930 \scriptstyle{\pm 0.013}$ & $0.839 \scriptstyle{\pm 0.020}$ & $0.664 \scriptstyle{\pm 0.075}$ \\
                 & 32 & $0.894 \scriptstyle{\pm 0.017}$ & $0.938 \scriptstyle{\pm 0.004}$ & $0.850 \scriptstyle{\pm 0.020}$ & $0.707 \scriptstyle{\pm 0.055}$ \\
      \midrule
      
        BESO & 4 & $0.917 \scriptstyle{\pm 0.019}$ & $0.839 \scriptstyle{\pm 0.026}$ & $0.909 \scriptstyle{\pm 0.011}$ & $0.423 \scriptstyle{\pm 0.074}$ \\
             & 8 & $0.950 \scriptstyle{\pm 0.015}$ & $0.856 \scriptstyle{\pm 0.018}$ & $0.878 \scriptstyle{\pm 0.015}$ & $0.561 \scriptstyle{\pm 0.065}$ \\
             & 16 & $0.944 \scriptstyle{\pm 0.010}$ & $0.864 \scriptstyle{\pm 0.015}$ & $0.861 \scriptstyle{\pm 0.016}$ & $0.711 \scriptstyle{\pm 0.030}$ \\
             & 32 & $0.938 \scriptstyle{\pm 0.009}$ & $0.868 \scriptstyle{\pm 0.020}$ & $0.865 \scriptstyle{\pm 0.021}$ & $0.733 \scriptstyle{\pm 0.031}$ \\
        
	\bottomrule
\end{tabular}

}
\vskip -0.15in
\end{table}



==> results/tables/image.tex <==
\begin{table}[hbtp]
\centering
 \caption{Performance of IL methods using image-based states in Aligning, Sorting-4 and Sorting-6 tasks}\label{image_table}
\resizebox{\textwidth}{!}{  

\begin{tabular}{l|cc|cc|cc}
	\toprule 
            & \multicolumn{2}{c|}{Aligning} & \multicolumn{2}{c|}{Sorting-4} & \multicolumn{2}{c}{Sorting-6} \\
            
        \midrule

        & Success Rate & Entropy & Success Rate & Entropy & S1 & Entropy \\

	\midrule

        BC-MLP  & 
        $0.148 \scriptstyle{\pm 0.045}$ & $0.0 \scriptstyle{\pm 0.0}$ &
        $0.666 \scriptstyle{\pm 0.080}$ & $0.0 \scriptstyle{\pm 0.0}$ & 
        $0.636 \scriptstyle{\pm 0.026}$ & $0.0 \scriptstyle{\pm 0.0}$  
         \\
        % -------------------------------------------------------------- %
        % BC-GMM  & 
        % 0 & 0 & 
        % 0 & 0 & 
        % 0 & 0 \\
        % -------------------------------------------------------------- %
        VAE-State & 
        $0.121 \scriptstyle{\pm 0.035}$ & $0.013 \scriptstyle{\pm 0.019}$ &
        $0.653 \scriptstyle{\pm 0.061}$ & $0.165 \scriptstyle{\pm 0.010}$ & 
        $0.570 \scriptstyle{\pm 0.023}$ & $0.236 \scriptstyle{\pm 0.013}$ \\
        % $0.517 \scriptstyle{\pm 0.059}$ & $0.038 \scriptstyle{\pm 0.022}$\\
        % -------------------------------------------------------------- %
        BeT-MLP & 
        $0.203 \scriptstyle{\pm 0.035}$ & $0.053 \scriptstyle{\pm 0.028}$ &
        $0.671 \scriptstyle{\pm 0.014}$ & $\mathbf{0.296 \scriptstyle{\pm 0.033}}$ & 
        $0.616 \scriptstyle{\pm 0.035}$ & $\mathbf{0.365 \scriptstyle{\pm 0.022}}$ \\ 
        % $0.467 \scriptstyle{\pm 0.046}$ & $0.195 \scriptstyle{\pm 0.044}$\\
        % -------------------------------------------------------------- %
        IBC & 
        $0.179 \scriptstyle{\pm 0.028}$ & $\mathbf{0.071 \scriptstyle{\pm 0.052}}$ &
        $0.707 \scriptstyle{\pm 0.031}$ & $0.236 \scriptstyle{\pm 0.027}$ & 
        $0.664 \scriptstyle{\pm 0.039}$ & $0.328 \scriptstyle{\pm 0.026}$ \\ 
        % $0.002 \scriptstyle{\pm 0.003}$ & $0.0 \scriptstyle{\pm 0.0}$\\
        % -------------------------------------------------------------- %
        DDPM-MLP & 
        $\mathbf{0.233 \scriptstyle{\pm 0.029}}$ & $0.060 \scriptstyle{\pm 0.033}$& 
        $\mathbf{0.763 \scriptstyle{\pm 0.028}}$ & $0.237 \scriptstyle{\pm 0.028}$ & 
        $\mathbf{0.748 \scriptstyle{\pm 0.026}}$ & $0.359 \scriptstyle{\pm 0.025}$ \\ 
        % $0.645 \scriptstyle{\pm 0.050}$ & $0.137 \scriptstyle{\pm 0.061}$\\
        % -------------------------------------------------------------- %
 %        \midrule

 %         & Success Rate & Entropy & Success Rate & Entropy & Success Rate & Entropy \\

	% \midrule

        BC-GPT  & 
        $0.084 \scriptstyle{\pm 0.015}$ & $0.0 \scriptstyle{\pm 0.0}$ &
        $0.654 \scriptstyle{\pm 0.048}$ & $0.0 \scriptstyle{\pm 0.0}$ & 
        $0.590 \scriptstyle{\pm 0.017}$ & $0.0 \scriptstyle{\pm 0.0}$ \\
        % $0.515 \scriptstyle{\pm 0.092}$ & $0.236 \scriptstyle{\pm 0.086}$ \\
        % -------------------------------------------------------------- %
        % LSTM-GMM & 
        % 0 & 0 & 
        % 0 & 0 & 
        % 0 & 0\\
        % -------------------------------------------------------------- %
        BeT & 
        $0.154 \scriptstyle{\pm 0.067}$ & $0.023 \scriptstyle{\pm 0.012}$&
        $0.676 \scriptstyle{\pm 0.035}$ & $\mathbf{0.305 \scriptstyle{\pm 0.029}}$ & 
        $0.617 \scriptstyle{\pm 0.033}$ & $\mathbf{0.380 \scriptstyle{\pm 0.019}}$ \\
        % $0.500 \scriptstyle{\pm 0.054}$ & $0.325 \scriptstyle{\pm 0.082}$\\
        % -------------------------------------------------------------- %
        DDPM-GPT & 
        $0.316 \scriptstyle{\pm 0.026}$ & $0.089 \scriptstyle{\pm 0.021}$ & 
        $\mathbf{0.770 \scriptstyle{\pm 0.022}}$ & $0.270 \scriptstyle{\pm 0.033}$ & 
        $0.710 \scriptstyle{\pm 0.029}$ & $0.314 \scriptstyle{\pm 0.042}$ \\ 
        % $0.704 \scriptstyle{\pm 0.024}$ & $0.349 \scriptstyle{\pm 0.053}$\\
        % -------------------------------------------------------------- %
        BESO  & 
        $\mathbf{0.359 \scriptstyle{\pm 0.031}}$ & $\mathbf{0.151 \scriptstyle{\pm 0.051}}$ & 
        $0.764 \scriptstyle{\pm 0.026}$ & $0.281 \scriptstyle{\pm 0.035}$ & 
        $\mathbf{0.719 \scriptstyle{\pm 0.025}}$ & $0.352 \scriptstyle{\pm 0.018}$\\

        % \midrule
        VAE-ACT &
        $0.166 \scriptstyle{\pm 0.017}$ & $0.021 \scriptstyle{\pm 0.011}$ &
        $0.717 \scriptstyle{\pm 0.038}$ & $0.217 \scriptstyle{\pm 0.024}$ & 
        $0.604 \scriptstyle{\pm 0.017}$ & $0.276 \scriptstyle{\pm 0.007}$ 
        % $0.572 \scriptstyle{\pm 0.081}$ & $0.219 \scriptstyle{\pm 0.051}$
        \\

        % \midrule
        DDPM-ACT &
        $0.278 \scriptstyle{\pm 0.071}$ & $0.139 \scriptstyle{\pm 0.054}$ &
        $0.659 \scriptstyle{\pm 0.063}$ & $0.346 \scriptstyle{\pm 0.028}$ & 
        $0.643 \scriptstyle{\pm 0.036}$ & $0.397 \scriptstyle{\pm 0.025}$ 
        % $0.572 \scriptstyle{\pm 0.081}$ & $0.219 \scriptstyle{\pm 0.051}$
        \\
        
	\bottomrule
\end{tabular}

}
\vskip -0.15in
\end{table}



\begin{table}[hbtp]
\centering
 \caption{Performance of IL methods using image-based states in Aligning, Sorting-4 and Sorting-6 tasks}\label{image_table}
\resizebox{\textwidth}{!}{  

\begin{tabular}{l|cc|cc|cc}
	\toprule 
            & \multicolumn{2}{c|}{Aligning (T2)} & \multicolumn{2}{c|}{Sorting-4 (T4)} & \multicolumn{2}{c}{Sorting-6 (T4)} \\
            
        \midrule

        & Success Rate & Entropy & Success Rate & Entropy & S1 & Entropy \\

	\midrule

        \nohist{BC-MLP}  & 
        \nohist{$0.148 \scriptstyle{\pm 0.045}$} & \nohist{$0.0 \scriptstyle{\pm 0.0}$} &
        \nohist{$0.666 \scriptstyle{\pm 0.080}$} & \nohist{$0.0 \scriptstyle{\pm 0.0}$} & 
        \nohist{$0.636 \scriptstyle{\pm 0.026}$} & \nohist{$0.0 \scriptstyle{\pm 0.0}$}  
         \\
        % -------------------------------------------------------------- %
        % BC-GMM  & 
        % 0 & 0 & 
        % 0 & 0 & 
        % 0 & 0 \\
        % -------------------------------------------------------------- %
        \nohist{VAE-State}  &
        \nohist{$0.203 \scriptstyle{\pm 0.035}$} & \nohist{$0.053 \scriptstyle{\pm 0.028}$} &
        \nohist{$0.671 \scriptstyle{\pm 0.014}$} & \nohist{$\mathbf{0.296 \scriptstyle{\pm 0.033}}$} & 
        \nohist{$0.616 \scriptstyle{\pm 0.035}$} & \nohist{$\mathbf{0.365 \scriptstyle{\pm 0.022}}$ } \\ 
        % $0.467 \scriptstyle{\pm 0.046}$ & $0.195 \scriptstyle{\pm 0.044}$\\
        % -------------------------------------------------------------- %
        \nohist{IBC} & 
        \nohist{$0.179 \scriptstyle{\pm 0.028}$ }& \nohist{$\mathbf{0.071 \scriptstyle{\pm 0.052}}$ }&
        \nohist{$0.707 \scriptstyle{\pm 0.031}$ }& \nohist{$0.236 \scriptstyle{\pm 0.027}$ }& 
        \nohist{$0.664 \scriptstyle{\pm 0.039}$ }& \nohist{$0.328 \scriptstyle{\pm 0.026}$ }\\ 
        % $0.002 \scriptstyle{\pm 0.003}$ & $0.0 \scriptstyle{\pm 0.0}$\\
        % -------------------------------------------------------------- %
        \nohist{DDPM-MLP} & 
        \nohist{$\mathbf{0.233 \scriptstyle{\pm 0.029}}$} & \nohist{$0.060 \scriptstyle{\pm 0.033}$}& 
        \nohist{$\mathbf{0.763 \scriptstyle{\pm 0.028}}$} & \nohist{$0.237 \scriptstyle{\pm 0.028}$} & 
        \nohist{$\mathbf{0.748 \scriptstyle{\pm 0.026}}$} & \nohist{$0.359 \scriptstyle{\pm 0.025}$} \\ 
        % $0.645 \scriptstyle{\pm 0.050}$ & $0.137 \scriptstyle{\pm 0.061}$\\
        % -------------------------------------------------------------- %
                \midrule

        \ac{VAE-ACT} &
        \ac{$0.166 \scriptstyle{\pm 0.017}$} & \ac{$0.021 \scriptstyle{\pm 0.011}$} &
        \ac{$0.717 \scriptstyle{\pm 0.038}$} & \ac{$0.217 \scriptstyle{\pm 0.024}$} & 
        \ac{$0.604 \scriptstyle{\pm 0.017}$} & \ac{$0.276 \scriptstyle{\pm 0.007}$} 
        % $0.572 \scriptstyle{\pm 0.081}$ & $0.219 \scriptstyle{\pm 0.051}$
        \\

        
        \midrule

 %         & Success Rate & Entropy & Success Rate & Entropy & Success Rate & Entropy \\

	% \midrule

        \hist{BC-GPT}  & 
        \hist{$0.084 \scriptstyle{\pm 0.015}$} & \hist{$0.0 \scriptstyle{\pm 0.0}$} &
        \hist{$0.654 \scriptstyle{\pm 0.048}$} & \hist{$0.0 \scriptstyle{\pm 0.0}$} & 
        \hist{$0.590 \scriptstyle{\pm 0.017}$} & \hist{$0.0 \scriptstyle{\pm 0.0}$} \\
        % $0.515 \scriptstyle{\pm 0.092}$ & $0.236 \scriptstyle{\pm 0.086}$ \\
        % -------------------------------------------------------------- %
        % LSTM-GMM & 
        % 0 & 0 & 
        % 0 & 0 & 
        % 0 & 0\\
        % -------------------------------------------------------------- %
        \hist{BeT} & 
        \hist{$0.154 \scriptstyle{\pm 0.067}$} & \hist{$0.023 \scriptstyle{\pm 0.012}$}&
        \hist{$0.676 \scriptstyle{\pm 0.035}$} & \hist{$\mathbf{0.305 \scriptstyle{\pm 0.029}}$} & 
        \hist{$0.617 \scriptstyle{\pm 0.033}$} & \hist{$\mathbf{0.380 \scriptstyle{\pm 0.019}}$} \\
        % $0.500 \scriptstyle{\pm 0.054}$ & $0.325 \scriptstyle{\pm 0.082}$\\
        % -------------------------------------------------------------- %
        \hist{DDPM-GPT} & 
        \hist{$0.316 \scriptstyle{\pm 0.026}$} & \hist{$0.089 \scriptstyle{\pm 0.021}$} & 
        \hist{$\mathbf{0.770 \scriptstyle{\pm 0.022}}$} & \hist{$0.270 \scriptstyle{\pm 0.033}$} & 
        \hist{$0.710 \scriptstyle{\pm 0.029}$} & \hist{$0.314 \scriptstyle{\pm 0.042}$} \\ 
        % $0.704 \scriptstyle{\pm 0.024}$ & $0.349 \scriptstyle{\pm 0.053}$\\
        % -------------------------------------------------------------- %
        \hist{BESO}  & 
        \hist{$\mathbf{0.359 \scriptstyle{\pm 0.031}}$} & \hist{$\mathbf{0.151 \scriptstyle{\pm 0.051}}$ }& 
        \hist{$0.764 \scriptstyle{\pm 0.026}$} & \hist{$0.281 \scriptstyle{\pm 0.035}$ }& 
        \hist{$\mathbf{0.719 \scriptstyle{\pm 0.025}}$} & \hist{$0.352 \scriptstyle{\pm 0.018}$}
        \\

        \midrule
        \both{DDPM-ACT} &
        \both{$0.278 \scriptstyle{\pm 0.071}$} & \both{$0.139 \scriptstyle{\pm 0.054}$} &
        \both{$0.659 \scriptstyle{\pm 0.063}$} & \both{$0.346 \scriptstyle{\pm 0.028}$} & 
        \both{$0.643 \scriptstyle{\pm 0.036}$} & \both{$0.397 \scriptstyle{\pm 0.025}$} 
        % $0.572 \scriptstyle{\pm 0.081}$ & $0.219 \scriptstyle{\pm 0.051}$
        \\
        
	\bottomrule
\end{tabular}

}
\vskip -0.15in
\end{table}






%T%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[hbtp]
\centering
 \caption{
 Performance of IL methods using image-based states in Aligning, Sorting-4 and Sorting-6 tasks.
  Performance of IL methods using image-based states in Aligning, Sorting-4 and Sorting-6 tasks.
   Performance of IL methods using image-based states in Aligning, Sorting-4 and Sorting-6 tasks.
 Performance of IL methods using image-based states in Aligning, Sorting-4 and Sorting-6 tasks.
 }\label{image_table}
\resizebox{\textwidth}{!}{  

\begin{tabular}{l|cc|cc|cc}
	\toprule 
        & Success Rate & Entropy & Success Rate & Entropy & S1 & Entropy \\
        \midrule
            & \multicolumn{2}{c|}{Aligning (T2)} & \multicolumn{2}{c|}{Sorting-4 (T4)} & \multicolumn{2}{c}{Sorting-6 (T4)} \\
	\midrule
        \nohist{BC-MLP}  & 
        \nohist{$0.148 \scriptstyle{\pm 0.045}$} & \nohist{$0.0 \scriptstyle{\pm 0.0}$} &
        \nohist{$0.666 \scriptstyle{\pm 0.080}$} & \nohist{$0.0 \scriptstyle{\pm 0.0}$} & 
        \nohist{$0.636 \scriptstyle{\pm 0.026}$} & \nohist{$0.0 \scriptstyle{\pm 0.0}$}   \\
        % -------------------------------------------------------------- %
        \nohist{VAE-State}  &
        \nohist{$0.203 \scriptstyle{\pm 0.035}$} & \nohist{$0.053 \scriptstyle{\pm 0.028}$} &
        \nohist{$0.671 \scriptstyle{\pm 0.014}$} & \nohist{$\mathbf{0.296 \scriptstyle{\pm 0.033}}$} & 
        \nohist{$0.616 \scriptstyle{\pm 0.035}$} & \nohist{$\mathbf{0.365 \scriptstyle{\pm 0.022}}$ } \\ 
        % -------------------------------------------------------------- %
        \nohist{IBC} & 
        \nohist{$0.179 \scriptstyle{\pm 0.028}$ }& \nohist{$\mathbf{0.071 \scriptstyle{\pm 0.052}}$ }&
        \nohist{$0.707 \scriptstyle{\pm 0.031}$ }& \nohist{$0.236 \scriptstyle{\pm 0.027}$ }& 
        \nohist{$0.664 \scriptstyle{\pm 0.039}$ }& \nohist{$0.328 \scriptstyle{\pm 0.026}$ }\\ 
        % -------------------------------------------------------------- %
        \nohist{DDPM-MLP} & 
        \nohist{$\mathbf{0.233 \scriptstyle{\pm 0.029}}$} & \nohist{$0.060 \scriptstyle{\pm 0.033}$}& 
        \nohist{$\mathbf{0.763 \scriptstyle{\pm 0.028}}$} & \nohist{$0.237 \scriptstyle{\pm 0.028}$} & 
        \nohist{$\mathbf{0.748 \scriptstyle{\pm 0.026}}$} & \nohist{$0.359 \scriptstyle{\pm 0.025}$} \\ 
        % -------------------------------------------------------------- %
        \ac{VAE-ACT} &
        \ac{$0.166 \scriptstyle{\pm 0.017}$} & \ac{$0.021 \scriptstyle{\pm 0.011}$} &
        \ac{$0.717 \scriptstyle{\pm 0.038}$} & \ac{$0.217 \scriptstyle{\pm 0.024}$} & 
        \ac{$0.604 \scriptstyle{\pm 0.017}$} & \ac{$0.276 \scriptstyle{\pm 0.007}$} \\
        % -------------------------------------------------------------- %
        \hist{BC-GPT}  & 
        \hist{$0.084 \scriptstyle{\pm 0.015}$} & \hist{$0.0 \scriptstyle{\pm 0.0}$} &
        \hist{$0.654 \scriptstyle{\pm 0.048}$} & \hist{$0.0 \scriptstyle{\pm 0.0}$} & 
        \hist{$0.590 \scriptstyle{\pm 0.017}$} & \hist{$0.0 \scriptstyle{\pm 0.0}$} \\
        % -------------------------------------------------------------- %
        \hist{BeT} & 
        \hist{$0.154 \scriptstyle{\pm 0.067}$} & \hist{$0.023 \scriptstyle{\pm 0.012}$}&
        \hist{$0.676 \scriptstyle{\pm 0.035}$} & \hist{$\mathbf{0.305 \scriptstyle{\pm 0.029}}$} & 
        \hist{$0.617 \scriptstyle{\pm 0.033}$} & \hist{$\mathbf{0.380 \scriptstyle{\pm 0.019}}$} \\
        % -------------------------------------------------------------- %
        \hist{DDPM-GPT} & 
        \hist{$0.316 \scriptstyle{\pm 0.026}$} & \hist{$0.089 \scriptstyle{\pm 0.021}$} & 
        \hist{$\mathbf{0.770 \scriptstyle{\pm 0.022}}$} & \hist{$0.270 \scriptstyle{\pm 0.033}$} & 
        \hist{$0.710 \scriptstyle{\pm 0.029}$} & \hist{$0.314 \scriptstyle{\pm 0.042}$} \\ 
        % -------------------------------------------------------------- %
        \hist{BESO}  & 
        \hist{$\mathbf{0.359 \scriptstyle{\pm 0.031}}$} & \hist{$\mathbf{0.151 \scriptstyle{\pm 0.051}}$ }& 
        \hist{$0.764 \scriptstyle{\pm 0.026}$} & \hist{$0.281 \scriptstyle{\pm 0.035}$ }& 
        \hist{$\mathbf{0.719 \scriptstyle{\pm 0.025}}$} & \hist{$0.352 \scriptstyle{\pm 0.018}$} \\
        % -------------------------------------------------------------- %
        \both{DDPM-ACT} &
        \both{$0.278 \scriptstyle{\pm 0.071}$} & \both{$0.139 \scriptstyle{\pm 0.054}$} &
        \both{$0.659 \scriptstyle{\pm 0.063}$} & \both{$0.346 \scriptstyle{\pm 0.028}$} & 
        \both{$0.643 \scriptstyle{\pm 0.036}$} & \both{$0.397 \scriptstyle{\pm 0.025}$} \\
        % -------------------------------------------------------------- %
        \midrule
            & \multicolumn{2}{c|}{Aligning (T2)} & \multicolumn{2}{c|}{Sorting-4 (T4)} & \multicolumn{2}{c}{Sorting-6 (T4)} \\
	\midrule
        \nohist{BC-MLP}  & 
        \nohist{$0.148 \scriptstyle{\pm 0.045}$} & \nohist{$0.0 \scriptstyle{\pm 0.0}$} &
        \nohist{$0.666 \scriptstyle{\pm 0.080}$} & \nohist{$0.0 \scriptstyle{\pm 0.0}$} & 
        \nohist{$0.636 \scriptstyle{\pm 0.026}$} & \nohist{$0.0 \scriptstyle{\pm 0.0}$}   \\
        % -------------------------------------------------------------- %
        \nohist{VAE-State}  &
        \nohist{$0.203 \scriptstyle{\pm 0.035}$} & \nohist{$0.053 \scriptstyle{\pm 0.028}$} &
        \nohist{$0.671 \scriptstyle{\pm 0.014}$} & \nohist{$\mathbf{0.296 \scriptstyle{\pm 0.033}}$} & 
        \nohist{$0.616 \scriptstyle{\pm 0.035}$} & \nohist{$\mathbf{0.365 \scriptstyle{\pm 0.022}}$ } \\ 
        % -------------------------------------------------------------- %
        \nohist{IBC} & 
        \nohist{$0.179 \scriptstyle{\pm 0.028}$ }& \nohist{$\mathbf{0.071 \scriptstyle{\pm 0.052}}$ }&
        \nohist{$0.707 \scriptstyle{\pm 0.031}$ }& \nohist{$0.236 \scriptstyle{\pm 0.027}$ }& 
        \nohist{$0.664 \scriptstyle{\pm 0.039}$ }& \nohist{$0.328 \scriptstyle{\pm 0.026}$ }\\ 
        % -------------------------------------------------------------- %
        \nohist{DDPM-MLP} & 
        \nohist{$\mathbf{0.233 \scriptstyle{\pm 0.029}}$} & \nohist{$0.060 \scriptstyle{\pm 0.033}$}& 
        \nohist{$\mathbf{0.763 \scriptstyle{\pm 0.028}}$} & \nohist{$0.237 \scriptstyle{\pm 0.028}$} & 
        \nohist{$\mathbf{0.748 \scriptstyle{\pm 0.026}}$} & \nohist{$0.359 \scriptstyle{\pm 0.025}$} \\ 
        % -------------------------------------------------------------- %
        \ac{VAE-ACT} &
        \ac{$0.166 \scriptstyle{\pm 0.017}$} & \ac{$0.021 \scriptstyle{\pm 0.011}$} &
        \ac{$0.717 \scriptstyle{\pm 0.038}$} & \ac{$0.217 \scriptstyle{\pm 0.024}$} & 
        \ac{$0.604 \scriptstyle{\pm 0.017}$} & \ac{$0.276 \scriptstyle{\pm 0.007}$} \\
        % -------------------------------------------------------------- %
        \hist{BC-GPT}  & 
        \hist{$0.084 \scriptstyle{\pm 0.015}$} & \hist{$0.0 \scriptstyle{\pm 0.0}$} &
        \hist{$0.654 \scriptstyle{\pm 0.048}$} & \hist{$0.0 \scriptstyle{\pm 0.0}$} & 
        \hist{$0.590 \scriptstyle{\pm 0.017}$} & \hist{$0.0 \scriptstyle{\pm 0.0}$} \\
        % -------------------------------------------------------------- %
        \hist{BeT} & 
        \hist{$0.154 \scriptstyle{\pm 0.067}$} & \hist{$0.023 \scriptstyle{\pm 0.012}$}&
        \hist{$0.676 \scriptstyle{\pm 0.035}$} & \hist{$\mathbf{0.305 \scriptstyle{\pm 0.029}}$} & 
        \hist{$0.617 \scriptstyle{\pm 0.033}$} & \hist{$\mathbf{0.380 \scriptstyle{\pm 0.019}}$} \\
        % -------------------------------------------------------------- %
        \hist{DDPM-GPT} & 
        \hist{$0.316 \scriptstyle{\pm 0.026}$} & \hist{$0.089 \scriptstyle{\pm 0.021}$} & 
        \hist{$\mathbf{0.770 \scriptstyle{\pm 0.022}}$} & \hist{$0.270 \scriptstyle{\pm 0.033}$} & 
        \hist{$0.710 \scriptstyle{\pm 0.029}$} & \hist{$0.314 \scriptstyle{\pm 0.042}$} \\ 
        % -------------------------------------------------------------- %
        \hist{BESO}  & 
        \hist{$\mathbf{0.359 \scriptstyle{\pm 0.031}}$} & \hist{$\mathbf{0.151 \scriptstyle{\pm 0.051}}$ }& 
        \hist{$0.764 \scriptstyle{\pm 0.026}$} & \hist{$0.281 \scriptstyle{\pm 0.035}$ }& 
        \hist{$\mathbf{0.719 \scriptstyle{\pm 0.025}}$} & \hist{$0.352 \scriptstyle{\pm 0.018}$} \\
        % -------------------------------------------------------------- %
        \both{DDPM-ACT} &
        \both{$0.278 \scriptstyle{\pm 0.071}$} & \both{$0.139 \scriptstyle{\pm 0.054}$} &
        \both{$0.659 \scriptstyle{\pm 0.063}$} & \both{$0.346 \scriptstyle{\pm 0.028}$} & 
        \both{$0.643 \scriptstyle{\pm 0.036}$} & \both{$0.397 \scriptstyle{\pm 0.025}$} \\
        % -------------------------------------------------------------- %
        \midrule
            & \multicolumn{2}{c|}{Aligning (T2)} & \multicolumn{2}{c|}{Sorting-4 (T4)} & \multicolumn{2}{c}{Sorting-6 (T4)} \\
	\midrule
        \nohist{BC-MLP}  & 
        \nohist{$0.148 \scriptstyle{\pm 0.045}$} & \nohist{$0.0 \scriptstyle{\pm 0.0}$} &
        \nohist{$0.666 \scriptstyle{\pm 0.080}$} & \nohist{$0.0 \scriptstyle{\pm 0.0}$} & 
        \nohist{$0.636 \scriptstyle{\pm 0.026}$} & \nohist{$0.0 \scriptstyle{\pm 0.0}$}   \\
        % -------------------------------------------------------------- %
        \nohist{VAE-State}  &
        \nohist{$0.203 \scriptstyle{\pm 0.035}$} & \nohist{$0.053 \scriptstyle{\pm 0.028}$} &
        \nohist{$0.671 \scriptstyle{\pm 0.014}$} & \nohist{$\mathbf{0.296 \scriptstyle{\pm 0.033}}$} & 
        \nohist{$0.616 \scriptstyle{\pm 0.035}$} & \nohist{$\mathbf{0.365 \scriptstyle{\pm 0.022}}$ } \\ 
        % -------------------------------------------------------------- %
        \nohist{IBC} & 
        \nohist{$0.179 \scriptstyle{\pm 0.028}$ }& \nohist{$\mathbf{0.071 \scriptstyle{\pm 0.052}}$ }&
        \nohist{$0.707 \scriptstyle{\pm 0.031}$ }& \nohist{$0.236 \scriptstyle{\pm 0.027}$ }& 
        \nohist{$0.664 \scriptstyle{\pm 0.039}$ }& \nohist{$0.328 \scriptstyle{\pm 0.026}$ }\\ 
        % -------------------------------------------------------------- %
        \nohist{DDPM-MLP} & 
        \nohist{$\mathbf{0.233 \scriptstyle{\pm 0.029}}$} & \nohist{$0.060 \scriptstyle{\pm 0.033}$}& 
        \nohist{$\mathbf{0.763 \scriptstyle{\pm 0.028}}$} & \nohist{$0.237 \scriptstyle{\pm 0.028}$} & 
        \nohist{$\mathbf{0.748 \scriptstyle{\pm 0.026}}$} & \nohist{$0.359 \scriptstyle{\pm 0.025}$} \\ 
        % -------------------------------------------------------------- %
        \ac{VAE-ACT} &
        \ac{$0.166 \scriptstyle{\pm 0.017}$} & \ac{$0.021 \scriptstyle{\pm 0.011}$} &
        \ac{$0.717 \scriptstyle{\pm 0.038}$} & \ac{$0.217 \scriptstyle{\pm 0.024}$} & 
        \ac{$0.604 \scriptstyle{\pm 0.017}$} & \ac{$0.276 \scriptstyle{\pm 0.007}$} \\
        % -------------------------------------------------------------- %
        \hist{BC-GPT}  & 
        \hist{$0.084 \scriptstyle{\pm 0.015}$} & \hist{$0.0 \scriptstyle{\pm 0.0}$} &
        \hist{$0.654 \scriptstyle{\pm 0.048}$} & \hist{$0.0 \scriptstyle{\pm 0.0}$} & 
        \hist{$0.590 \scriptstyle{\pm 0.017}$} & \hist{$0.0 \scriptstyle{\pm 0.0}$} \\
        % -------------------------------------------------------------- %
        \hist{BeT} & 
        \hist{$0.154 \scriptstyle{\pm 0.067}$} & \hist{$0.023 \scriptstyle{\pm 0.012}$}&
        \hist{$0.676 \scriptstyle{\pm 0.035}$} & \hist{$\mathbf{0.305 \scriptstyle{\pm 0.029}}$} & 
        \hist{$0.617 \scriptstyle{\pm 0.033}$} & \hist{$\mathbf{0.380 \scriptstyle{\pm 0.019}}$} \\
        % -------------------------------------------------------------- %
        \hist{DDPM-GPT} & 
        \hist{$0.316 \scriptstyle{\pm 0.026}$} & \hist{$0.089 \scriptstyle{\pm 0.021}$} & 
        \hist{$\mathbf{0.770 \scriptstyle{\pm 0.022}}$} & \hist{$0.270 \scriptstyle{\pm 0.033}$} & 
        \hist{$0.710 \scriptstyle{\pm 0.029}$} & \hist{$0.314 \scriptstyle{\pm 0.042}$} \\ 
        % -------------------------------------------------------------- %
        \hist{BESO}  & 
        \hist{$\mathbf{0.359 \scriptstyle{\pm 0.031}}$} & \hist{$\mathbf{0.151 \scriptstyle{\pm 0.051}}$ }& 
        \hist{$0.764 \scriptstyle{\pm 0.026}$} & \hist{$0.281 \scriptstyle{\pm 0.035}$ }& 
        \hist{$\mathbf{0.719 \scriptstyle{\pm 0.025}}$} & \hist{$0.352 \scriptstyle{\pm 0.018}$} \\
        % -------------------------------------------------------------- %
        \both{DDPM-ACT} &
        \both{$0.278 \scriptstyle{\pm 0.071}$} & \both{$0.139 \scriptstyle{\pm 0.054}$} &
        \both{$0.659 \scriptstyle{\pm 0.063}$} & \both{$0.346 \scriptstyle{\pm 0.028}$} & 
        \both{$0.643 \scriptstyle{\pm 0.036}$} & \both{$0.397 \scriptstyle{\pm 0.025}$} \\
        % -------------------------------------------------------------- %
        \midrule
            & \multicolumn{2}{c|}{Aligning (T2)} & \multicolumn{2}{c|}{Sorting-4 (T4)} & \multicolumn{2}{c}{Sorting-6 (T4)} \\
	\midrule
        \nohist{BC-MLP}  & 
        \nohist{$0.148 \scriptstyle{\pm 0.045}$} & \nohist{$0.0 \scriptstyle{\pm 0.0}$} &
        \nohist{$0.666 \scriptstyle{\pm 0.080}$} & \nohist{$0.0 \scriptstyle{\pm 0.0}$} & 
        \nohist{$0.636 \scriptstyle{\pm 0.026}$} & \nohist{$0.0 \scriptstyle{\pm 0.0}$}   \\
        % -------------------------------------------------------------- %
        \nohist{VAE-State}  &
        \nohist{$0.203 \scriptstyle{\pm 0.035}$} & \nohist{$0.053 \scriptstyle{\pm 0.028}$} &
        \nohist{$0.671 \scriptstyle{\pm 0.014}$} & \nohist{$\mathbf{0.296 \scriptstyle{\pm 0.033}}$} & 
        \nohist{$0.616 \scriptstyle{\pm 0.035}$} & \nohist{$\mathbf{0.365 \scriptstyle{\pm 0.022}}$ } \\ 
        % -------------------------------------------------------------- %
        \nohist{IBC} & 
        \nohist{$0.179 \scriptstyle{\pm 0.028}$ }& \nohist{$\mathbf{0.071 \scriptstyle{\pm 0.052}}$ }&
        \nohist{$0.707 \scriptstyle{\pm 0.031}$ }& \nohist{$0.236 \scriptstyle{\pm 0.027}$ }& 
        \nohist{$0.664 \scriptstyle{\pm 0.039}$ }& \nohist{$0.328 \scriptstyle{\pm 0.026}$ }\\ 
        % -------------------------------------------------------------- %
        \nohist{DDPM-MLP} & 
        \nohist{$\mathbf{0.233 \scriptstyle{\pm 0.029}}$} & \nohist{$0.060 \scriptstyle{\pm 0.033}$}& 
        \nohist{$\mathbf{0.763 \scriptstyle{\pm 0.028}}$} & \nohist{$0.237 \scriptstyle{\pm 0.028}$} & 
        \nohist{$\mathbf{0.748 \scriptstyle{\pm 0.026}}$} & \nohist{$0.359 \scriptstyle{\pm 0.025}$} \\ 
        % -------------------------------------------------------------- %
        \ac{VAE-ACT} &
        \ac{$0.166 \scriptstyle{\pm 0.017}$} & \ac{$0.021 \scriptstyle{\pm 0.011}$} &
        \ac{$0.717 \scriptstyle{\pm 0.038}$} & \ac{$0.217 \scriptstyle{\pm 0.024}$} & 
        \ac{$0.604 \scriptstyle{\pm 0.017}$} & \ac{$0.276 \scriptstyle{\pm 0.007}$} \\
        % -------------------------------------------------------------- %
        \hist{BC-GPT}  & 
        \hist{$0.084 \scriptstyle{\pm 0.015}$} & \hist{$0.0 \scriptstyle{\pm 0.0}$} &
        \hist{$0.654 \scriptstyle{\pm 0.048}$} & \hist{$0.0 \scriptstyle{\pm 0.0}$} & 
        \hist{$0.590 \scriptstyle{\pm 0.017}$} & \hist{$0.0 \scriptstyle{\pm 0.0}$} \\
        % -------------------------------------------------------------- %
        \hist{BeT} & 
        \hist{$0.154 \scriptstyle{\pm 0.067}$} & \hist{$0.023 \scriptstyle{\pm 0.012}$}&
        \hist{$0.676 \scriptstyle{\pm 0.035}$} & \hist{$\mathbf{0.305 \scriptstyle{\pm 0.029}}$} & 
        \hist{$0.617 \scriptstyle{\pm 0.033}$} & \hist{$\mathbf{0.380 \scriptstyle{\pm 0.019}}$} \\
        % -------------------------------------------------------------- %
        \hist{DDPM-GPT} & 
        \hist{$0.316 \scriptstyle{\pm 0.026}$} & \hist{$0.089 \scriptstyle{\pm 0.021}$} & 
        \hist{$\mathbf{0.770 \scriptstyle{\pm 0.022}}$} & \hist{$0.270 \scriptstyle{\pm 0.033}$} & 
        \hist{$0.710 \scriptstyle{\pm 0.029}$} & \hist{$0.314 \scriptstyle{\pm 0.042}$} \\ 
        % -------------------------------------------------------------- %
        \hist{BESO}  & 
        \hist{$\mathbf{0.359 \scriptstyle{\pm 0.031}}$} & \hist{$\mathbf{0.151 \scriptstyle{\pm 0.051}}$ }& 
        \hist{$0.764 \scriptstyle{\pm 0.026}$} & \hist{$0.281 \scriptstyle{\pm 0.035}$ }& 
        \hist{$\mathbf{0.719 \scriptstyle{\pm 0.025}}$} & \hist{$0.352 \scriptstyle{\pm 0.018}$} \\
        % -------------------------------------------------------------- %
        \both{DDPM-ACT} &
        \both{$0.278 \scriptstyle{\pm 0.071}$} & \both{$0.139 \scriptstyle{\pm 0.054}$} &
        \both{$0.659 \scriptstyle{\pm 0.063}$} & \both{$0.346 \scriptstyle{\pm 0.028}$} & 
        \both{$0.643 \scriptstyle{\pm 0.036}$} & \both{$0.397 \scriptstyle{\pm 0.025}$} \\
        % -------------------------------------------------------------- %
        \midrule
            & \multicolumn{2}{c|}{Aligning (T2)} & \multicolumn{2}{c|}{Sorting-4 (T4)} & \multicolumn{2}{c}{Sorting-6 (T4)} \\
	\midrule
        \nohist{BC-MLP}  & 
        \nohist{$0.148 \scriptstyle{\pm 0.045}$} & \nohist{$0.0 \scriptstyle{\pm 0.0}$} &
        \nohist{$0.666 \scriptstyle{\pm 0.080}$} & \nohist{$0.0 \scriptstyle{\pm 0.0}$} & 
        \nohist{$0.636 \scriptstyle{\pm 0.026}$} & \nohist{$0.0 \scriptstyle{\pm 0.0}$}   \\
        % -------------------------------------------------------------- %
        \nohist{VAE-State}  &
        \nohist{$0.203 \scriptstyle{\pm 0.035}$} & \nohist{$0.053 \scriptstyle{\pm 0.028}$} &
        \nohist{$0.671 \scriptstyle{\pm 0.014}$} & \nohist{$\mathbf{0.296 \scriptstyle{\pm 0.033}}$} & 
        \nohist{$0.616 \scriptstyle{\pm 0.035}$} & \nohist{$\mathbf{0.365 \scriptstyle{\pm 0.022}}$ } \\ 
        % -------------------------------------------------------------- %
        \nohist{IBC} & 
        \nohist{$0.179 \scriptstyle{\pm 0.028}$ }& \nohist{$\mathbf{0.071 \scriptstyle{\pm 0.052}}$ }&
        \nohist{$0.707 \scriptstyle{\pm 0.031}$ }& \nohist{$0.236 \scriptstyle{\pm 0.027}$ }& 
        \nohist{$0.664 \scriptstyle{\pm 0.039}$ }& \nohist{$0.328 \scriptstyle{\pm 0.026}$ }\\ 
        % -------------------------------------------------------------- %
        \nohist{DDPM-MLP} & 
        \nohist{$\mathbf{0.233 \scriptstyle{\pm 0.029}}$} & \nohist{$0.060 \scriptstyle{\pm 0.033}$}& 
        \nohist{$\mathbf{0.763 \scriptstyle{\pm 0.028}}$} & \nohist{$0.237 \scriptstyle{\pm 0.028}$} & 
        \nohist{$\mathbf{0.748 \scriptstyle{\pm 0.026}}$} & \nohist{$0.359 \scriptstyle{\pm 0.025}$} \\ 
        % -------------------------------------------------------------- %
        \ac{VAE-ACT} &
        \ac{$0.166 \scriptstyle{\pm 0.017}$} & \ac{$0.021 \scriptstyle{\pm 0.011}$} &
        \ac{$0.717 \scriptstyle{\pm 0.038}$} & \ac{$0.217 \scriptstyle{\pm 0.024}$} & 
        \ac{$0.604 \scriptstyle{\pm 0.017}$} & \ac{$0.276 \scriptstyle{\pm 0.007}$} \\
        % -------------------------------------------------------------- %
        \hist{BC-GPT}  & 
        \hist{$0.084 \scriptstyle{\pm 0.015}$} & \hist{$0.0 \scriptstyle{\pm 0.0}$} &
        \hist{$0.654 \scriptstyle{\pm 0.048}$} & \hist{$0.0 \scriptstyle{\pm 0.0}$} & 
        \hist{$0.590 \scriptstyle{\pm 0.017}$} & \hist{$0.0 \scriptstyle{\pm 0.0}$} \\
        % -------------------------------------------------------------- %
        \hist{BeT} & 
        \hist{$0.154 \scriptstyle{\pm 0.067}$} & \hist{$0.023 \scriptstyle{\pm 0.012}$}&
        \hist{$0.676 \scriptstyle{\pm 0.035}$} & \hist{$\mathbf{0.305 \scriptstyle{\pm 0.029}}$} & 
        \hist{$0.617 \scriptstyle{\pm 0.033}$} & \hist{$\mathbf{0.380 \scriptstyle{\pm 0.019}}$} \\
        % -------------------------------------------------------------- %
        \hist{DDPM-GPT} & 
        \hist{$0.316 \scriptstyle{\pm 0.026}$} & \hist{$0.089 \scriptstyle{\pm 0.021}$} & 
        \hist{$\mathbf{0.770 \scriptstyle{\pm 0.022}}$} & \hist{$0.270 \scriptstyle{\pm 0.033}$} & 
        \hist{$0.710 \scriptstyle{\pm 0.029}$} & \hist{$0.314 \scriptstyle{\pm 0.042}$} \\ 
        % -------------------------------------------------------------- %
        \hist{BESO}  & 
        \hist{$\mathbf{0.359 \scriptstyle{\pm 0.031}}$} & \hist{$\mathbf{0.151 \scriptstyle{\pm 0.051}}$ }& 
        \hist{$0.764 \scriptstyle{\pm 0.026}$} & \hist{$0.281 \scriptstyle{\pm 0.035}$ }& 
        \hist{$\mathbf{0.719 \scriptstyle{\pm 0.025}}$} & \hist{$0.352 \scriptstyle{\pm 0.018}$} \\
        % -------------------------------------------------------------- %
        \both{DDPM-ACT} &
        \both{$0.278 \scriptstyle{\pm 0.071}$} & \both{$0.139 \scriptstyle{\pm 0.054}$} &
        \both{$0.659 \scriptstyle{\pm 0.063}$} & \both{$0.346 \scriptstyle{\pm 0.028}$} & 
        \both{$0.643 \scriptstyle{\pm 0.036}$} & \both{$0.397 \scriptstyle{\pm 0.025}$} \\
        % -------------------------------------------------------------- %
	\bottomrule
\end{tabular}

}
\vskip -0.15in
\end{table}



==> results/tables/image_stacking.tex <==
\begin{table}[hbtp]
\centering
 \caption{Image-based Policy on Stacking Task}\label{image_stack}
\resizebox{\textwidth}{!}{  

\begin{tabular}{l|cc|cc|cc}
	\toprule 
            % & \multicolumn{6}{c}{Stacking} \\
            
        % \midrule

         Methods &  S1 & Entropy & S2 & Entropy & S3 & Entropy \\

	\midrule

        BC-MLP  & 
        $0.531 \scriptstyle{\pm 0.054}$ & $0$ & 
        $0.133 \scriptstyle{\pm 0.059}$ & $0$ &
        $0$ & $0$ \\
        % -------------------------------------------------------------- %
        % BC-GMM  & 
        % 0 & 0 & 
        % 0 & 0  \\
        % -------------------------------------------------------------- %
        VAE-State & 
        $0.517 \scriptstyle{\pm 0.059}$ & $0.038 \scriptstyle{\pm 0.022}$ & 
        $0.089 \scriptstyle{\pm 0.050}$ & $0.028 \scriptstyle{\pm 0.032}$ &
        $0.001 \scriptstyle{\pm 0.001}$ & $0$\\
        % -------------------------------------------------------------- %
        BeT-MLP & 
        $0.467 \scriptstyle{\pm 0.046}$ & $0.195 \scriptstyle{\pm 0.044}$ & 
        $0.068 \scriptstyle{\pm 0.024}$ & $0.027 \scriptstyle{\pm 0.015}$ &
        $0$ & $0$\\
        % -------------------------------------------------------------- %
        IBC & 
        $0.002 \scriptstyle{\pm 0.003}$ & $0$ & 
        $0$ & $0$ &
        $0$ & $0$\\
        % -------------------------------------------------------------- %
        DDPM-MLP & 
        $0.645 \scriptstyle{\pm 0.050}$ & $0.137 \scriptstyle{\pm 0.061}$ & 
        $0.111 \scriptstyle{\pm 0.049}$ & $0.027 \scriptstyle{\pm 0.019}$ &
        $0.002 \scriptstyle{\pm 0.002}$ & $0$\\
        % -------------------------------------------------------------- %
        % \midrule

        %  history=5 $\rightarrow$ $\pi(a_t|s_{t-h+1:t})$ & S1 & Entropy & S2 & Entropy & S3 & Entropy \\

	\midrule

        BC-GPT  & 
        $0.515 \scriptstyle{\pm 0.092}$ & $0$ & 
        $0.143 \scriptstyle{\pm 0.037}$ & $0$ &
        $0.003 \scriptstyle{\pm 0.002}$ & $0$ \\
        % -------------------------------------------------------------- %
        % LSTM-GMM & 
        % 0 & 0 & 
        % 0 & 0 \\
        % -------------------------------------------------------------- %
        BeT & 
        $0.500 \scriptstyle{\pm 0.054}$ & $0.325 \scriptstyle{\pm 0.082}$ & 
        $0.143 \scriptstyle{\pm 0.031}$ & $0.057 \scriptstyle{\pm 0.022}$ & 
        $0.002 \scriptstyle{\pm 0.001}$ & $0$
         \\
        % -------------------------------------------------------------- %
        DDPM-GPT & 
        $0.704 \scriptstyle{\pm 0.024}$ & $0.349 \scriptstyle{\pm 0.053}$ & 
        $0.153 \scriptstyle{\pm 0.035}$ & $0.145 \scriptstyle{\pm 0.050}$ & 
        $0.007 \scriptstyle{\pm 0.004}$ & $0.012 \scriptstyle{\pm 0.019}$
         \\
        % -------------------------------------------------------------- %
        BESO  & 
        $0.655 \scriptstyle{\pm 0.061}$ & $0.182 \scriptstyle{\pm 0.020}$ & 
        $0.188 \scriptstyle{\pm 0.041}$ & $0.087 \scriptstyle{\pm 0.030}$ &
        $0.003 \scriptstyle{\pm 0.003}$ & $0.008 \scriptstyle{\pm 0.020}$\\

        \midrule
        VAE-ACT &
        $0.572 \scriptstyle{\pm 0.081}$ & $0.219 \scriptstyle{\pm 0.051}$ & 
        $0.196 \scriptstyle{\pm 0.057}$ & $0.115 \scriptstyle{\pm 0.037}$ & 
        $0.018 \scriptstyle{\pm 0.010}$ & $0.006 \scriptstyle{\pm 0.009}$
        \\
        \midrule
        DDPM-ACT &
        $0.752 \scriptstyle{\pm 0.045}$ & $0.334 \scriptstyle{\pm 0.073}$ & 
        $0.513 \scriptstyle{\pm 0.058}$ & $0.302 \scriptstyle{\pm 0.064}$ & 
        $0.244 \scriptstyle{\pm 0.043}$ & $0.093 \scriptstyle{\pm 0.042}$ 
        \\
	\bottomrule
\end{tabular}

}
\vskip -0.15in
\end{table}


==> results/tables/oa_bp.tex <==
\begin{table}[hbtp]
\centering
 \caption{Performance of IL methods in the Avoiding, Aligning and Pushing tasks}\label{oa_rp_bp}
 
\resizebox{\textwidth}{!}{  

\begin{tabular}{l|cc|cc|cc}
	\toprule 
            & \multicolumn{2}{c|}{Avoiding (T1)} & \multicolumn{2}{c|}{Aligning (T2)} & \multicolumn{2}{c}{Pushing (T3)} \\
            
        \midrule

         Methods & Success Rate & Entropy & Success Rate & Entropy & Success Rate & Entropy  \\

	\midrule

        BC-MLP  & 
        $0.666 \scriptstyle{\pm 0.512}$ & $0.0 \scriptstyle{\pm 0.0}$ & 
        $0.708 \scriptstyle{\pm 0.052}$ & $0.0 \scriptstyle{\pm 0.0}$ & 
        $0.522 \scriptstyle{\pm 0.165}$ & $0.0 \scriptstyle{\pm 0.0}$ 
        \\
        
        % -------------------------------------------------------------- %
        
        % BC-GMM  & 
        % $0.091 \scriptstyle{\pm 0.045}$ & $0.296 \scriptstyle{\pm 0.098}$ & 
        % 0 & 0 & 0 & 
        % 0 & 0 & 0
        % \\
        
        % -------------------------------------------------------------- %
        
        VAE-State & 
        $0.716 \scriptstyle{\pm 0.265}$ & $0.195 \scriptstyle{\pm 0.111}$ & 
        $0.579 \scriptstyle{\pm 0.138}$ & $0.030 \scriptstyle{\pm 0.053}$ & 
        $\mathbf{0.604 \scriptstyle{\pm 0.087}}$ & $0.170 \scriptstyle{\pm 0.031}$  \\

        % -------------------------------------------------------------- %
        
        BeT-MLP & 
        $0.665 \scriptstyle{\pm 0.136}$ & $0.836 \scriptstyle{\pm 0.071}$ & 
        $0.507 \scriptstyle{\pm 0.081}$ & $0.485 \scriptstyle{\pm 0.092}$ & 
        $0.420 \scriptstyle{\pm 0.049}$ & $0.628 \scriptstyle{\pm 0.123}$ \\

        % -------------------------------------------------------------- %
    
        IBC & 
        $\mathbf{0.760 \scriptstyle{\pm 0.046}}$ & $\mathbf{0.850 \scriptstyle{\pm 0.038}}$ & 
        $0.638 \scriptstyle{\pm 0.027}$ &  $0.300 \scriptstyle{\pm 0.048}$ & 
        $0.574 \scriptstyle{\pm 0.048}$ & $\mathbf{0.816 \scriptstyle{\pm 0.028}}$  \\

        % -------------------------------------------------------------- %
        
        DDPM-MLP & 
        $0.637 \scriptstyle{\pm 0.055}$ & $0.801 \scriptstyle{\pm 0.034}$ & 
        $\mathbf{0.763 \scriptstyle{\pm 0.039}}$ & $\mathbf{0.712 \scriptstyle{\pm 0.064}}$ &  
        $0.569 \scriptstyle{\pm 0.047}$ & $0.796 \scriptstyle{\pm 0.043}$  \\

        \midrule
        
        % history=5 $\rightarrow$ $\pi(a_t|s_{t-h+1:t})$ & Success Rate & Entropy & Success Rate & Distance Error & Entropy & Success Rate & Distance Error & Entropy \\

	% \midrule

        BC-GPT  & 
        $0.833 \scriptstyle{\pm 0.408}$ & $0.0 \scriptstyle{\pm 0.0}$ & 
        $0.833 \scriptstyle{\pm 0.043}$ & $0.0 \scriptstyle{\pm 0.0}$ & 
        $\mathbf{0.855 \scriptstyle{\pm 0.054}}$ & $0.0 \scriptstyle{\pm 0.0}$  \\

        % -------------------------------------------------------------- %
        
        % LSTM-GMM & 
        % 0 & 0 & 
        % 0 & 0 & 0 & 
        % 0 & 0 & 0 
        % \\

        % -------------------------------------------------------------- %
                
        BeT & 
        $0.747 \scriptstyle{\pm 0.030}$ & $0.844 \scriptstyle{\pm 0.035}$ & 
        $0.645 \scriptstyle{\pm 0.069}$ & $0.536 \scriptstyle{\pm 0.105}$ & 
        $0.724 \scriptstyle{\pm 0.051}$ & $0.788 \scriptstyle{\pm 0.031}$  \\
        % -------------------------------------------------------------- %
        
        DDPM-GPT & 
        $0.927 \scriptstyle{\pm 0.022}$ & $\mathbf{0.898 \scriptstyle{\pm 0.018}}$ & 
        $0.839 \scriptstyle{\pm 0.020}$ & $0.664 \scriptstyle{\pm 0.075}$ & 
        $0.847 \scriptstyle{\pm 0.050}$ & $0.862 \scriptstyle{\pm 0.017}$ 
        
        \\
        
        BESO & 
        $\mathbf{0.950 \scriptstyle{\pm 0.015}}$ & $0.856 \scriptstyle{\pm 0.018}$ & 
        $\mathbf{0.861 \scriptstyle{\pm 0.016}}$ & $\mathbf{0.711 \scriptstyle{\pm 0.030}}$ &
        $0.794 \scriptstyle{\pm 0.095}$ & $\mathbf{0.871 \scriptstyle{\pm 0.037}}$ 
        
        \\
        
        \midrule
        VAE-ACT  &
        $0.851 \scriptstyle{\pm 0.109}$ & $0.224 \scriptstyle{\pm 0.173}$ & 
        $\mathbf{0.891 \scriptstyle{\pm 0.022}}$ & $0.025 \scriptstyle{\pm 0.012}$ & 
        $\mathbf{0.951 \scriptstyle{\pm 0.033}}$ & $0.070 \scriptstyle{\pm 0.029}$
        \\
        
        \midrule
        DDPM-ACT  &
        $0.899 \scriptstyle{\pm 0.006}$ & $0.863 \scriptstyle{\pm 0.068}$ & 
        $0.849 \scriptstyle{\pm 0.023}$ & $\mathbf{0.749 \scriptstyle{\pm 0.041}}$ & 
        $0.920 \scriptstyle{\pm 0.027}$ & $0.859 \scriptstyle{\pm 0.012}$
        \\
	\bottomrule
\end{tabular}

}
\vskip -0.15in
\end{table}



% \begin{table}[t!]
% \centering
%  \caption{Results on Avoiding (T1) and Pushing (T3) for \st{proprioceptive} state representation.}\label{table:oa_bp}
 
% \resizebox{\textwidth}{!}{  

% \begin{tabular}{ll|ccccccccccc}
% 	\toprule 
%         %     & & \multicolumn{5}{c|}{MLP-based policy} & \multicolumn{6}{c}{Transformer-based policy} \\
            
%         % \midrule

%         Tasks & Metrics & BC-MLP & VAE-State & BeT-MLP & IBC & DDPM-MLP & BC-GPT & BeT & DDPM-GPT & BESO & VAE-ACT & DDPM-ACT  \\
% 	\midrule
%         T1 
%         & Success 
%         & \st{$0.666 \scriptstyle{\pm 0.512}$} 
%         & \st{$0.716 \scriptstyle{\pm 0.265}$} 
%         & \st{$0.665 \scriptstyle{\pm 0.136}$} 
%         & \st{${0.760 \scriptstyle{\pm 0.046}}$} 
%         & \st{$0.637 \scriptstyle{\pm 0.055}$} 
%         & \st{$0.833 \scriptstyle{\pm 0.408}$} 
%         & \st{$0.747 \scriptstyle{\pm 0.030}$} 
%         & \st{$0.927 \scriptstyle{\pm 0.022}$} 
%         & \st{$\mathbf{0.950 \scriptstyle{\pm 0.015}}$} 
%         & \st{$0.388 \scriptstyle{\pm 0.382}$} 
%         & \st{$0.899 \scriptstyle{\pm 0.006}$} 
%         \\
%         & Entropy  
%         & \st{$0.0 \scriptstyle{\pm 0.0}$ }
%         & \st{$0.195 \scriptstyle{\pm 0.111}$ }
%         & \st{$0.836 \scriptstyle{\pm 0.071}$ }
%         & \st{${0.850 \scriptstyle{\pm 0.038}}$ }
%         & \st{$0.801 \scriptstyle{\pm 0.034}$ }
%         & \st{$0.0 \scriptstyle{\pm 0.0}$ }
%         & \st{$0.844 \scriptstyle{\pm 0.035}$ }
%         & \st{$\mathbf{0.898 \scriptstyle{\pm 0.018}}$ }
%         & \st{$0.856 \scriptstyle{\pm 0.018}$ }
%         & \st{$0.126 \scriptstyle{\pm 0.146}$ }
%         & \st{$0.863 \scriptstyle{\pm 0.068}$}
%         \\
        
%         \midrule
%         T3 
%         & Success 
%         & \st{$0.522 \scriptstyle{\pm 0.165}$ }
%         & \st{${0.604 \scriptstyle{\pm 0.087}}$ }
%         & \st{$0.420 \scriptstyle{\pm 0.049}$ }
%         & \st{$0.574 \scriptstyle{\pm 0.048}$ }
%         & \st{$0.569 \scriptstyle{\pm 0.047}$ }
%         & \st{$0.855 \scriptstyle{\pm 0.054}$ }
%         & \st{$0.724 \scriptstyle{\pm 0.051}$ }
%         & \st{$0.847 \scriptstyle{\pm 0.050}$ }
%         & \st{$0.794 \scriptstyle{\pm 0.095}$ }
%         & \st{$\mathbf{0.951 \scriptstyle{\pm 0.033}}$ }
%         & \st{$0.920 \scriptstyle{\pm 0.027}$}
%         \\ 
%         & Entropy  
%         & \st{$0.0 \scriptstyle{\pm 0.0}$ }
%         & \st{$0.170 \scriptstyle{\pm 0.031}$ }
%         & \st{$0.628 \scriptstyle{\pm 0.123}$ }
%         & \st{${0.816 \scriptstyle{\pm 0.028}}$ }
%         & \st{$0.796 \scriptstyle{\pm 0.043}$ }
%         & \st{$0.0 \scriptstyle{\pm 0.0}$ }
%         & \st{$0.788 \scriptstyle{\pm 0.031}$ }
%         & \st{$0.862 \scriptstyle{\pm 0.017}$ }
%         & \st{$\mathbf{0.871 \scriptstyle{\pm 0.037}}$ }
%         & \st{$0.070 \scriptstyle{\pm 0.029}$ }
%         & \st{$0.859 \scriptstyle{\pm 0.012}$}
%         \\
% 	\bottomrule
% \end{tabular}

% }
% \vskip -0.15in
% \end{table}

==> results/tables/stack.tex <==
\begin{table}[hbtp]
\centering
 \caption{Performance of IL methods on the Stacking task with varying number of boxes}\label{table:stack}
\resizebox{\textwidth}{!}{  

\begin{tabular}{l|cc|cc|cc}
	\toprule 
            % & \multicolumn{6}{c}{Stacking} \\
            
        % \midrule

         Methods &  Stacking (1) & Entropy & Stacking (2) & Entropy & Stacking (3) & Entropy \\

	\midrule

        BC-MLP  & 
        $0.030 \scriptstyle{\pm 0.022}$ & $0.0 \scriptstyle{\pm 0.0}$ & 
        $0.0 \scriptstyle{\pm 0.0}$ & $0.0 \scriptstyle{\pm 0.0}$ &
        $0.0 \scriptstyle{\pm 0.0}$ & $0.0 \scriptstyle{\pm 0.0}$ \\
        % -------------------------------------------------------------- %
        % BC-GMM  & 
        % 0 & 0 & 
        % 0 & 0  \\
        % -------------------------------------------------------------- %
        VAE-State & 
        $0.036 \scriptstyle{\pm 0.023}$ & $0.064 \scriptstyle{\pm 0.092}$ & 
        $0.001 \scriptstyle{\pm 0.001}$ & $0.0 \scriptstyle{\pm 0.0}$ &
        $0.0 \scriptstyle{\pm 0.0}$ & $0.0 \scriptstyle{\pm 0.0}$\\
        % -------------------------------------------------------------- %
        BeT-MLP & 
        $0.102 \scriptstyle{\pm 0.059}$ & $\mathbf{0.120 \scriptstyle{\pm 0.031}}$ & 
        $0.003 \scriptstyle{\pm 0.001}$ & $0.0 \scriptstyle{\pm 0.0}$ &
        $0.0 \scriptstyle{\pm 0.0}$ & $0.0 \scriptstyle{\pm 0.0}$\\
        % -------------------------------------------------------------- %
        IBC & 
        $0.010 \scriptstyle{\pm 0.016}$ & $0.013 \scriptstyle{\pm 0.027}$ & 
        $0.0 \scriptstyle{\pm 0.0}$ & $0.0 \scriptstyle{\pm 0.0}$ &
        $0.0 \scriptstyle{\pm 0.0}$ & $0.0 \scriptstyle{\pm 0.0}$\\
        % -------------------------------------------------------------- %
        DDPM-MLP & 
        $\mathbf{0.244 \scriptstyle{\pm 0.161}}$ & $0.113 \scriptstyle{\pm 0.084}$ & 
        $\mathbf{0.042 \scriptstyle{\pm 0.045}}$ & $\mathbf{0.011 \scriptstyle{\pm 0.014}}$ &
        $\mathbf{0.001 \scriptstyle{\pm 0.0009}}$ & $\mathbf{0.096 \scriptstyle{\pm 0.193}}$\\
        % -------------------------------------------------------------- %
        % \midrule

        %  history=5 $\rightarrow$ $\pi(a_t|s_{t-h+1:t})$ & S1 & Entropy & S2 & Entropy & S3 & Entropy \\

	\midrule

        BC-GPT  & 
        $0.241 \scriptstyle{\pm 0.055}$ & $0.0 \scriptstyle{\pm 0.0}$ & 
        $0.025 \scriptstyle{\pm 0.016}$ & $0.0 \scriptstyle{\pm 0.0}$ &
        $0.0 \scriptstyle{\pm 0.0}$ & $0.0 \scriptstyle{\pm 0.0}$ \\
        % -------------------------------------------------------------- %
        % LSTM-GMM & 
        % 0 & 0 & 
        % 0 & 0 \\
        % -------------------------------------------------------------- %
        BeT & 
        $0.163 \scriptstyle{\pm 0.066}$ & $0.234 \scriptstyle{\pm 0.079}$ & 
        $0.025 \scriptstyle{\pm 0.015}$ & $0.051 \scriptstyle{\pm 0.035}$ & 
        $0.001 \scriptstyle{\pm 0.001}$ & $0.0 \scriptstyle{\pm 0.0}$
         \\
        % -------------------------------------------------------------- %
        DDPM-GPT & 
        $0.895 \scriptstyle{\pm 0.013}$ & $0.222 \scriptstyle{\pm 0.052}$ & 
        $\mathbf{0.708 \scriptstyle{\pm 0.031}}$ & $0.146 \scriptstyle{\pm 0.029}$ & 
        $\mathbf{0.120 \scriptstyle{\pm 0.018}}$ & $0.120 \scriptstyle{\pm 0.039}$
         \\
        % -------------------------------------------------------------- %
        BESO  & 
        $\mathbf{0.909 \scriptstyle{\pm 0.007}}$ & $\mathbf{0.382 \scriptstyle{\pm 0.053}}$ & 
        $0.685 \scriptstyle{\pm 0.034}$ & $\mathbf{0.177 \scriptstyle{\pm 0.058}}$ &
        $0.095 \scriptstyle{\pm 0.006}$ & $\mathbf{0.131 \scriptstyle{\pm 0.028}}$\\

        \midrule
        VAE-ACT &
        $0.308 \scriptstyle{\pm 0.096}$ & $0.095 \scriptstyle{\pm 0.027}$ & 
        $0.083 \scriptstyle{\pm 0.067}$ & $0.037 \scriptstyle{\pm 0.037}$ & 
        $0.0004$ & $0.0 \scriptstyle{\pm 0.0}$
        \\
        \midrule
        DDPM-ACT &
        $0.634 \scriptstyle{\pm 0.049}$ & $0.762 \scriptstyle{\pm 0.048}$ & 
        $0.300 \scriptstyle{\pm 0.053}$ & $0.503 \scriptstyle{\pm 0.070}$ & 
        $0.096 \scriptstyle{\pm 0.021}$ & $0.190 \scriptstyle{\pm 0.057}$ 
        \\
	\bottomrule
\end{tabular}

}
\vskip -0.15in
\end{table}


==> results/tables/vae_kl.tex <==
\begin{table}[hbtp]
\centering
 \caption{Ablation study of scaling factor for KL loss on Avoiding and Aligning}\label{vae_kl}
 
\resizebox{\textwidth}{!}{  

\begin{tabular}{lc|cc|cc}
	\toprule 
            & & \multicolumn{2}{c|}{Avoiding} & \multicolumn{2}{c}{Aligning} \\
            
        \midrule

         & Scaling for KL loss & Success Rate & Entropy & Success Rate & Entropy \\

	\midrule

        VAE-ACT & 0.01 & $0.654 \scriptstyle{\pm 0.292}$ & $0.277 \scriptstyle{\pm 0.246}$ & $0.916            \scriptstyle{\pm 0.036}$ & $0.037 \scriptstyle{\pm 0.027}$ \\
        
                 & 0.1 & $0.851 \scriptstyle{\pm 0.109}$ & $0.224 \scriptstyle{\pm 0.173}$ & $0.915 \scriptstyle{\pm 0.019}$ & $0.028 \scriptstyle{\pm 0.009}$ \\
                 
                 & 1 & $0.388 \scriptstyle{\pm 0.382}$ & $0.126 \scriptstyle{\pm 0.146}$ & $0.891 \scriptstyle{\pm 0.022}$ & $0.025 \scriptstyle{\pm 0.012}$ \\
                 
                 & 10 & $0.524 \scriptstyle{\pm 0.359}$ & $0.138 \scriptstyle{\pm 0.082}$ & 
                     $0.897 \scriptstyle{\pm 0.052}$ & $0.040 \scriptstyle{\pm 0.021}$ \\

                 & 100 & $0.309 \scriptstyle{\pm 0.406}$ & $0.124 \scriptstyle{\pm 0.142}$ & 
                     $0.902 \scriptstyle{\pm 0.042}$ & $0.039 \scriptstyle{\pm 0.023}$ \\
        
	\bottomrule
\end{tabular}

}
\vskip -0.15in
\end{table}



==> sections/acknowledgments.tex <==
\section{Acknowledgments}
Use unnumbered third level headings for the acknowledgments. All
acknowledgments, including those to funding agencies, go at the end of the paper.


==> sections/discussion.tex <==
\section{Discussion}
Based on our empirical study, we summarize our findings below.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{enumerate}
    % \item There exists a trade-off between task performance and diversity (Follows from all results)
    % \item History and Prediction horizon matter a lot for proprioceptive state representation. 
    % (Follows from State vs Image results)
    % \item Less diversity for image-based state representation (Follows from State vs Image results)
    % \item Manipulating Multiple Objects is challenging for state-based (Follows from State vs Image results)
    % \item Diffusion policies generalize well and work on low-data regimes (Follows from dataset size ablation)
    % \item Maybe something on hyperparameter sensitivity (Diffusion Policy needs more steps - maybe we can make this conclusion since Moritz uses 3 steps in his paper)

%general
    \item Transformer based methods do not suffer from mode averaging that much (in particular for more complex tasks / state representations) as it is a overparametrized model but can not capture diversity
    \item to capture diverse behavior, diffusion seems to be best suited. VAEs perform poorly, BET and IBC are soso. 
    \item other papers do not tune hyper parameters well enough in their comparisons (see IBC)
    \item GPT-based models overfit with less training data (diffusion helps)

%diffusion
    \item it depends on the transformer architecture how to choose the number of history 
    \item diffusion seems to "regularize" transformers to makes them less "data-hungry"
    \item number of diffusion steps increases diversity, successrates are only affected if too little steps are used (>4)

% representation
\item  state representations work well for precise control, but do not scale with the number of objects (invariances are not exploited)
\item image representations can deal well with many objects (size representation does not change), are harder to apply for precise control task
\item There is a need for better state representations for robotic manipulation




    
\end{enumerate}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> sections/experiments.bkp.tex <==
\section{Experimental Results}
In this section, we report experimental results with 11 imitation learning methods across 5 manipulation tasks. We conduct both state-based experiments and image-based experiments. According to the results, we present our findings and analyses for what could be influential for robot manipulation and how the current models deal with multi-modality.

\begin{table}[hbtp]
\centering
 \caption{Benchmark on Obstacle Avoidance (OA) and Block Push (BP)}\label{t_2}
 
\resizebox{\textwidth}{!}{  

\begin{tabular}{ll|ccccc|cccccc}
	\toprule 
            & & \multicolumn{5}{c|}{MLP-based policy} & \multicolumn{6}{c}{Transformer-based policy} \\
            
        \midrule

        Tasks & Metrics & MLP & CVAE & BeT-MLP & IBC & DDPM-MLP & GPT & BeT & DDPM-GPT & BESO & ACT & DiffusionPolicy  \\

	\midrule

        OA & Success & $0.666 \scriptstyle{\pm 0.512}$ & $0.716 \scriptstyle{\pm 0.265}$ & 
                        $0.665 \scriptstyle{\pm 0.136}$ & $\mathbf{0.760 \scriptstyle{\pm 0.046}}$ &
                        $0.637 \scriptstyle{\pm 0.055}$ & $0.833 \scriptstyle{\pm 0.408}$ &
                        $0.747 \scriptstyle{\pm 0.030}$ & $0.927 \scriptstyle{\pm 0.022}$ &
                        $\mathbf{0.950 \scriptstyle{\pm 0.015}}$ & $0.388 \scriptstyle{\pm 0.382}$ &
                        $0.899 \scriptstyle{\pm 0.006}$ \\
        & Entropy  &   0 & $0.195 \scriptstyle{\pm 0.111}$ &
                       $0.836 \scriptstyle{\pm 0.071}$ & $\mathbf{0.850 \scriptstyle{\pm 0.038}}$ &
                       $0.801 \scriptstyle{\pm 0.034}$ & 0 &
                       $0.844 \scriptstyle{\pm 0.035}$ & $\mathbf{0.898 \scriptstyle{\pm 0.018}}$ &
                       $0.856 \scriptstyle{\pm 0.018}$ & $0.126 \scriptstyle{\pm 0.146}$ &
                       $0.863 \scriptstyle{\pm 0.068}$
        \\
        
        \midrule
        BP & Success &  $0.522 \scriptstyle{\pm 0.165}$ & $\mathbf{0.604 \scriptstyle{\pm 0.087}}$ &
                        $0.420 \scriptstyle{\pm 0.049}$ & $0.574 \scriptstyle{\pm 0.048}$ &
                        $0.569 \scriptstyle{\pm 0.047}$ & $0.855 \scriptstyle{\pm 0.054}$ &
                        $0.724 \scriptstyle{\pm 0.051}$ & $0.847 \scriptstyle{\pm 0.050}$ &
                        $0.794 \scriptstyle{\pm 0.095}$ & $\mathbf{0.951 \scriptstyle{\pm 0.033}}$ &
                        $0.920 \scriptstyle{\pm 0.027}$\\ 
        & Entropy  &    0 & $0.170 \scriptstyle{\pm 0.031}$ &
                        $0.628 \scriptstyle{\pm 0.123}$ & $\mathbf{0.816 \scriptstyle{\pm 0.028}}$ &
                        $0.796 \scriptstyle{\pm 0.043}$ & 0 &
                        $0.788 \scriptstyle{\pm 0.031}$ & $0.862 \scriptstyle{\pm 0.017}$ &
                        $\mathbf{0.871 \scriptstyle{\pm 0.037}}$ & $0.070 \scriptstyle{\pm 0.029}$ &
                        $0.859 \scriptstyle{\pm 0.012}$

        \\
	\bottomrule
\end{tabular}

}
\vskip -0.15in
\end{table}


\begin{figure*}[hbtp]
        \centering
        \begin{minipage}[t!]{0.48\textwidth}
            \centering 
            \includegraphics[width=0.48\textwidth]{figures/block_push/gg_rr.pdf}
            \includegraphics[width=0.48\textwidth]{figures/block_push/gr_rg.pdf}
            \subcaption[]{Obstacle Avoidance}
        \end{minipage}
         \hfill
        \centering
        \begin{minipage}[t!]{0.48\textwidth}
            \centering 
            \includegraphics[width=0.48\textwidth]{figures/block_push/rr_gg.pdf}
            \includegraphics[width=0.48\textwidth]{figures/block_push/rg_gr.pdf}
            \subcaption[]{Block Push}
        \end{minipage}
         \hfill
        \caption[ ]
        {\small \textbf{Simulation Visualization} Top View of various simulated trajectories given the same context. (a) 100 simulations from CVAE and DDPM-GPT. (b) 16 simulations from CVAE and DDPM-GPT}
        \label{fig:simulation_oa_bp}
    \end{figure*}

% \begin{minipage}{\textwidth}
  
%   \begin{minipage}[b]{0.49\textwidth}
%     \centering
%     \resizebox{0.8\textwidth}{!}{ 
%         \begin{tabular}{l|cc|cc}
% 	\toprule 
%             & \multicolumn{2}{c|}{Obstacle Avoidance} & \multicolumn{2}{c}{Block Push (4 modes)} \\
            
%         \midrule

%          history=1 & Success Rate & Entropy & Success Rate & Entropy  \\

% 	\midrule

%         MLP  & 
%         $0.666 \scriptstyle{\pm 0.512}$ & 0 & 
%         $0.522 \scriptstyle{\pm 0.165}$ & $0$ 
%         \\
        
%         % -------------------------------------------------------------- %
        
%         % BC-GMM  & 
%         % $0.091 \scriptstyle{\pm 0.045}$ & $0.296 \scriptstyle{\pm 0.098}$ & 
%         % 0 & 0 & 0 & 
%         % 0 & 0 & 0
%         % \\
        
%         % -------------------------------------------------------------- %
        
%         CVAE & 
%         $0.716 \scriptstyle{\pm 0.265}$ & $0.195 \scriptstyle{\pm 0.111}$ &  
%         $\mathbf{0.604 \scriptstyle{\pm 0.087}}$ & $0.170 \scriptstyle{\pm 0.031}$  \\

%         % -------------------------------------------------------------- %
        
%         BeT-MLP & 
%         $0.665 \scriptstyle{\pm 0.136}$ & $0.836 \scriptstyle{\pm 0.071}$ & 
%         $0.420 \scriptstyle{\pm 0.049}$ & $0.628 \scriptstyle{\pm 0.123}$ \\

%         % -------------------------------------------------------------- %
        
%         IBC & 
%         $\mathbf{0.760 \scriptstyle{\pm 0.046}}$ & $\mathbf{0.850 \scriptstyle{\pm 0.038}}$ & 
%         $0.574 \scriptstyle{\pm 0.048}$ & $\mathbf{0.816 \scriptstyle{\pm 0.028}}$  \\

%         % -------------------------------------------------------------- %
        
%         DDPM-MLP & 
%         $0.637 \scriptstyle{\pm 0.055}$ & $0.801 \scriptstyle{\pm 0.034}$ & 
%         $0.569 \scriptstyle{\pm 0.047}$ & $0.796 \scriptstyle{\pm 0.043}$  \\

%         \midrule
        
%         history=5 & Success Rate & Entropy & Success Rate & Entropy \\

% 	\midrule

%         GPT  & 
%         $0.833 \scriptstyle{\pm 0.408}$ & $0$ & 
%         $0.855 \scriptstyle{\pm 0.054}$ & $0$  \\
  
%         BeT & 
%         $0.747 \scriptstyle{\pm 0.030}$ & $0.844 \scriptstyle{\pm 0.035}$ &  
%         $0.724 \scriptstyle{\pm 0.051}$ & $0.788 \scriptstyle{\pm 0.031}$  \\
%         % -------------------------------------------------------------- %
        
%         DDPM-GPT & 
%         $0.927 \scriptstyle{\pm 0.022}$ & $\mathbf{0.898 \scriptstyle{\pm 0.018}}$ & 
%         $0.847 \scriptstyle{\pm 0.050}$ & $0.862 \scriptstyle{\pm 0.017}$ 
        
%         \\
        
%         BESO & 
%         $\mathbf{0.950 \scriptstyle{\pm 0.015}}$ & $0.856 \scriptstyle{\pm 0.018}$ & 
%         $0.794 \scriptstyle{\pm 0.095}$ & $\mathbf{0.871 \scriptstyle{\pm 0.037}}$ 
        
%         \\
        
%         \midrule
%         ACT &
%         $0.388 \scriptstyle{\pm 0.382}$ & $0.126 \scriptstyle{\pm 0.146}$ & 
%         $\mathbf{0.951 \scriptstyle{\pm 0.033}}$ & $0.070 \scriptstyle{\pm 0.029}$
%         \\
        
%         \midrule
%         DiffusionPolicy &
%         $0.899 \scriptstyle{\pm 0.006}$ & $0.863 \scriptstyle{\pm 0.068}$ & 
%         $0.920 \scriptstyle{\pm 0.027}$ & $0.859 \scriptstyle{\pm 0.012}$
%         \\
% 	\bottomrule
%         \end{tabular}
%     }
%       \captionof{table}{Benchmark on Obstacle Avoidance and Block Push}
      
%     \end{minipage}

% \hfill
    
% \begin{minipage}[b]{0.49\textwidth}
%     \centering
%     \includegraphics[]{figures/obstacle_avoidance/Fig:ICML23:obsavoid_success.pdf}
%     \captionof{figure}{A table beside a figure}
%   \end{minipage}
  
    
% \end{minipage}

% \begin{table}[hbtp]
% \centering
%  \caption{2d robot manipulation tasks benchmark with state policy}\label{t_2}
 
% \resizebox{0.5\textwidth}{!}{  

% \begin{tabular}{l|cc|cc}
% 	\toprule 
%             & \multicolumn{2}{c|}{Obstacle Avoidance} & \multicolumn{2}{c}{Block Push (4 modes)} \\
            
%         \midrule

%          history=1 & Success Rate & Entropy & Success Rate & Entropy  \\

% 	\midrule

%         MLP  & 
%         $0.666 \scriptstyle{\pm 0.512}$ & 0 & 
%         % $0.708 \scriptstyle{\pm 0.052}$ & $0.094 \scriptstyle{\pm 0.024}$ & $0$ & 
%         $0.522 \scriptstyle{\pm 0.165}$ & $0$ 
%         \\
        
%         % -------------------------------------------------------------- %
        
%         % BC-GMM  & 
%         % $0.091 \scriptstyle{\pm 0.045}$ & $0.296 \scriptstyle{\pm 0.098}$ & 
%         % 0 & 0 & 0 & 
%         % 0 & 0 & 0
%         % \\
        
%         % -------------------------------------------------------------- %
        
%         CVAE & 
%         $0.716 \scriptstyle{\pm 0.265}$ & $0.195 \scriptstyle{\pm 0.111}$ & 
%         % $0.579 \scriptstyle{\pm 0.138}$ & $0.122 \scriptstyle{\pm 0.040}$ & $0.030 \scriptstyle{\pm 0.053}$ & 
%         $\mathbf{0.604 \scriptstyle{\pm 0.087}}$ & $0.170 \scriptstyle{\pm 0.031}$  \\

%         % -------------------------------------------------------------- %
        
%         BeT-MLP & 
%         $0.665 \scriptstyle{\pm 0.136}$ & $0.836 \scriptstyle{\pm 0.071}$ & 
%         % $0.507 \scriptstyle{\pm 0.081}$ & $0.143 \scriptstyle{\pm 0.030}$ & $0.485 \scriptstyle{\pm 0.092}$ & 
%         $0.420 \scriptstyle{\pm 0.049}$ & $0.628 \scriptstyle{\pm 0.123}$ \\

%         % -------------------------------------------------------------- %
        
%         IBC & 
%         $\mathbf{0.760 \scriptstyle{\pm 0.046}}$ & $\mathbf{0.850 \scriptstyle{\pm 0.038}}$ & 
%         % $0.638 \scriptstyle{\pm 0.027}$ & $0.107 \scriptstyle{\pm 0.011}$ & $0.300 \scriptstyle{\pm 0.048}$ & 
%         $0.574 \scriptstyle{\pm 0.048}$ & $\mathbf{0.816 \scriptstyle{\pm 0.028}}$  \\

%         % -------------------------------------------------------------- %
        
%         DDPM-MLP & 
%         $0.637 \scriptstyle{\pm 0.055}$ & $0.801 \scriptstyle{\pm 0.034}$ & 
%         % $\mathbf{0.763 \scriptstyle{\pm 0.039}}$ & $\mathbf{0.082 \scriptstyle{\pm 0.017}}$ & $\mathbf{0.712 \scriptstyle{\pm 0.064}}$ &  
%         $0.569 \scriptstyle{\pm 0.047}$ & $0.796 \scriptstyle{\pm 0.043}$  \\

%         \midrule
        
%         history=5 & Success Rate & Entropy & Success Rate & Entropy \\

% 	\midrule

%         GPT  & 
%         $0.833 \scriptstyle{\pm 0.408}$ & $0$ & 
%         % $0.833 \scriptstyle{\pm 0.043}$ & $0.070 \scriptstyle{\pm 0.037}$ & $0$ & 
%         $0.855 \scriptstyle{\pm 0.054}$ & $0$  \\

%         % -------------------------------------------------------------- %
        
%         % LSTM-GMM & 
%         % 0 & 0 & 
%         % 0 & 0 & 0 & 
%         % 0 & 0 & 0 
%         % \\

%         % -------------------------------------------------------------- %
                
%         BeT & 
%         $0.747 \scriptstyle{\pm 0.030}$ & $0.844 \scriptstyle{\pm 0.035}$ & 
%         % $0.645 \scriptstyle{\pm 0.069}$ & $0.115 \scriptstyle{\pm 0.009}$ & $0.536 \scriptstyle{\pm 0.105}$ & 
%         $0.724 \scriptstyle{\pm 0.051}$ & $0.788 \scriptstyle{\pm 0.031}$  \\
%         % -------------------------------------------------------------- %
        
%         DDPM-GPT & 
%         $0.927 \scriptstyle{\pm 0.022}$ & $\mathbf{0.898 \scriptstyle{\pm 0.018}}$ & 
%         % $0.839 \scriptstyle{\pm 0.020}$ & $0.062 \scriptstyle{\pm 0.009}$ & $0.664 \scriptstyle{\pm 0.075}$ & 
%         $0.847 \scriptstyle{\pm 0.050}$ & $0.862 \scriptstyle{\pm 0.017}$ 
        
%         \\
        
%         BESO & 
%         $\mathbf{0.950 \scriptstyle{\pm 0.015}}$ & $0.856 \scriptstyle{\pm 0.018}$ & 
%         % $0.861 \scriptstyle{\pm 0.016}$ & $0.053 \scriptstyle{\pm 0.004}$ & $0.711 \scriptstyle{\pm 0.030}$ &
%         $0.794 \scriptstyle{\pm 0.095}$ & $\mathbf{0.871 \scriptstyle{\pm 0.037}}$ 
        
%         \\
        
%         \midrule
%         ACT &
%         $0.388 \scriptstyle{\pm 0.382}$ & $0.126 \scriptstyle{\pm 0.146}$ & 
%         % $\mathbf{0.891 \scriptstyle{\pm 0.022}}$ & $\mathbf{0.048 \scriptstyle{\pm 0.014}}$ & $0.025 \scriptstyle{\pm 0.012}$ & 
%         $\mathbf{0.951 \scriptstyle{\pm 0.033}}$ & $0.070 \scriptstyle{\pm 0.029}$
%         \\
        
%         \midrule
%         DiffusionPolicy &
%         $0.899 \scriptstyle{\pm 0.006}$ & $0.863 \scriptstyle{\pm 0.068}$ & 
%         % $0.849 \scriptstyle{\pm 0.023}$ & $0.056 \scriptstyle{\pm 0.009}$ & $\mathbf{0.749 \scriptstyle{\pm 0.041}}$ & 
%         $0.920 \scriptstyle{\pm 0.027}$ & $0.859 \scriptstyle{\pm 0.012}$
%         \\
% 	\bottomrule
% \end{tabular}

% }
% \vskip -0.15in
% \end{table}


% \begin{table}[hbtp]
% \centering
%  \caption{2d robot manipulation tasks benchmark with state policy}\label{t_2}
 
% \resizebox{\textwidth}{!}{  

% \begin{tabular}{l|cc|ccc|ccc}
% 	\toprule 
%             & \multicolumn{2}{c|}{Obstacle Avoidance} & \multicolumn{3}{c|}{Robot Push (2 modes)} & \multicolumn{3}{c}{Block Push (4 modes)} \\
            
%         \midrule

%          history=1 $\rightarrow$ $\pi(a_t|s_t)$ & Success Rate & Entropy & Success Rate & Distance Error & Entropy & Success Rate & Distance Error & Entropy  \\

% 	\midrule

%         MLP  & 
%         $0.666 \scriptstyle{\pm 0.512}$ & 0 & 
%         $0.708 \scriptstyle{\pm 0.052}$ & $0.094 \scriptstyle{\pm 0.024}$ & $0$ & 
%         $0.522 \scriptstyle{\pm 0.165}$ & $0.130 \scriptstyle{\pm 0.043} $ & $0$ 
%         \\
        
%         % -------------------------------------------------------------- %
        
%         % BC-GMM  & 
%         % $0.091 \scriptstyle{\pm 0.045}$ & $0.296 \scriptstyle{\pm 0.098}$ & 
%         % 0 & 0 & 0 & 
%         % 0 & 0 & 0
%         % \\
        
%         % -------------------------------------------------------------- %
        
%         CVAE & 
%         $0.716 \scriptstyle{\pm 0.265}$ & $0.195 \scriptstyle{\pm 0.111}$ & 
%         $0.579 \scriptstyle{\pm 0.138}$ & $0.122 \scriptstyle{\pm 0.040}$ & $0.030 \scriptstyle{\pm 0.053}$ & 
%         $\mathbf{0.604 \scriptstyle{\pm 0.087}}$ & $0.108 \scriptstyle{\pm 0.025}$ & $0.170 \scriptstyle{\pm 0.031}$  \\

%         % -------------------------------------------------------------- %
        
%         BeT-MLP & 
%         $0.665 \scriptstyle{\pm 0.136}$ & $0.836 \scriptstyle{\pm 0.071}$ & 
%         $0.507 \scriptstyle{\pm 0.081}$ & $0.143 \scriptstyle{\pm 0.030}$ & $0.485 \scriptstyle{\pm 0.092}$ & 
%         $0.420 \scriptstyle{\pm 0.049}$ & $0.143 \scriptstyle{\pm 0.010}$ & $0.628 \scriptstyle{\pm 0.123}$ \\

%         % -------------------------------------------------------------- %
        
%         IBC & 
%         $\mathbf{0.760 \scriptstyle{\pm 0.046}}$ & $\mathbf{0.850 \scriptstyle{\pm 0.038}}$ & 
%         $0.638 \scriptstyle{\pm 0.027}$ & $0.107 \scriptstyle{\pm 0.011}$ & $0.300 \scriptstyle{\pm 0.048}$ & 
%         $0.574 \scriptstyle{\pm 0.048}$ & $\mathbf{0.107 \scriptstyle{\pm 0.015}}$ & $\mathbf{0.816 \scriptstyle{\pm 0.028}}$  \\

%         % -------------------------------------------------------------- %
        
%         DDPM-MLP & 
%         $0.637 \scriptstyle{\pm 0.055}$ & $0.801 \scriptstyle{\pm 0.034}$ & 
%         $\mathbf{0.763 \scriptstyle{\pm 0.039}}$ & $\mathbf{0.082 \scriptstyle{\pm 0.017}}$ & $\mathbf{0.712 \scriptstyle{\pm 0.064}}$ &  
%         $0.569 \scriptstyle{\pm 0.047}$ & $0.111 \scriptstyle{\pm 0.012}$ & $0.796 \scriptstyle{\pm 0.043}$  \\

%         \midrule
        
%         history=5 $\rightarrow$ $\pi(a_t|s_{t-h+1:t})$ & Success Rate & Entropy & Success Rate & Distance Error & Entropy & Success Rate & Distance Error & Entropy \\

% 	\midrule

%         GPT  & 
%         $0.833 \scriptstyle{\pm 0.408}$ & $0$ & 
%         $0.833 \scriptstyle{\pm 0.043}$ & $0.070 \scriptstyle{\pm 0.037}$ & $0$ & 
%         $0.855 \scriptstyle{\pm 0.054}$ & $0.063 \scriptstyle{\pm 0.014}$ & $0$  \\

%         % -------------------------------------------------------------- %
        
%         % LSTM-GMM & 
%         % 0 & 0 & 
%         % 0 & 0 & 0 & 
%         % 0 & 0 & 0 
%         % \\

%         % -------------------------------------------------------------- %
                
%         BeT & 
%         $0.747 \scriptstyle{\pm 0.030}$ & $0.844 \scriptstyle{\pm 0.035}$ & 
%         $0.645 \scriptstyle{\pm 0.069}$ & $0.115 \scriptstyle{\pm 0.009}$ & $0.536 \scriptstyle{\pm 0.105}$ & 
%         $0.724 \scriptstyle{\pm 0.051}$ & $0.079 \scriptstyle{\pm 0.009}$ & $0.788 \scriptstyle{\pm 0.031}$  \\
%         % -------------------------------------------------------------- %
        
%         DDPM-GPT & 
%         $0.927 \scriptstyle{\pm 0.022}$ & $\mathbf{0.898 \scriptstyle{\pm 0.018}}$ & 
%         $0.839 \scriptstyle{\pm 0.020}$ & $0.062 \scriptstyle{\pm 0.009}$ & $0.664 \scriptstyle{\pm 0.075}$ & 
%         $0.847 \scriptstyle{\pm 0.050}$ & $0.056\scriptstyle{\pm 0.012}$ & $0.862 \scriptstyle{\pm 0.017}$ 
        
%         \\
        
%         BESO & 
%         $\mathbf{0.950 \scriptstyle{\pm 0.015}}$ & $0.856 \scriptstyle{\pm 0.018}$ & 
%         $0.861 \scriptstyle{\pm 0.016}$ & $0.053 \scriptstyle{\pm 0.004}$ & $0.711 \scriptstyle{\pm 0.030}$ &
%         $0.794 \scriptstyle{\pm 0.095}$ & $0.060 \scriptstyle{\pm 0.015}$ & $\mathbf{0.871 \scriptstyle{\pm 0.037}}$ 
        
%         \\
        
%         \midrule
%         ACT $\rightarrow$ $\pi(a_{t:t+k}|s_t)$ &
%         $0.388 \scriptstyle{\pm 0.382}$ & $0.126 \scriptstyle{\pm 0.146}$ & 
%         $\mathbf{0.891 \scriptstyle{\pm 0.022}}$ & $\mathbf{0.048 \scriptstyle{\pm 0.014}}$ & $0.025 \scriptstyle{\pm 0.012}$ & 
%         $\mathbf{0.951 \scriptstyle{\pm 0.033}}$ & $\mathbf{0.041 \scriptstyle{\pm 0.009}}$ & $0.070 \scriptstyle{\pm 0.029}$
%         \\
        
%         \midrule
%         DiffusionPolicy $\rightarrow$ $\pi(a_{t:t+k}|s_{t-h+1:t})$ &
%         $0.899 \scriptstyle{\pm 0.006}$ & $0.863 \scriptstyle{\pm 0.068}$ & 
%         $0.849 \scriptstyle{\pm 0.023}$ & $0.056 \scriptstyle{\pm 0.009}$ & $\mathbf{0.749 \scriptstyle{\pm 0.041}}$ & 
%         $0.920 \scriptstyle{\pm 0.027}$ & $0.043 \scriptstyle{\pm 0.006}$ & $0.859 \scriptstyle{\pm 0.012}$
%         \\
% 	\bottomrule
% \end{tabular}

% }
% \vskip -0.15in
% \end{table}

\subsection{State-based policy comparison}
We first evaluate all methods on the Obstacle Avoidance, which is designed to test the model's ability to learn multi-modal distributions. In this task, we only have training dataset and all models are trained for 2000 epochs and simulated using the last checkpoint with 6 seeds. For other tasks, we split the demonstrations into training data (90\%) and validation data (10\%). We report the simulation results using the model with best loss on validation data. Notice that we use the same loss during training and evaluation in order to match each model's objective. We mainly use success rate and mode entropy as metrics for most tasks, except for Box Alignment and Block Push, which are additionally evaluated by distance error (the detailed definition can be found in Appendix \ref{Tasks details}). The results are reported in Table \ref{t_2}, \ref{sorting_table} and \ref{cs_table}. We present our key findings below.

\textbf{Multiple ways to deal with multi-modality}. Since deterministic models including MLP and GPT can only generate one solution give a context, they are not able to learn diverse behaviors. VAE based models including CVAE and ACT can generate different behaviors, but the mode entropy is quite low which means it only covers a small part of distributions. The IBC, BeT and diffusion based models are all able to learn multi-modal distributions.

\textbf{The trade-off between success rate and entropy}. We find that there is a trade-off between success rate and entropy. For most tasks, it is hard to find one method that is best on both success rate and entropy. Increasing the entropy or diversity to some extent will degrade the success rate. The MLP and GPT has $0$ entropy, but their success rate is quite high across all methods, better than other BeT and some diffusion methods. The ACT shows best success rate on almost all tasks, but it's entropy is very low.

\textbf{History and action chunking matter a lot}. From the experiments, the models with historical inputs or action sequence generally perform much better than step-based models.

\textbf{Diffusion based models generalize very well}. 

\textbf{Manipulating multiple objects is challenging for state-based policy}. In this task, we simply stack the features of robots and boxes, which could be problematic when there are dozens of objects. The observation space becomes rather complex when increasing the number of boxes. From the experiments, we observe a severe performance drop when sorting 4 and 6 boxes. 


\begin{table}[hbtp]
\centering
 \caption{Benchmark on Box Alignment and Sorting tasks}\label{sorting_table}
\resizebox{\textwidth}{!}{  

\begin{tabular}{l|cc|cc|cc}
	\toprule 
            & \multicolumn{2}{c|}{Box Alignment} & \multicolumn{2}{c|}{Sorting 4 boxes} & \multicolumn{2}{c}{Sorting 6 boxes} \\
            
        % \midrule

          & Success Rate & Entropy & Success Rate & Entropy & Success Rate & Entropy \\

	\midrule

        MLP  & 
        $0.708 \scriptstyle{\pm 0.052}$ / $0.148 \scriptstyle{\pm 0.045}$ & $0$ / $0$ & 
        $0.058 \scriptstyle{\pm 0.048}$ / $0.666 \scriptstyle{\pm 0.080}$ & $0$ / $0$ & 
        $0.016 \scriptstyle{\pm 0.014}$ / $0.636 \scriptstyle{\pm 0.026}$ & $0$ / $0$ \\
        % -------------------------------------------------------------- %
        % BC-GMM  & 
        % 0 & 0 & 
        % 0 & 0 & 
        % 0 & 0 \\
        % -------------------------------------------------------------- %
        CVAE & 
        $0.579 \scriptstyle{\pm 0.138}$ / $0.121 \scriptstyle{\pm 0.035}$  & $0.030 \scriptstyle{\pm 0.053}$ / $0.013 \scriptstyle{\pm 0.019}$  & 
        $0.079 \scriptstyle{\pm 0.042}$ / $0.653 \scriptstyle{\pm 0.061}$ & $0.090 \scriptstyle{\pm 0.032}$ / $0.165 \scriptstyle{\pm 0.010}$ & 
        $0.030 \scriptstyle{\pm 0.016}$ / $0.570 \scriptstyle{\pm 0.023}$ & $0.086 \scriptstyle{\pm 0.017}$ / $0.236 \scriptstyle{\pm 0.013}$\\
        % -------------------------------------------------------------- %
        BeT-MLP & 
        $0.507 \scriptstyle{\pm 0.081}$ / $0.203 \scriptstyle{\pm 0.035}$ & $0.485 \scriptstyle{\pm 0.092}$ / $0.053 \scriptstyle{\pm 0.028}$ & 
        $0.003 \scriptstyle{\pm 0.001}$ / $0.671 \scriptstyle{\pm 0.014}$& $0.021 \scriptstyle{\pm 0.052}$ / $0.296 \scriptstyle{\pm 0.033}$& 
        $0$ / $0.616 \scriptstyle{\pm 0.035}$& $0$ / $0.365 \scriptstyle{\pm 0.022}$\\
        % -------------------------------------------------------------- %
        IBC & 
        $0.638 \scriptstyle{\pm 0.027}$  / $0.179 \scriptstyle{\pm 0.028}$ & $0.300 \scriptstyle{\pm 0.048}$ / $0.071 \scriptstyle{\pm 0.052}$ & 
        $0.080 \scriptstyle{\pm 0.016}$ / $0.707 \scriptstyle{\pm 0.031}$& $0.097 \scriptstyle{\pm 0.026}$ / $0.236 \scriptstyle{\pm 0.027}$& 
        $0.007 \scriptstyle{\pm 0.005}$ / $0.664 \scriptstyle{\pm 0.039}$& $0.024 \scriptstyle{\pm 0.028}$ / $0.328 \scriptstyle{\pm 0.026}$\\
        % -------------------------------------------------------------- %
        DDPM-MLP & 
        $\mathbf{0.763 \scriptstyle{\pm 0.039}}$ / $0.233 \scriptstyle{\pm 0.029}$ & $\mathbf{0.712 \scriptstyle{\pm 0.064}}$ / $0.060 \scriptstyle{\pm 0.033}$& 
        $0.032 \scriptstyle{\pm 0.009}$ / $0.763 \scriptstyle{\pm 0.028}$& $0.071 \scriptstyle{\pm 0.025}$ / $0.237 \scriptstyle{\pm 0.028}$& 
        $0$ / $0.748 \scriptstyle{\pm 0.026}$ & $0$ / $0.359 \scriptstyle{\pm 0.025}$\\
        % -------------------------------------------------------------- %
        % \midrulet
 %          & Success & Entropy & Success & Entropy & Success & Entropy \\
	% \midrule

        GPT  & 
        $0.833 \scriptstyle{\pm 0.043}$ / $0.084 \scriptstyle{\pm 0.015}$ & $0$ / $0$& 
        $0.075 \scriptstyle{\pm 0.063}$ / $0.654 \scriptstyle{\pm 0.048}$ & $0$ / $0$& 
        $0.011 \scriptstyle{\pm 0.008}$ / $0.590 \scriptstyle{\pm 0.017}$ & $0$ / $0$\\
        % -------------------------------------------------------------- %
        % LSTM-GMM & 
        % 0 & 0 & 
        % 0 & 0 & 
        % 0 & 0\\
        % -------------------------------------------------------------- %
        BeT & 
        $0.645 \scriptstyle{\pm 0.069}$ / $0.154 \scriptstyle{\pm 0.067}$ & $0.536 \scriptstyle{\pm 0.105}$ / $0.023 \scriptstyle{\pm 0.012}$& 
        $0.018 \scriptstyle{\pm 0.010}$ / $0.676 \scriptstyle{\pm 0.035}$ & $0.059 \scriptstyle{\pm 0.035}$ / $0.305 \scriptstyle{\pm 0.029}$& 
        $0$ / $0.617 \scriptstyle{\pm 0.033}$ & $0$ / $0.380 \scriptstyle{\pm 0.019}$\\
        % -------------------------------------------------------------- %
        DDPM-GPT & 
        $0.839 \scriptstyle{\pm 0.020}$ / $0.316 \scriptstyle{\pm 0.026}$ & $0.664 \scriptstyle{\pm 0.075}$ / $0.089 \scriptstyle{\pm 0.021}$& 
        $0.337 \scriptstyle{\pm 0.084}$ / $0.770 \scriptstyle{\pm 0.022}$ & $\mathbf{0.372 \scriptstyle{\pm 0.068}}$ / $0.270 \scriptstyle{\pm 0.033}$ & 
        $0.008 \scriptstyle{\pm 0.006}$ / $0.710 \scriptstyle{\pm 0.029}$ & $0.031 \scriptstyle{\pm 0.028}$ / $0.314 \scriptstyle{\pm 0.042}$\\
        % -------------------------------------------------------------- %
        BESO  & 
        $0.861 \scriptstyle{\pm 0.016}$ & $0.711 \scriptstyle{\pm 0.030}$ & 
        $0.188 \scriptstyle{\pm 0.042}$ & $0.232 \scriptstyle{\pm 0.040}$ & 
        $0$ & $0$ \\

        % \midrule
        ACT &
        $\mathbf{0.891 \scriptstyle{\pm 0.022}}$ / $0.166 \scriptstyle{\pm 0.017}$ & $0.025 \scriptstyle{\pm 0.012}$ / $0.021 \scriptstyle{\pm 0.011}$ & 
        $\mathbf{0.565 \scriptstyle{\pm 0.108}}$ / $0.717 \scriptstyle{\pm 0.038}$ & $0.114 \scriptstyle{\pm 0.020}$ / $0.217 \scriptstyle{\pm 0.024}$& 
        $0.033 \scriptstyle{\pm 0.022}$ / $0.604 \scriptstyle{\pm 0.017}$ & $0.062 \scriptstyle{\pm 0.024}$ / $0.276 \scriptstyle{\pm 0.007}$
        \\
        % \midrule
        DiffusionPolicy &
        $0.849 \scriptstyle{\pm 0.023}$ & $\mathbf{0.749 \scriptstyle{\pm 0.041}}$ & 
        $0.300 \scriptstyle{\pm 0.060}$ & $0.300 \scriptstyle{\pm 0.051}$ & 
        $0.001 \scriptstyle{\pm 0}$ & $0$ 
        \\
	\bottomrule
\end{tabular}

}

\vskip -0.15in
\end{table}



\subsection{Image-based policy comparison}
Except for state-based results, we also implemented image-based policies for each manipulation task. For fair comparison, all the methods share the same image encoder ResNet-18. The results are reported in Table \ref{image_table}. Here we mainly report the results on sorting task and cubestacking task, since these two tasks are quite hard for state-based policy. It is very interesting to find that image-based policy actually performs much better than state-based policy on these two tasks. 

\textbf{Image-based policy can perform better than state-based policy on multi-objects tasks}

\textbf{Sequential information does not improve performance for image-based policy}

\textbf{It is hard for image-based policy to capture multi-modal distribution}


\begin{figure*}[htbp]
        \centering
        % \subfigure[Obstacle Avoidance]{
            \begin{minipage}[t!]{0.48\textwidth}
                \centering 
                \includegraphics[width=0.48\textwidth]{figures/diffusionpolicy_ablation/Success Rate.pdf}
                \includegraphics[width=0.48\textwidth]{figures/diffusionpolicy_ablation/Entropy.pdf}

                \subcaption[]{Diffusion Policy Ablation}
            \end{minipage}
        % }
        \hfill
        % \subfigure[Obstacle Avoidance]{
            \begin{minipage}[t!]{0.48\textwidth}
                \centering 
                \includegraphics[width=0.48\textwidth]{figures/diffusionpolicy_ablation/ddpm_Success Rate.pdf}
                \includegraphics[width=0.48\textwidth]{figures/diffusionpolicy_ablation/ddpm_Entropy.pdf}

                \subcaption[]{GPT-based policy Ablation}
            \end{minipage}
        \caption[ ]
        {\small \textbf{Environments.} We created 5 tasks in this paper, including one toy task Obstacle Avoidance and 4 robot manipulation tasks. For each task, we collected a large amount of human demonstrations with diverse behaviors. }
        \label{fig:environments}
\end{figure*}

\subsection{Ablation study on historical input and action sequence}
From the above results, both historical inputs and action sequence help a lot with state-based policies. In order to explore more about how these two factors influence the model's performance, we conduct an ablation study using DiffusionPolicy.



\begin{figure*}[htbp]
        \centering
        % \subfigure[Obstacle Avoidance]{
            \begin{minipage}[t!]{0.48\textwidth}
                \centering 
                \includegraphics[width=0.48\textwidth]{figures/obstacle_avoidance/oa_beso_ablation.pdf}
                \includegraphics[width=0.48\textwidth]{figures/obstacle_avoidance/oa_bet_ablation.pdf}

                \subcaption[]{Diffusion Policy Ablation}
            \end{minipage}
        % }
        % \hfill
        % % \subfigure[Obstacle Avoidance]{
        %     \begin{minipage}[t!]{0.48\textwidth}
        %         \centering 
        %         \includegraphics[width=0.48\textwidth]{figures/diffusionpolicy_ablation/ddpm_Success Rate.pdf}
        %         \includegraphics[width=0.48\textwidth]{figures/diffusionpolicy_ablation/ddpm_Entropy.pdf}

        %         \subcaption[]{GPT-based policy Ablation}
        %     \end{minipage}
        \caption[ ]
        {\small \textbf{Environments.} We created 5 tasks in this paper, including one toy task Obstacle Avoidance and 4 robot manipulation tasks. For each task, we collected a large amount of human demonstrations with diverse behaviors. }
        \label{fig:environments}
\end{figure*}

\subsection{How can model learn better multi-modality}


\subsection{Ablation Study on Dataset Size}
Recording demonstrations is very tedious for imitation learning. In order to study how many demonstrations could be enough to train a well-performed policy, we generate three subsets which contain 25\%, 50\% and 75\% demonstrations of the whole dataset for the block push and box alignment tasks. Here we only compare the methods with historical inputs since they perform much better than MLP-based methods. The results are presented in table 5. 

\subsection{Policy Selection}
Model selection is a challenging problem for imitation learning. Choosing model either with best loss on evaluation data or with last checkpoint could cause significantly performance drop \cite{mandlekar2021matters}. Previous works would report the best simulation results during training, while this would require more training time and is not suitable for real world. In this paper, we conduct an ablation study on different model selection methods.

\subsection{Inference time comparison}
....
% \subsection{Ablation Study on different size of model}
% All the methods share the same size of MLP or transformer in our main experiments for fair comparison. However, for some tasks with large dataset such as sorting 4/6 boxes and cubestacking, the model could underfit the data. We provide an ablation study to test the influence of different network's size.


\begin{table}[hbtp]
\centering
 \caption{CubeStacking task benchmark}\label{cs_table}
\resizebox{\textwidth}{!}{  

\begin{tabular}{l|cc|cc|cc}
	\toprule 
            & \multicolumn{4}{c}{CubeStacking} \\
            
        \midrule

         history=1 $\rightarrow$ $\pi(a_t|s_t)$ &  S1 & Entropy & S2 & Entropy & S3 & Entropy \\

	\midrule

        MLP  & 
        $0.030 \scriptstyle{\pm 0.022}$ & $0$ & 
        0 & 0 &
        0 & 0 \\
        % -------------------------------------------------------------- %
        % BC-GMM  & 
        % 0 & 0 & 
        % 0 & 0  \\
        % -------------------------------------------------------------- %
        CVAE & 
        $0.036 \scriptstyle{\pm 0.023}$ & $0.064 \scriptstyle{\pm 0.092}$ & 
        $0.001 \scriptstyle{\pm 0.001}$ & $0$ &
        $0$ & $0$\\
        % -------------------------------------------------------------- %
        BeT-MLP & 
        $0.102 \scriptstyle{\pm 0.059}$ & $0.120 \scriptstyle{\pm 0.031}$ & 
        $0.003 \scriptstyle{\pm 0.001}$ & $0$ &
        $0$ & $0$\\
        % -------------------------------------------------------------- %
        IBC & 
        $0.010 \scriptstyle{\pm 0.016}$ & $0.013 \scriptstyle{\pm 0.027}$ & 
        $0$ & $0$ &
        $0$ & $0$\\
        % -------------------------------------------------------------- %
        DDPM-mlp & 
        $0.244 \scriptstyle{\pm 0.161}$ & $0.113 \scriptstyle{\pm 0.084}$ & 
        $0.042 \scriptstyle{\pm 0.045}$ & $0.011 \scriptstyle{\pm 0.014}$ &
        $0.001 \scriptstyle{\pm 0.0009}$ & $0.096 \scriptstyle{\pm 0.193}$\\
        % -------------------------------------------------------------- %
        \midrule

         history=5 $\rightarrow$ $\pi(a_t|s_{t-h+1:t})$ & S1 & Entropy & S2 & Entropy & S3 & Entropy \\

	\midrule

        GPT  & 
        $0.241 \scriptstyle{\pm 0.055}$ & $0$ & 
        $0.025 \scriptstyle{\pm 0.016}$ & $0$ &
        $0$ & $0$ \\
        % -------------------------------------------------------------- %
        % LSTM-GMM & 
        % 0 & 0 & 
        % 0 & 0 \\
        % -------------------------------------------------------------- %
        BeT & 
        $0.163 \scriptstyle{\pm 0.066}$ & $0.234 \scriptstyle{\pm 0.079}$ & 
        $0.025 \scriptstyle{\pm 0.015}$ & $0.051 \scriptstyle{\pm 0.035}$ & 
        $0.001 \scriptstyle{\pm 0.001}$ & $0$
         \\
        % -------------------------------------------------------------- %
        DDPM-GPT & 
        $0.895 \scriptstyle{\pm 0.013}$ & $0.222 \scriptstyle{\pm 0.052}$ & 
        $0.708 \scriptstyle{\pm 0.031}$ & $0.146 \scriptstyle{\pm 0.029}$ & 
        $0.120 \scriptstyle{\pm 0.018}$ & $0.120 \scriptstyle{\pm 0.039}$
         \\
        % -------------------------------------------------------------- %
        BESO  & 
        $0.909 \scriptstyle{\pm 0.007}$ & $0.382 \scriptstyle{\pm 0.053}$ & 
        $0.685 \scriptstyle{\pm 0.034}$ & $0.177 \scriptstyle{\pm 0.058}$ &
        $0.095 \scriptstyle{\pm 0.006}$ & $0.131 \scriptstyle{\pm 0.028}$\\

        \midrule
        ACT $\rightarrow$ $\pi(a_{t:t+k}|s_t)$ &
        $0.308 \scriptstyle{\pm 0.096}$ & $0.095 \scriptstyle{\pm 0.027}$ & 
        $0.083 \scriptstyle{\pm 0.067}$ & $0.037 \scriptstyle{\pm 0.037}$ & 
        $0.0004$ & $0$
        \\
        \midrule
        DiffusionPolicy $\rightarrow$ $\pi(a_{t:t+k}|s_{t-h+1:t})$ &
        $0.634 \scriptstyle{\pm 0.049}$ & $0.762 \scriptstyle{\pm 0.048}$ & 
        $0.300 \scriptstyle{\pm 0.053}$ & $0.503 \scriptstyle{\pm 0.070}$ & 
        $0.096 \scriptstyle{\pm 0.021}$ & $0.190 \scriptstyle{\pm 0.057}$ 
        \\
	\bottomrule
\end{tabular}

}
\vskip -0.15in
\end{table}


% \begin{table}[hbtp]
% \centering
%  \caption{image-based policy benchmark}\label{image_table}
% \resizebox{\textwidth}{!}{  

% \begin{tabular}{l|cc|cc|cc}
% 	\toprule 
%             & \multicolumn{2}{c|}{Sorting 4 boxes} & \multicolumn{2}{c|}{Sorting 6 boxes} & \multicolumn{2}{c}{cubestacking} \\
            
%         \midrule

%          history=1 (classic mdp) & Success Rate & Entropy & Success Rate & Entropy & S1 & Entropy \\

% 	\midrule

%         MLP  & 
%         $0.666 \scriptstyle{\pm 0.080}$ & $0.996 \scriptstyle{\pm 0.031}$ & 
%         $0.636 \scriptstyle{\pm 0.026}$ & $0.210 \scriptstyle{\pm 0.015}$ & 
%         $0.531 \scriptstyle{\pm 0.054}$ & $0.021 \scriptstyle{\pm 0.014}$ \\
%         % -------------------------------------------------------------- %
%         % BC-GMM  & 
%         % 0 & 0 & 
%         % 0 & 0 & 
%         % 0 & 0 \\
%         % -------------------------------------------------------------- %
%         CVAE & 
%         $0.653 \scriptstyle{\pm 0.061}$ & $0.165 \scriptstyle{\pm 0.010}$ & 
%         $0.570 \scriptstyle{\pm 0.023}$ & $0.236 \scriptstyle{\pm 0.013}$ & 
%         $0.517 \scriptstyle{\pm 0.059}$ & $0.038 \scriptstyle{\pm 0.022}$\\
%         % -------------------------------------------------------------- %
%         BeT-MLP & 
%         $0.671 \scriptstyle{\pm 0.014}$ & $0.296 \scriptstyle{\pm 0.033}$ & 
%         $0.616 \scriptstyle{\pm 0.035}$ & $0.365 \scriptstyle{\pm 0.022}$ & 
%         $0.467 \scriptstyle{\pm 0.046}$ & $0.195 \scriptstyle{\pm 0.044}$\\
%         % -------------------------------------------------------------- %
%         IBC & 
%         $0.707 \scriptstyle{\pm 0.031}$ & $0.236 \scriptstyle{\pm 0.027}$ & 
%         $0.664 \scriptstyle{\pm 0.039}$ & $0.328 \scriptstyle{\pm 0.026}$ & 
%         $0.002 \scriptstyle{\pm 0.003}$ & $0$\\
%         % -------------------------------------------------------------- %
%         DDPM-mlp & 
%         $0.763 \scriptstyle{\pm 0.028}$ & $0.237 \scriptstyle{\pm 0.028}$ & 
%         $0.748 \scriptstyle{\pm 0.026}$ & $0.359 \scriptstyle{\pm 0.025}$ & 
%         $0.645 \scriptstyle{\pm 0.050}$ & $0.137 \scriptstyle{\pm 0.061}$\\
%         % -------------------------------------------------------------- %
%         \midrule

%          history=5 & Success Rate & Entropy & Success Rate & Entropy & Success Rate & Entropy \\

% 	\midrule

%         GPT  & 
%         $0.654 \scriptstyle{\pm 0.048}$ & $0.156 \scriptstyle{\pm 0.018}$ & 
%         $0.590 \scriptstyle{\pm 0.017}$ & $0.297 \scriptstyle{\pm 0.023}$ & 
%         $0.515 \scriptstyle{\pm 0.092}$ & $0.236 \scriptstyle{\pm 0.086}$ \\
%         % -------------------------------------------------------------- %
%         % LSTM-GMM & 
%         % 0 & 0 & 
%         % 0 & 0 & 
%         % 0 & 0\\
%         % -------------------------------------------------------------- %
%         BeT & 
%         $0.676 \scriptstyle{\pm 0.035}$ & $0.305 \scriptstyle{\pm 0.029}$ & 
%         $0.617 \scriptstyle{\pm 0.033}$ & $0.380 \scriptstyle{\pm 0.019}$ & 
%         $0.500 \scriptstyle{\pm 0.054}$ & $0.325 \scriptstyle{\pm 0.082}$\\
%         % -------------------------------------------------------------- %
%         DDPM-GPT & 
%         $0.770 \scriptstyle{\pm 0.022}$ & $0.270 \scriptstyle{\pm 0.033}$ & 
%         $0.710 \scriptstyle{\pm 0.029}$ & $0.314 \scriptstyle{\pm 0.042}$ & 
%         $0.704 \scriptstyle{\pm 0.024}$ & $0.349 \scriptstyle{\pm 0.053}$\\
%         % -------------------------------------------------------------- %
%         BESO  & 
%         0 & 0 & 
%         0 & 0 & 
%         0 & 0\\

%         \midrule
%         ACT $\rightarrow$ $\pi(a_{t:t+k}|s_t)$ &
%         $0.717 \scriptstyle{\pm 0.038}$ & $0.217 \scriptstyle{\pm 0.024}$ & 
%         $0.604 \scriptstyle{\pm 0.017}$ & $0.276 \scriptstyle{\pm 0.007}$ & 
%         $0.572 \scriptstyle{\pm 0.081}$ & $0.219 \scriptstyle{\pm 0.051}$
%         \\
        
% 	\bottomrule
% \end{tabular}

% }
% \vskip -0.15in
% \end{table}


% \begin{table}[hbtp]
% \centering
%  \caption{Ablation study with historical inputs and action sequence for DiffusionPolicy}\label{image_table}
% \resizebox{\textwidth}{!}{  

% \begin{tabular}{l|cc|cc|cc}
% 	\toprule 
%             & \multicolumn{2}{c|}{Obstacle Avoidance} & \multicolumn{2}{c|}{Robot Push} & \multicolumn{2}{c}{Block Push}  \\
            
%         \midrule

%           & Success Rate & Entropy & Success Rate & Entropy & Success Rate & Entropy \\

% 	\midrule

%         h=1,a=1  & 
%         $0.647 \scriptstyle{\pm 0.015}$ & $0.876 \scriptstyle{\pm 0.035}$ & 
%         $0.728 \scriptstyle{\pm 0.049}$ & $0.601 \scriptstyle{\pm 0.049}$ & 
%         $0.389 \scriptstyle{\pm 0.077}$ & $0.729 \scriptstyle{\pm 0.045}$ \\
%         % -------------------------------------------------------------- %
        
%         h=5,a=1 & 
%         $0.674 \scriptstyle{\pm 0.169}$ & $0.778 \scriptstyle{\pm 0.084}$ &
%         $0.757 \scriptstyle{\pm 0.044}$ & $0.782 \scriptstyle{\pm 0.046}$ & 
%         $0.425 \scriptstyle{\pm 0.214}$ & $0.649 \scriptstyle{\pm 0.150}$\\
%         % -------------------------------------------------------------- %
        
%         h=1,a=4 & 
%         $0.871 \scriptstyle{\pm 0.018}$ & $0.916 \scriptstyle{\pm 0.004}$ &
%         $0.830 \scriptstyle{\pm 0.025}$ & $0.726 \scriptstyle{\pm 0.065}$ & 
%         $0.929 \scriptstyle{\pm 0.015}$ & $0.896 \scriptstyle{\pm 0.018}$  
%         \\
%         % -------------------------------------------------------------- %
        
%         h=5,a=4 & 
%         $0.904 \scriptstyle{\pm 0.022}$ & $0.906 \scriptstyle{\pm 0.021}$ &
%         $0.859 \scriptstyle{\pm 0.022}$ & $0.755 \scriptstyle{\pm 0.052}$ & 
%         $0.926 \scriptstyle{\pm 0.021}$ & $0.905 \scriptstyle{\pm 0.013}$ 
%         \\

        
% 	\bottomrule
% \end{tabular}

% }
% \vskip -0.15in
% \end{table}


% \begin{table}[hbtp]
% \centering
%  \caption{Ablation study on length of trajectory for robot push}\label{t:2}
% \resizebox{\textwidth}{!}{  

% \begin{tabular}{l|cc|cc|cc|cc}
% 	\toprule 
%             & \multicolumn{2}{c|}{history=1} & \multicolumn{2}{c|}{history=3} & \multicolumn{2}{c|}{history=5} & \multicolumn{2}{c}{history=10} \\

%         \midrule

%                  & Success Rate & Entropy & Success Rate & Entropy & Success Rate & Entropy & Success Rate & Entropy \\

% 	\midrule

%         GPT  & 
%         $0.0 \scriptstyle{\pm 0.0}$ & $0.0 \scriptstyle{\pm 0.0}$ &
%         $0.806 \scriptstyle{\pm 0.055}$ & $0.073 \scriptstyle{\pm 0.018}$ & 
%         $0.825 \scriptstyle{\pm 0.024}$ & $0.090 \scriptstyle{\pm 0.025}$ & 
%         $0.831 \scriptstyle{\pm 0.024}$ & $0.336 \scriptstyle{\pm 0.071}$ \\
%         % -------------------------------------------------------------- %
%         BeT & 
%         $0.529 \scriptstyle{\pm 0.035}$ & $0.385 \scriptstyle{\pm 0.067}$ &
%         $0.634 \scriptstyle{\pm 0.034}$ & $0.479 \scriptstyle{\pm 0.101}$ & 
%         $0.608 \scriptstyle{\pm 0.045}$ & $0.471 \scriptstyle{\pm 0.138}$ & 
%         $0.684 \scriptstyle{\pm 0.055}$ & $0.482 \scriptstyle{\pm 0.141}$\\
%         % -------------------------------------------------------------- %
%         DDPM-GPT & 
%         $0.732 \scriptstyle{\pm 0.021}$ & $0.541 \scriptstyle{\pm 0.056}$ & 
%         $0.818 \scriptstyle{\pm 0.030}$ & $0.665 \scriptstyle{\pm 0.045}$ & 
%         $0.839 \scriptstyle{\pm 0.016}$ & $0.775 \scriptstyle{\pm 0.061}$ & 
%         $0.858 \scriptstyle{\pm 0.018}$ & $0.756 \scriptstyle{\pm 0.077}$\\
%         % -------------------------------------------------------------- %
%         BESO  & 
%         0 & 0 & 
%         0 & 0 & 
%         0 & 0\\
        
% 	\bottomrule
% \end{tabular}

% }
% \vskip -0.15in
% \end{table}

\begin{table}[hbtp]
\centering
 \caption{Ablation study on the size of dataset for robot push}\label{t:2}
\resizebox{\textwidth}{!}{  

\begin{tabular}{l|cc|cc|cc|cc}
	\toprule 
            & \multicolumn{2}{c|}{25\% dataset} & \multicolumn{2}{c|}{50\% dataset} & \multicolumn{2}{c}{75\% dataset} & \multicolumn{2}{c}{100\% dataset} \\

        \midrule

                 & Success Rate & entropy & Success Rate & entropy & Success Rate & entropy & 
                 Success Rate & entropy\\

	\midrule
        MLP & 
        $0.208 \scriptstyle{\pm 0.125}$ & $0$ & 
        $0.586 \scriptstyle{\pm 0.078}$ & $0$ & 
        $0.691 \scriptstyle{\pm 0.066}$ & $0$ &
        $0.708 \scriptstyle{\pm 0.052}$ & $0$\\
        % -------------------------------------------------------------- %
        CVAE  & 
        $0.035 \scriptstyle{\pm 0.034}$ & $0.002 \scriptstyle{\pm 0.005}$ & 
        $0.121 \scriptstyle{\pm 0.062}$ & $0.020 \scriptstyle{\pm 0.026}$ & 
        $0.363 \scriptstyle{\pm 0.086}$ & $0.034 \scriptstyle{\pm 0.032}$ &
        $0.579 \scriptstyle{\pm 0.138}$ & $0.030 \scriptstyle{\pm 0.053}$\\
        % -------------------------------------------------------------- %
        BeT-MLP & 
        $0.194 \scriptstyle{\pm 0.099}$ & $0.120 \scriptstyle{\pm 0.084}$ & 
        $0.466 \scriptstyle{\pm 0.025}$ & $0.345 \scriptstyle{\pm 0.097}$ & 
        $0.438 \scriptstyle{\pm 0.103}$ & $0.381 \scriptstyle{\pm 0.156}$ &
        $0.507 \scriptstyle{\pm 0.081}$ & $0.485 \scriptstyle{\pm 0.092}$\\
        % -------------------------------------------------------------- %
        IBC & 
        $0.392 \scriptstyle{\pm 0.039}$ & $0.220 \scriptstyle{\pm 0.049}$ & 
        $0.554 \scriptstyle{\pm 0.033}$ & $0.307 \scriptstyle{\pm 0.141}$ & 
        $0.602 \scriptstyle{\pm 0.086}$ & $0.293 \scriptstyle{\pm 0.094}$ &
        $0.638 \scriptstyle{\pm 0.027}$ & $0.300 \scriptstyle{\pm 0.048}$\\
        % -------------------------------------------------------------- %
        DDPM & 
        $0.336 \scriptstyle{\pm 0.131}$ & $0.275 \scriptstyle{\pm 0.162}$ & 
        $0.699 \scriptstyle{\pm 0.009}$ & $0.628 \scriptstyle{\pm 0.041}$ & 
        $0.748 \scriptstyle{\pm 0.029}$ & $0.652 \scriptstyle{\pm 0.029}$ &
        $0.763 \scriptstyle{\pm 0.039}$ & $0.712 \scriptstyle{\pm 0.064}$\\
        % -------------------------------------------------------------- %
        GPT & 
        $0.483 \scriptstyle{\pm 0.086}$ & $0.055 \scriptstyle{\pm 0.019}$ & 
        $0.747 \scriptstyle{\pm 0.060}$ & $0.074 \scriptstyle{\pm 0.040}$ & 
        $0.789 \scriptstyle{\pm 0.039}$ & $0.089 \scriptstyle{\pm 0.036}$ &
        $0.833 \scriptstyle{\pm 0.043}$ & $0$\\
        % -------------------------------------------------------------- %
        BeT & 
        $0.384 \scriptstyle{\pm 0.041}$ & $0.315 \scriptstyle{\pm 0.079}$ & 
        $0.550 \scriptstyle{\pm 0.076}$ & $0.391 \scriptstyle{\pm 0.100}$ & 
        $0.592 \scriptstyle{\pm 0.031}$ & $0.460 \scriptstyle{\pm 0.074}$ &
        $0.645 \scriptstyle{\pm 0.069}$ & $0.536 \scriptstyle{\pm 0.105}$\\
        % -------------------------------------------------------------- %
        DDPM-GPT & 
        $0.690 \scriptstyle{\pm 0.048}$ & $0.573 \scriptstyle{\pm 0.060}$ & 
        $0.785 \scriptstyle{\pm 0.021}$ & $0.699 \scriptstyle{\pm 0.034}$ &
        $0.835 \scriptstyle{\pm 0.024}$ & $0.753 \scriptstyle{\pm 0.037}$ & 
        $0.839 \scriptstyle{\pm 0.020}$ & $0.664 \scriptstyle{\pm 0.075}$\\
        % -------------------------------------------------------------- %
        BESO  & 
        $0.705 \scriptstyle{\pm 0.044}$ & $0.579 \scriptstyle{\pm 0.066}$ & 
        $0.820 \scriptstyle{\pm 0.023}$ & $0.712 \scriptstyle{\pm 0.029}$ & 
        $0.836 \scriptstyle{\pm 0.010}$ & $0.761 \scriptstyle{\pm 0.044}$ &
        $0.861 \scriptstyle{\pm 0.016}$ & $0.711 \scriptstyle{\pm 0.030}$\\
        % -------------------------------------------------------------- %
        ACT & 
        $0.668 \scriptstyle{\pm 0.112}$ & $0.049 \scriptstyle{\pm 0.031}$ & 
        $0.892 \scriptstyle{\pm 0.028}$ & $0.089 \scriptstyle{\pm 0.023}$ & 
        $0.899 \scriptstyle{\pm 0.026}$ & $0.140 \scriptstyle{\pm 0.023}$ &
        $0.891 \scriptstyle{\pm 0.022}$ & $0.025 \scriptstyle{\pm 0.012}$\\
        % -------------------------------------------------------------- %
        DiffusionPolicy & 
        $0.711 \scriptstyle{\pm 0.027}$ & $0.650 \scriptstyle{\pm 0.020}$ & 
        $0.831 \scriptstyle{\pm 0.013}$ & $0.666 \scriptstyle{\pm 0.067}$ & 
        $0.848 \scriptstyle{\pm 0.025}$ & $0.715 \scriptstyle{\pm 0.068}$ &
        $0.849 \scriptstyle{\pm 0.023}$ & $0.749 \scriptstyle{\pm 0.041}$\\
        % -------------------------------------------------------------- %
        
	\bottomrule
\end{tabular}

}
\vskip -0.15in
\end{table}

% \begin{table}[hbtp]
% \centering
%  \caption{Ablation study on the size of dataset for Block Push}\label{t:2}
% \resizebox{\textwidth}{!}{  

% \begin{tabular}{l|cc|cc|cc|cc}
% 	\toprule 
%             & \multicolumn{2}{c|}{25\% dataset} & \multicolumn{2}{c|}{50\% dataset} & \multicolumn{2}{c}{75\% dataset} & \multicolumn{2}{c}{100\% dataset} \\

%         \midrule

%                  & Success Rate & entropy & Success Rate & entropy & Success Rate & entropy \\

% 	\midrule

%         CVAE  & 
%         $0 \scriptstyle{\pm 0}$ & $0 \scriptstyle{\pm 0}$ & 
%         $0 \scriptstyle{\pm 0}$ & $0 \scriptstyle{\pm 0}$ & 
%         0 & 0 \\
%         % -------------------------------------------------------------- %
%         DDPM & 
%         0 & 0 & 
%         0 & 0 & 
%         0 & 0\\
%         % -------------------------------------------------------------- %
%         BeT & 
%         $0 \scriptstyle{\pm 0}$ & $0 \scriptstyle{\pm 0}$ & 
%         $0 \scriptstyle{\pm 0}$ & $0 \scriptstyle{\pm 0}$ & 
%         0 & 0\\
%         % -------------------------------------------------------------- %
%         DDPM-GPT & 
%         $0 \scriptstyle{\pm 0}$ & $0 \scriptstyle{\pm 0}$ & 
%         $0 \scriptstyle{\pm 0}$ & $0 \scriptstyle{\pm 0}$ & 
%         0 & 0\\
%         % -------------------------------------------------------------- %
%         BESO  & 
%         0 & 0 & 
%         0 & 0 & 
%         0 & 0\\
        
% 	\bottomrule
% \end{tabular}

% }
% \vskip -0.15in
% \end{table}


% \begin{table}[hbtp]
% \centering
%  \caption{Ablation study with DDPM-GPT policy selection standards}\label{image_table}
% \resizebox{\textwidth}{!}{  

% \begin{tabular}{l|cc|cc|cc}
% 	\toprule 
%             & \multicolumn{2}{c|}{Robot Push} & \multicolumn{2}{c|}{Sorting 4 Boxes} & \multicolumn{2}{c}{Image-based Sorting 4 boxes}  \\
            
%         \midrule

%           & Success Rate & Entropy & Success Rate & Entropy & Success Rate & Entropy \\

% 	\midrule

%         MSE loss  & 
%         $0. \scriptstyle{\pm 0.}$ & $0. \scriptstyle{\pm 0.}$ & 
%         $0. \scriptstyle{\pm 0.}$ & $0. \scriptstyle{\pm 0.}$ & 
%         $0. \scriptstyle{\pm 0.}$ & $0. \scriptstyle{\pm 0.}$ \\
%         % -------------------------------------------------------------- %
        
%         ELBO & 
%         $0.839 \scriptstyle{\pm 0.016}$ & $0.775 \scriptstyle{\pm 0.061}$ &
%         $0.340 \scriptstyle{\pm 0.064}$ & $0.392 \scriptstyle{\pm 0.067}$ & 
%         $0. \scriptstyle{\pm 0.}$ & $0. \scriptstyle{\pm 0.}$\\
%         % -------------------------------------------------------------- %
        
%         Last checkpoint & 
%         $0. \scriptstyle{\pm 0.}$ & $0. \scriptstyle{\pm 0.}$ &
%         $0.491 \scriptstyle{\pm 0.071}$ & $0.430 \scriptstyle{\pm 0.049}$ & 
%         $0. \scriptstyle{\pm 0.}$ & $0. \scriptstyle{\pm 0.}$  
%         \\
%         % -------------------------------------------------------------- %
        
%         Simulation performance & 
%         $0. \scriptstyle{\pm 0.}$ & $0. \scriptstyle{\pm 0.}$ &
%         $0. \scriptstyle{\pm 0.}$ & $0. \scriptstyle{\pm 0.}$ & 
%         $0.770 \scriptstyle{\pm 0.022}$ & $0.270 \scriptstyle{\pm 0.033}$ 
%         \\

        
% 	\bottomrule
% \end{tabular}

% }
% \vskip -0.15in
% \end{table}


% \begin{table}[hbtp]
% \centering
%  \caption{Ablation study with DDPM-GPT policy selection standards}\label{image_table}
% \resizebox{\textwidth}{!}{  

% \begin{tabular}{l|cc|cc|cc}
% 	\toprule 
%             & \multicolumn{2}{c|}{Robot Push} & \multicolumn{2}{c|}{Sorting 4 Boxes} & \multicolumn{2}{c}{Image-based Sorting 4 boxes}  \\
            
%         \midrule

%           & Success Rate & Entropy & Success Rate & Entropy & Success Rate & Entropy \\

% 	\midrule

%         MSE loss  & 
%         $0. \scriptstyle{\pm 0.}$ & $0. \scriptstyle{\pm 0.}$ & 
%         $0. \scriptstyle{\pm 0.}$ & $0. \scriptstyle{\pm 0.}$ & 
%         $0. \scriptstyle{\pm 0.}$ & $0. \scriptstyle{\pm 0.}$ \\
%         % -------------------------------------------------------------- %
        
%         ELBO & 
%         $0.839 \scriptstyle{\pm 0.016}$ & $0.775 \scriptstyle{\pm 0.061}$ &
%         $0.340 \scriptstyle{\pm 0.064}$ & $0.392 \scriptstyle{\pm 0.067}$ & 
%         $0. \scriptstyle{\pm 0.}$ & $0. \scriptstyle{\pm 0.}$\\
%         % -------------------------------------------------------------- %
        
%         Last checkpoint & 
%         $0. \scriptstyle{\pm 0.}$ & $0. \scriptstyle{\pm 0.}$ &
%         $0.491 \scriptstyle{\pm 0.071}$ & $0.430 \scriptstyle{\pm 0.049}$ & 
%         $0. \scriptstyle{\pm 0.}$ & $0. \scriptstyle{\pm 0.}$  
%         \\
%         % -------------------------------------------------------------- %
        
%         Simulation performance & 
%         $0. \scriptstyle{\pm 0.}$ & $0. \scriptstyle{\pm 0.}$ &
%         $0. \scriptstyle{\pm 0.}$ & $0. \scriptstyle{\pm 0.}$ & 
%         $0.770 \scriptstyle{\pm 0.022}$ & $0.270 \scriptstyle{\pm 0.033}$ 
%         \\

        
% 	\bottomrule
% \end{tabular}

% }
% \vskip -0.15in
% \end{table}

==> sections/experiments_old.tex <==
\section{Experimental Results}
In this section, we report experimental results with 11 imitation learning methods across 5 manipulation tasks. We conduct both state-based experiments and image-based experiments. According to the results, we present our findings and analyses for what could be influential for robot manipulation and how the current models deal with multi-modality.



\begin{table}[hbtp]
\centering
 \caption{2d robot manipulation tasks benchmark with state policy}\label{t_2}
 
\resizebox{\textwidth}{!}{  

\begin{tabular}{l|cc|ccc|ccc}
	\toprule 
            & \multicolumn{2}{c|}{Obstacle Avoidance} & \multicolumn{3}{c|}{Robot Push (2 modes)} & \multicolumn{3}{c}{Block Push (4 modes)} \\
            
        \midrule

         history=1 $\rightarrow$ $\pi(a_t|s_t)$ & Success Rate & Entropy & Success Rate & Distance Error & Entropy & Success Rate & Distance Error & Entropy  \\

	\midrule

        MLP  & 
        $0.666 \scriptstyle{\pm 0.512}$ & 0 & 
        $0.708 \scriptstyle{\pm 0.052}$ & $0.094 \scriptstyle{\pm 0.024}$ & $0$ & 
        $0.522 \scriptstyle{\pm 0.165}$ & $0.130 \scriptstyle{\pm 0.043} $ & $0$ 
        \\
        
        % -------------------------------------------------------------- %
        
        % BC-GMM  & 
        % $0.091 \scriptstyle{\pm 0.045}$ & $0.296 \scriptstyle{\pm 0.098}$ & 
        % 0 & 0 & 0 & 
        % 0 & 0 & 0
        % \\
        
        % -------------------------------------------------------------- %
        
        CVAE & 
        $0.716 \scriptstyle{\pm 0.265}$ & $0.195 \scriptstyle{\pm 0.111}$ & 
        $0.579 \scriptstyle{\pm 0.138}$ & $0.122 \scriptstyle{\pm 0.040}$ & $0.030 \scriptstyle{\pm 0.053}$ & 
        $\mathbf{0.604 \scriptstyle{\pm 0.087}}$ & $0.108 \scriptstyle{\pm 0.025}$ & $0.170 \scriptstyle{\pm 0.031}$  \\

        % -------------------------------------------------------------- %
        
        BeT-MLP & 
        $0.665 \scriptstyle{\pm 0.136}$ & $0.836 \scriptstyle{\pm 0.071}$ & 
        $0.507 \scriptstyle{\pm 0.081}$ & $0.143 \scriptstyle{\pm 0.030}$ & $0.485 \scriptstyle{\pm 0.092}$ & 
        $0.420 \scriptstyle{\pm 0.049}$ & $0.143 \scriptstyle{\pm 0.010}$ & $0.628 \scriptstyle{\pm 0.123}$ \\

        % -------------------------------------------------------------- %
        
        IBC & 
        $\mathbf{0.760 \scriptstyle{\pm 0.046}}$ & $\mathbf{0.850 \scriptstyle{\pm 0.038}}$ & 
        $0.638 \scriptstyle{\pm 0.027}$ & $0.107 \scriptstyle{\pm 0.011}$ & $0.300 \scriptstyle{\pm 0.048}$ & 
        $0.574 \scriptstyle{\pm 0.048}$ & $\mathbf{0.107 \scriptstyle{\pm 0.015}}$ & $\mathbf{0.816 \scriptstyle{\pm 0.028}}$  \\

        % -------------------------------------------------------------- %
        
        DDPM-MLP & 
        $0.637 \scriptstyle{\pm 0.055}$ & $0.801 \scriptstyle{\pm 0.034}$ & 
        $\mathbf{0.763 \scriptstyle{\pm 0.039}}$ & $\mathbf{0.082 \scriptstyle{\pm 0.017}}$ & $\mathbf{0.712 \scriptstyle{\pm 0.064}}$ &  
        $0.569 \scriptstyle{\pm 0.047}$ & $0.111 \scriptstyle{\pm 0.012}$ & $0.796 \scriptstyle{\pm 0.043}$  \\

        \midrule
        
        history=5 $\rightarrow$ $\pi(a_t|s_{t-h+1:t})$ & Success Rate & Entropy & Success Rate & Distance Error & Entropy & Success Rate & Distance Error & Entropy \\

	\midrule

        GPT  & 
        $0.833 \scriptstyle{\pm 0.408}$ & $0$ & 
        $0.833 \scriptstyle{\pm 0.043}$ & $0.070 \scriptstyle{\pm 0.037}$ & $0$ & 
        $0.855 \scriptstyle{\pm 0.054}$ & $0.063 \scriptstyle{\pm 0.014}$ & $0$  \\

        % -------------------------------------------------------------- %
        
        % LSTM-GMM & 
        % 0 & 0 & 
        % 0 & 0 & 0 & 
        % 0 & 0 & 0 
        % \\

        % -------------------------------------------------------------- %
                
        BeT & 
        $0.747 \scriptstyle{\pm 0.030}$ & $0.844 \scriptstyle{\pm 0.035}$ & 
        $0.645 \scriptstyle{\pm 0.069}$ & $0.115 \scriptstyle{\pm 0.009}$ & $0.536 \scriptstyle{\pm 0.105}$ & 
        $0.724 \scriptstyle{\pm 0.051}$ & $0.079 \scriptstyle{\pm 0.009}$ & $0.788 \scriptstyle{\pm 0.031}$  \\
        % -------------------------------------------------------------- %
        
        DDPM-GPT & 
        $0.927 \scriptstyle{\pm 0.022}$ & $\mathbf{0.898 \scriptstyle{\pm 0.018}}$ & 
        $0.839 \scriptstyle{\pm 0.020}$ & $0.062 \scriptstyle{\pm 0.009}$ & $0.664 \scriptstyle{\pm 0.075}$ & 
        $0.847 \scriptstyle{\pm 0.050}$ & $0.056\scriptstyle{\pm 0.012}$ & $0.862 \scriptstyle{\pm 0.017}$ 
        
        \\
        
        BESO & 
        $\mathbf{0.950 \scriptstyle{\pm 0.015}}$ & $0.856 \scriptstyle{\pm 0.018}$ & 
        $0.861 \scriptstyle{\pm 0.016}$ & $0.053 \scriptstyle{\pm 0.004}$ & $0.711 \scriptstyle{\pm 0.030}$ &
        $0.794 \scriptstyle{\pm 0.095}$ & $0.060 \scriptstyle{\pm 0.015}$ & $\mathbf{0.871 \scriptstyle{\pm 0.037}}$ 
        
        \\
        
        \midrule
        ACT $\rightarrow$ $\pi(a_{t:t+k}|s_t)$ &
        $0.388 \scriptstyle{\pm 0.382}$ & $0.126 \scriptstyle{\pm 0.146}$ & 
        $\mathbf{0.891 \scriptstyle{\pm 0.022}}$ & $\mathbf{0.048 \scriptstyle{\pm 0.014}}$ & $0.025 \scriptstyle{\pm 0.012}$ & 
        $\mathbf{0.951 \scriptstyle{\pm 0.033}}$ & $\mathbf{0.041 \scriptstyle{\pm 0.009}}$ & $0.070 \scriptstyle{\pm 0.029}$
        \\
        
        \midrule
        DiffusionPolicy $\rightarrow$ $\pi(a_{t:t+k}|s_{t-h+1:t})$ &
        $0.899 \scriptstyle{\pm 0.006}$ & $0.863 \scriptstyle{\pm 0.068}$ & 
        $0.849 \scriptstyle{\pm 0.023}$ & $0.056 \scriptstyle{\pm 0.009}$ & $\mathbf{0.749 \scriptstyle{\pm 0.041}}$ & 
        $0.920 \scriptstyle{\pm 0.027}$ & $0.043 \scriptstyle{\pm 0.006}$ & $0.859 \scriptstyle{\pm 0.012}$
        \\
	\bottomrule
\end{tabular}

}
\vskip -0.15in
\end{table}

\subsection{State-based policy comparison}
We first evaluate all methods on the Obstacle Avoidance, which is designed to test the model's ability to learn multi-modal distributions. In this task, we only have training dataset and all models are trained for 2000 epochs and simulated using the last checkpoint with 6 seeds. For other tasks, we split the demonstrations into training data (90\%) and validation data (10\%). We report the simulation results using the model with best loss on validation data. Notice that we use the same loss during training and evaluation in order to match each model's objective. We mainly use success rate and mode entropy as metrics for most tasks, except for Box Alignment and Block Push, which are additionally evaluated by distance error (the detailed definition can be found in Appendix \ref{Tasks details}). The results are reported in Table \ref{t_2}, \ref{sorting_table} and \ref{cs_table}. We present our key findings below.

\textbf{Multiple ways to deal with multi-modality}. Since deterministic models including MLP and GPT can only generate one solution give a context, they are not able to learn diverse behaviors. VAE based models including CVAE and ACT can generate different behaviors, but the mode entropy is quite low which means it only covers a small part of distributions. The IBC, BeT and diffusion based models are all able to learn multi-modal distributions.

\textbf{The trade-off between success rate and entropy}. We find that there is a trade-off between success rate and entropy. For most tasks, it is hard to find one method that is best on both success rate and entropy. Increasing the entropy or diversity to some extent will degrade the success rate. The MLP and GPT has $0$ entropy, but their success rate is quite high across all methods, better than other BeT and some diffusion methods. The ACT shows best success rate on almost all tasks, but it's entropy is very low.

\textbf{History and action chunking matter a lot}. From the experiments, the models with historical inputs or action sequence generally perform much better than step-based models.

\textbf{Diffusion based models generalize very well}. 

\textbf{Manipulating multiple objects is challenging for state-based policy}. In this task, we simply stack the features of robots and boxes, which could be problematic when there are dozens of objects. The observation space becomes rather complex when increasing the number of boxes. From the experiments, we observe a severe performance drop when sorting 4 and 6 boxes. 

\subsection{Image-based policy comparison}
Except for state-based results, we also implemented image-based policies for each manipulation task. For fair comparison, all the methods share the same image encoder ResNet-18. The results are reported in Table \ref{image_table}. Here we mainly report the results on sorting task and cubestacking task, since these two tasks are quite hard for state-based policy. It is very interesting to find that image-based policy actually performs much better than state-based policy on these two tasks. 

\textbf{Image-based policy can perform better than state-based policy on multi-objects tasks}

\textbf{Sequential information does not improve performance for image-based policy}

\textbf{It is hard for image-based policy to capture multi-modal distribution}


\begin{figure*}[t]
        \centering
        % \subfigure[Obstacle Avoidance]{
            \begin{minipage}[t!]{0.48\textwidth}
                \centering 
                \includegraphics[width=0.48\textwidth]{figures/diffusionpolicy_ablation/Success Rate.pdf}
                \includegraphics[width=0.48\textwidth]{figures/diffusionpolicy_ablation/Entropy.pdf}

                \subcaption[]{Diffusion Policy Ablation}
            \end{minipage}
        % }
        \hfill
        % \subfigure[Obstacle Avoidance]{
            \begin{minipage}[t!]{0.48\textwidth}
                \centering 
                \includegraphics[width=0.48\textwidth]{figures/diffusionpolicy_ablation/ddpm_Success Rate.pdf}
                \includegraphics[width=0.48\textwidth]{figures/diffusionpolicy_ablation/ddpm_Entropy.pdf}

                \subcaption[]{GPT-based policy Ablation}
            \end{minipage}
        % }
        % \begin{minipage}[t!]{0.2\textwidth}
        %     \centering 
        %     \includegraphics[width=\textwidth]{figures/diffusionpolicy_ablation/Success Rate.pdf}
        %     \includegraphics[width=\textwidth]{figures/diffusionpolicy_ablation/Entropy.pdf}
        %     \subcaption[]{Diffusion Policy Ablation}
        %     \label{fig:diffusionpolicy_ablation}
        % \end{minipage}
        % \hfill
        % \begin{minipage}[t!]{0.2\textwidth}
        %     \centering 
        %     \includegraphics[width=\textwidth]{figures/diffusionpolicy_ablation/ddpm_Success Rate.pdf}
        %     \includegraphics[width=\textwidth]{figures/diffusionpolicy_ablation/ddpm_Entropy.pdf}
        %     \subcaption[]{GPT-based policy Ablation}
        %     \label{fig:diffusionpolicy_ablation}
        % \end{minipage}
        % \hfill
        \caption[ ]
        {\small \textbf{Environments.} We created 5 tasks in this paper, including one toy task Obstacle Avoidance and 4 robot manipulation tasks. For each task, we collected a large amount of human demonstrations with diverse behaviors. }
        \label{fig:environments}
\end{figure*}

\subsection{Ablation study on historical input and action sequence}
From the above results, both historical inputs and action sequence help a lot with state-based policies. In order to explore more about how these two factors influence the model's performance, we conduct an ablation study using DiffusionPolicy.

\subsection{Ablation Study on Dataset Size}
Recording demonstrations is very tedious for imitation learning. In order to study how many demonstrations could be enough to train a well-performed policy, we generate three subsets which contain 25\%, 50\% and 75\% demonstrations of the whole dataset for the block push and box alignment tasks. Here we only compare the methods with historical inputs since they perform much better than MLP-based methods. The results are presented in table 5. 

\subsection{Policy Selection}
Model selection is a challenging problem for imitation learning. Choosing model either with best loss on evaluation data or with last checkpoint could cause significantly performance drop \cite{mandlekar2021matters}. Previous works would report the best simulation results during training, while this would require more training time and is not suitable for real world. In this paper, we conduct an ablation study on different model selection methods.

\subsection{Inference time comparison}
....
% \subsection{Ablation Study on different size of model}
% All the methods share the same size of MLP or transformer in our main experiments for fair comparison. However, for some tasks with large dataset such as sorting 4/6 boxes and cubestacking, the model could underfit the data. We provide an ablation study to test the influence of different network's size.


\begin{table}[hbtp]
\centering
 \caption{Sorting tasks benchmark}\label{sorting_table}
\resizebox{\textwidth}{!}{  

\begin{tabular}{l|cc|cc|cc}
	\toprule 
            & \multicolumn{2}{c|}{Sorting 2 boxes} & \multicolumn{2}{c|}{Sorting 4 boxes} & \multicolumn{2}{c}{Sorting 6 boxes} \\
            
        \midrule

         history=1 $\rightarrow$ $\pi(a_t|s_t)$ & Success Rate & Entropy & Success Rate & Entropy & Success Rate & Entropy \\

	\midrule

        MLP  & 
        $0.444 \scriptstyle{\pm 0.069}$ & $0$ & 
        $0.058 \scriptstyle{\pm 0.048}$ & $0$ & 
        $0.016 \scriptstyle{\pm 0.014}$ & 0 \\
        % -------------------------------------------------------------- %
        % BC-GMM  & 
        % 0 & 0 & 
        % 0 & 0 & 
        % 0 & 0 \\
        % -------------------------------------------------------------- %
        CVAE & 
        $0.451 \scriptstyle{\pm 0.059}$ & $0.106 \scriptstyle{\pm 0.051}$ & 
        $0.079 \scriptstyle{\pm 0.042}$ & $0.090 \scriptstyle{\pm 0.032}$ & 
        $0.030 \scriptstyle{\pm 0.016}$ & $0.086 \scriptstyle{\pm 0.017}$\\
        % -------------------------------------------------------------- %
        BeT-MLP & 
        $0.317 \scriptstyle{\pm 0.070}$ & $0.309 \scriptstyle{\pm 0.059}$ & 
        $0.003 \scriptstyle{\pm 0.001}$ & $0.021 \scriptstyle{\pm 0.052}$ & 
        $0$ & $0$\\
        % -------------------------------------------------------------- %
        IBC & 
        $0.459 \scriptstyle{\pm 0.033}$ & $\mathbf{0.370 \scriptstyle{\pm 0.071}}$ & 
        $0.080 \scriptstyle{\pm 0.016}$ & $0.097 \scriptstyle{\pm 0.026}$ & 
        $0.007 \scriptstyle{\pm 0.005}$ & $0.024 \scriptstyle{\pm 0.028}$\\
        % -------------------------------------------------------------- %
        DDPM-mlp & 
        $\mathbf{0.460 \scriptstyle{\pm 0.039}}$ & $0.327 \scriptstyle{\pm 0.037}$ & 
        $0.032 \scriptstyle{\pm 0.009}$ & $0.071 \scriptstyle{\pm 0.025}$ & 
        $0$ & $0$\\
        % -------------------------------------------------------------- %
        \midrule

         history=5 $\rightarrow$ $\pi(a_t|s_{t-h+1:t})$ & Success Rate & Entropy & Success Rate & Entropy & Success Rate & Entropy \\

	\midrule

        GPT  & 
        $0.800 \scriptstyle{\pm 0.040}$ & $0$ & 
        $0.075 \scriptstyle{\pm 0.063}$ & $0$ & 
        $0.007 \scriptstyle{\pm 0.003}$ & $0$ \\
        % -------------------------------------------------------------- %
        % LSTM-GMM & 
        % 0 & 0 & 
        % 0 & 0 & 
        % 0 & 0\\
        % -------------------------------------------------------------- %
        BeT & 
        $0.680 \scriptstyle{\pm 0.060}$ & $\mathbf{0.473 \scriptstyle{\pm 0.049}}$ & 
        $0.018 \scriptstyle{\pm 0.010}$ & $0.059 \scriptstyle{\pm 0.035}$ & 
        $0$ & $0$\\
        % -------------------------------------------------------------- %
        DDPM-GPT & 
        $0.854 \scriptstyle{\pm 0.013}$ & $0.431 \scriptstyle{\pm 0.060}$ & 
        $0.337 \scriptstyle{\pm 0.084}$ & $\mathbf{0.372 \scriptstyle{\pm 0.068}}$ & 
        $0.005 \scriptstyle{\pm 0.003}$ & $0.031 \scriptstyle{\pm 0.029}$\\
        % -------------------------------------------------------------- %
        BESO  & 
        $0.784 \scriptstyle{\pm 0.026}$ & $0.387 \scriptstyle{\pm 0.038}$ & 
        $0.188 \scriptstyle{\pm 0.042}$ & $0.232 \scriptstyle{\pm 0.040}$ & 
        $0.020 \scriptstyle{\pm 0.002}$ & $0.055 \scriptstyle{\pm 0.031}$ \\

        \midrule
        ACT $\rightarrow$ $\pi(a_{t:t+k}|s_t)$ &
        $0.858 \scriptstyle{\pm 0.073}$ & $0.012 \scriptstyle{\pm 0.018}$ & 
        $\mathbf{0.565 \scriptstyle{\pm 0.108}}$ & $0.114 \scriptstyle{\pm 0.020}$ & 
        $0.021 \scriptstyle{\pm 0.019}$ & $0.057 \scriptstyle{\pm 0.040}$
        \\
        \midrule
        DiffusionPolicy $\rightarrow$ $\pi(a_{t:t+k}|s_{t-h+1:t})$ &
        $\mathbf{0.882 \scriptstyle{\pm 0.023}}$ & $0.347 \scriptstyle{\pm 0.048}$ & 
        $0.300 \scriptstyle{\pm 0.060}$ & $0.300 \scriptstyle{\pm 0.051}$ & 
        $0.0 \scriptstyle{\pm 0.0}$ & $0.0 \scriptstyle{\pm 0.0}$ 
        \\
	\bottomrule
\end{tabular}

}

\vskip -0.15in
\end{table}


\begin{table}[hbtp]
\centering
 \caption{CubeStacking task benchmark}\label{cs_table}
\resizebox{\textwidth}{!}{  

\begin{tabular}{l|cc|cc|cc}
	\toprule 
            & \multicolumn{4}{c}{CubeStacking} \\
            
        \midrule

         history=1 $\rightarrow$ $\pi(a_t|s_t)$ &  S1 & Entropy & S2 & Entropy & S3 & Entropy \\

	\midrule

        MLP  & 
        $0.030 \scriptstyle{\pm 0.022}$ & $0$ & 
        0 & 0 &
        0 & 0 \\
        % -------------------------------------------------------------- %
        % BC-GMM  & 
        % 0 & 0 & 
        % 0 & 0  \\
        % -------------------------------------------------------------- %
        CVAE & 
        $0.036 \scriptstyle{\pm 0.023}$ & $0.064 \scriptstyle{\pm 0.092}$ & 
        $0.001 \scriptstyle{\pm 0.001}$ & $0$ &
        $0$ & $0$\\
        % -------------------------------------------------------------- %
        BeT-MLP & 
        $0.102 \scriptstyle{\pm 0.059}$ & $0.120 \scriptstyle{\pm 0.031}$ & 
        $0.003 \scriptstyle{\pm 0.001}$ & $0$ &
        $0$ & $0$\\
        % -------------------------------------------------------------- %
        IBC & 
        $0.010 \scriptstyle{\pm 0.016}$ & $0.013 \scriptstyle{\pm 0.027}$ & 
        $0$ & $0$ &
        $0$ & $0$\\
        % -------------------------------------------------------------- %
        DDPM-mlp & 
        $0.244 \scriptstyle{\pm 0.161}$ & $0.113 \scriptstyle{\pm 0.084}$ & 
        $0.042 \scriptstyle{\pm 0.045}$ & $0.011 \scriptstyle{\pm 0.014}$ &
        $0.001 \scriptstyle{\pm 0.0009}$ & $0.096 \scriptstyle{\pm 0.193}$\\
        % -------------------------------------------------------------- %
        \midrule

         history=5 $\rightarrow$ $\pi(a_t|s_{t-h+1:t})$ & S1 & Entropy & S2 & Entropy & S3 & Entropy \\

	\midrule

        GPT  & 
        $0.241 \scriptstyle{\pm 0.055}$ & $0$ & 
        $0.025 \scriptstyle{\pm 0.016}$ & $0$ &
        $0$ & $0$ \\
        % -------------------------------------------------------------- %
        % LSTM-GMM & 
        % 0 & 0 & 
        % 0 & 0 \\
        % -------------------------------------------------------------- %
        BeT & 
        $0.163 \scriptstyle{\pm 0.066}$ & $0.234 \scriptstyle{\pm 0.079}$ & 
        $0.025 \scriptstyle{\pm 0.015}$ & $0.051 \scriptstyle{\pm 0.035}$ & 
        $0.001 \scriptstyle{\pm 0.001}$ & $0$
         \\
        % -------------------------------------------------------------- %
        DDPM-GPT & 
        $0.895 \scriptstyle{\pm 0.013}$ & $0.222 \scriptstyle{\pm 0.052}$ & 
        $0.708 \scriptstyle{\pm 0.031}$ & $0.146 \scriptstyle{\pm 0.029}$ & 
        $0.120 \scriptstyle{\pm 0.018}$ & $0.120 \scriptstyle{\pm 0.039}$
         \\
        % -------------------------------------------------------------- %
        BESO  & 
        $0.909 \scriptstyle{\pm 0.007}$ & $0.382 \scriptstyle{\pm 0.053}$ & 
        $0.685 \scriptstyle{\pm 0.034}$ & $0.177 \scriptstyle{\pm 0.058}$ &
        $0.095 \scriptstyle{\pm 0.006}$ & $0.131 \scriptstyle{\pm 0.028}$\\

        \midrule
        ACT $\rightarrow$ $\pi(a_{t:t+k}|s_t)$ &
        $0.308 \scriptstyle{\pm 0.096}$ & $0.095 \scriptstyle{\pm 0.027}$ & 
        $0.083 \scriptstyle{\pm 0.067}$ & $0.037 \scriptstyle{\pm 0.037}$ & 
        $0.0004$ & $0$
        \\
        \midrule
        DiffusionPolicy $\rightarrow$ $\pi(a_{t:t+k}|s_{t-h+1:t})$ &
        $0.482 \scriptstyle{\pm 0.093}$ & $0.593 \scriptstyle{\pm 0.163}$ & 
        $0.170 \scriptstyle{\pm 0.059}$ & $0.305 \scriptstyle{\pm 0.095}$ & 
        $0.029 \scriptstyle{\pm 0.019}$ & $0.090 \scriptstyle{\pm 0.051}$ 
        \\
	\bottomrule
\end{tabular}

}
\vskip -0.15in
\end{table}


\begin{table}[hbtp]
\centering
 \caption{image-based policy benchmark}\label{image_table}
\resizebox{\textwidth}{!}{  

\begin{tabular}{l|cc|cc|cc}
	\toprule 
            & \multicolumn{2}{c|}{Sorting 4 boxes} & \multicolumn{2}{c|}{Sorting 6 boxes} & \multicolumn{2}{c}{cubestacking} \\
            
        \midrule

         history=1 (classic mdp) & Success Rate & Entropy & Success Rate & Entropy & S1 & Entropy \\

	\midrule

        MLP  & 
        $0.666 \scriptstyle{\pm 0.080}$ & $0.996 \scriptstyle{\pm 0.031}$ & 
        $0.636 \scriptstyle{\pm 0.026}$ & $0.210 \scriptstyle{\pm 0.015}$ & 
        $0.531 \scriptstyle{\pm 0.054}$ & $0.021 \scriptstyle{\pm 0.014}$ \\
        % -------------------------------------------------------------- %
        % BC-GMM  & 
        % 0 & 0 & 
        % 0 & 0 & 
        % 0 & 0 \\
        % -------------------------------------------------------------- %
        CVAE & 
        $0.653 \scriptstyle{\pm 0.061}$ & $0.165 \scriptstyle{\pm 0.010}$ & 
        $0.570 \scriptstyle{\pm 0.023}$ & $0.236 \scriptstyle{\pm 0.013}$ & 
        $0.517 \scriptstyle{\pm 0.059}$ & $0.038 \scriptstyle{\pm 0.022}$\\
        % -------------------------------------------------------------- %
        BeT-MLP & 
        $0.671 \scriptstyle{\pm 0.014}$ & $0.296 \scriptstyle{\pm 0.033}$ & 
        $0.616 \scriptstyle{\pm 0.035}$ & $0.365 \scriptstyle{\pm 0.022}$ & 
        $0.467 \scriptstyle{\pm 0.046}$ & $0.195 \scriptstyle{\pm 0.044}$\\
        % -------------------------------------------------------------- %
        IBC & 
        $0.707 \scriptstyle{\pm 0.031}$ & $0.236 \scriptstyle{\pm 0.027}$ & 
        $0.664 \scriptstyle{\pm 0.039}$ & $0.328 \scriptstyle{\pm 0.026}$ & 
        $0.002 \scriptstyle{\pm 0.003}$ & $0$\\
        % -------------------------------------------------------------- %
        DDPM-mlp & 
        $0.763 \scriptstyle{\pm 0.028}$ & $0.237 \scriptstyle{\pm 0.028}$ & 
        $0.748 \scriptstyle{\pm 0.026}$ & $0.359 \scriptstyle{\pm 0.025}$ & 
        $0.645 \scriptstyle{\pm 0.050}$ & $0.137 \scriptstyle{\pm 0.061}$\\
        % -------------------------------------------------------------- %
        \midrule

         history=5 & Success Rate & Entropy & Success Rate & Entropy & Success Rate & Entropy \\

	\midrule

        GPT  & 
        $0.654 \scriptstyle{\pm 0.048}$ & $0.156 \scriptstyle{\pm 0.018}$ & 
        $0.590 \scriptstyle{\pm 0.017}$ & $0.297 \scriptstyle{\pm 0.023}$ & 
        $0.515 \scriptstyle{\pm 0.092}$ & $0.236 \scriptstyle{\pm 0.086}$ \\
        % -------------------------------------------------------------- %
        % LSTM-GMM & 
        % 0 & 0 & 
        % 0 & 0 & 
        % 0 & 0\\
        % -------------------------------------------------------------- %
        BeT & 
        $0.676 \scriptstyle{\pm 0.035}$ & $0.305 \scriptstyle{\pm 0.029}$ & 
        $0.617 \scriptstyle{\pm 0.033}$ & $0.380 \scriptstyle{\pm 0.019}$ & 
        $0.500 \scriptstyle{\pm 0.054}$ & $0.325 \scriptstyle{\pm 0.082}$\\
        % -------------------------------------------------------------- %
        DDPM-GPT & 
        $0.770 \scriptstyle{\pm 0.022}$ & $0.270 \scriptstyle{\pm 0.033}$ & 
        $0.710 \scriptstyle{\pm 0.029}$ & $0.314 \scriptstyle{\pm 0.042}$ & 
        $0.704 \scriptstyle{\pm 0.024}$ & $0.349 \scriptstyle{\pm 0.053}$\\
        % -------------------------------------------------------------- %
        BESO  & 
        0 & 0 & 
        0 & 0 & 
        0 & 0\\

        \midrule
        ACT $\rightarrow$ $\pi(a_{t:t+k}|s_t)$ &
        $0.717 \scriptstyle{\pm 0.038}$ & $0.217 \scriptstyle{\pm 0.024}$ & 
        $0.604 \scriptstyle{\pm 0.017}$ & $0.276 \scriptstyle{\pm 0.007}$ & 
        $0.572 \scriptstyle{\pm 0.081}$ & $0.219 \scriptstyle{\pm 0.051}$
        \\
        
	\bottomrule
\end{tabular}

}
\vskip -0.15in
\end{table}


% \begin{table}[hbtp]
% \centering
%  \caption{Ablation study with historical inputs and action sequence for DiffusionPolicy}\label{image_table}
% \resizebox{\textwidth}{!}{  

% \begin{tabular}{l|cc|cc|cc}
% 	\toprule 
%             & \multicolumn{2}{c|}{Obstacle Avoidance} & \multicolumn{2}{c|}{Robot Push} & \multicolumn{2}{c}{Block Push}  \\
            
%         \midrule

%           & Success Rate & Entropy & Success Rate & Entropy & Success Rate & Entropy \\

% 	\midrule

%         h=1,a=1  & 
%         $0.647 \scriptstyle{\pm 0.015}$ & $0.876 \scriptstyle{\pm 0.035}$ & 
%         $0.728 \scriptstyle{\pm 0.049}$ & $0.601 \scriptstyle{\pm 0.049}$ & 
%         $0.389 \scriptstyle{\pm 0.077}$ & $0.729 \scriptstyle{\pm 0.045}$ \\
%         % -------------------------------------------------------------- %
        
%         h=5,a=1 & 
%         $0.674 \scriptstyle{\pm 0.169}$ & $0.778 \scriptstyle{\pm 0.084}$ &
%         $0.757 \scriptstyle{\pm 0.044}$ & $0.782 \scriptstyle{\pm 0.046}$ & 
%         $0.425 \scriptstyle{\pm 0.214}$ & $0.649 \scriptstyle{\pm 0.150}$\\
%         % -------------------------------------------------------------- %
        
%         h=1,a=4 & 
%         $0.871 \scriptstyle{\pm 0.018}$ & $0.916 \scriptstyle{\pm 0.004}$ &
%         $0.830 \scriptstyle{\pm 0.025}$ & $0.726 \scriptstyle{\pm 0.065}$ & 
%         $0.929 \scriptstyle{\pm 0.015}$ & $0.896 \scriptstyle{\pm 0.018}$  
%         \\
%         % -------------------------------------------------------------- %
        
%         h=5,a=4 & 
%         $0.904 \scriptstyle{\pm 0.022}$ & $0.906 \scriptstyle{\pm 0.021}$ &
%         $0.859 \scriptstyle{\pm 0.022}$ & $0.755 \scriptstyle{\pm 0.052}$ & 
%         $0.926 \scriptstyle{\pm 0.021}$ & $0.905 \scriptstyle{\pm 0.013}$ 
%         \\

        
% 	\bottomrule
% \end{tabular}

% }
% \vskip -0.15in
% \end{table}


% \begin{table}[hbtp]
% \centering
%  \caption{Ablation study on length of trajectory for robot push}\label{t:2}
% \resizebox{\textwidth}{!}{  

% \begin{tabular}{l|cc|cc|cc|cc}
% 	\toprule 
%             & \multicolumn{2}{c|}{history=1} & \multicolumn{2}{c|}{history=3} & \multicolumn{2}{c|}{history=5} & \multicolumn{2}{c}{history=10} \\

%         \midrule

%                  & Success Rate & Entropy & Success Rate & Entropy & Success Rate & Entropy & Success Rate & Entropy \\

% 	\midrule

%         GPT  & 
%         $0.0 \scriptstyle{\pm 0.0}$ & $0.0 \scriptstyle{\pm 0.0}$ &
%         $0.806 \scriptstyle{\pm 0.055}$ & $0.073 \scriptstyle{\pm 0.018}$ & 
%         $0.825 \scriptstyle{\pm 0.024}$ & $0.090 \scriptstyle{\pm 0.025}$ & 
%         $0.831 \scriptstyle{\pm 0.024}$ & $0.336 \scriptstyle{\pm 0.071}$ \\
%         % -------------------------------------------------------------- %
%         BeT & 
%         $0.529 \scriptstyle{\pm 0.035}$ & $0.385 \scriptstyle{\pm 0.067}$ &
%         $0.634 \scriptstyle{\pm 0.034}$ & $0.479 \scriptstyle{\pm 0.101}$ & 
%         $0.608 \scriptstyle{\pm 0.045}$ & $0.471 \scriptstyle{\pm 0.138}$ & 
%         $0.684 \scriptstyle{\pm 0.055}$ & $0.482 \scriptstyle{\pm 0.141}$\\
%         % -------------------------------------------------------------- %
%         DDPM-GPT & 
%         $0.732 \scriptstyle{\pm 0.021}$ & $0.541 \scriptstyle{\pm 0.056}$ & 
%         $0.818 \scriptstyle{\pm 0.030}$ & $0.665 \scriptstyle{\pm 0.045}$ & 
%         $0.839 \scriptstyle{\pm 0.016}$ & $0.775 \scriptstyle{\pm 0.061}$ & 
%         $0.858 \scriptstyle{\pm 0.018}$ & $0.756 \scriptstyle{\pm 0.077}$\\
%         % -------------------------------------------------------------- %
%         BESO  & 
%         0 & 0 & 
%         0 & 0 & 
%         0 & 0\\
        
% 	\bottomrule
% \end{tabular}

% }
% \vskip -0.15in
% \end{table}

\begin{table}[hbtp]
\centering
 \caption{Ablation study on the size of dataset for robot push}\label{t:2}
\resizebox{\textwidth}{!}{  

\begin{tabular}{l|cc|cc|cc|cc}
	\toprule 
            & \multicolumn{2}{c|}{25\% dataset} & \multicolumn{2}{c|}{50\% dataset} & \multicolumn{2}{c}{75\% dataset} & \multicolumn{2}{c}{100\% dataset} \\

        \midrule

                 & Success Rate & entropy & Success Rate & entropy & Success Rate & entropy & 
                 Success Rate & entropy\\

	\midrule
        MLP & 
        $0.208 \scriptstyle{\pm 0.125}$ & $0$ & 
        $0.586 \scriptstyle{\pm 0.078}$ & $0$ & 
        $0.691 \scriptstyle{\pm 0.066}$ & $0$ &
        $0.708 \scriptstyle{\pm 0.052}$ & $0$\\
        % -------------------------------------------------------------- %
        CVAE  & 
        $0.035 \scriptstyle{\pm 0.034}$ & $0.002 \scriptstyle{\pm 0.005}$ & 
        $0.121 \scriptstyle{\pm 0.062}$ & $0.020 \scriptstyle{\pm 0.026}$ & 
        $0.363 \scriptstyle{\pm 0.086}$ & $0.034 \scriptstyle{\pm 0.032}$ &
        $0.579 \scriptstyle{\pm 0.138}$ & $0.030 \scriptstyle{\pm 0.053}$\\
        % -------------------------------------------------------------- %
        BeT-MLP & 
        $0.194 \scriptstyle{\pm 0.099}$ & $0.120 \scriptstyle{\pm 0.084}$ & 
        $0.466 \scriptstyle{\pm 0.025}$ & $0.345 \scriptstyle{\pm 0.097}$ & 
        $0.438 \scriptstyle{\pm 0.103}$ & $0.381 \scriptstyle{\pm 0.156}$ &
        $0.507 \scriptstyle{\pm 0.081}$ & $0.485 \scriptstyle{\pm 0.092}$\\
        % -------------------------------------------------------------- %
        IBC & 
        $0.392 \scriptstyle{\pm 0.039}$ & $0.220 \scriptstyle{\pm 0.049}$ & 
        $0.554 \scriptstyle{\pm 0.033}$ & $0.307 \scriptstyle{\pm 0.141}$ & 
        $0.602 \scriptstyle{\pm 0.086}$ & $0.293 \scriptstyle{\pm 0.094}$ &
        $0.638 \scriptstyle{\pm 0.027}$ & $0.300 \scriptstyle{\pm 0.048}$\\
        % -------------------------------------------------------------- %
        DDPM & 
        $0.336 \scriptstyle{\pm 0.131}$ & $0.275 \scriptstyle{\pm 0.162}$ & 
        $0.699 \scriptstyle{\pm 0.009}$ & $0.628 \scriptstyle{\pm 0.041}$ & 
        $0.748 \scriptstyle{\pm 0.029}$ & $0.652 \scriptstyle{\pm 0.029}$ &
        $0.763 \scriptstyle{\pm 0.039}$ & $0.712 \scriptstyle{\pm 0.064}$\\
        % -------------------------------------------------------------- %
        GPT & 
        $0.483 \scriptstyle{\pm 0.086}$ & $0.055 \scriptstyle{\pm 0.019}$ & 
        $0.747 \scriptstyle{\pm 0.060}$ & $0.074 \scriptstyle{\pm 0.040}$ & 
        $0.789 \scriptstyle{\pm 0.039}$ & $0.089 \scriptstyle{\pm 0.036}$ &
        $0.833 \scriptstyle{\pm 0.043}$ & $0$\\
        % -------------------------------------------------------------- %
        BeT & 
        $0.384 \scriptstyle{\pm 0.041}$ & $0.315 \scriptstyle{\pm 0.079}$ & 
        $0.550 \scriptstyle{\pm 0.076}$ & $0.391 \scriptstyle{\pm 0.100}$ & 
        $0.592 \scriptstyle{\pm 0.031}$ & $0.460 \scriptstyle{\pm 0.074}$ &
        $0.645 \scriptstyle{\pm 0.069}$ & $0.536 \scriptstyle{\pm 0.105}$\\
        % -------------------------------------------------------------- %
        DDPM-GPT & 
        $0.690 \scriptstyle{\pm 0.048}$ & $0.573 \scriptstyle{\pm 0.060}$ & 
        $0.785 \scriptstyle{\pm 0.021}$ & $0.699 \scriptstyle{\pm 0.034}$ &
        $0.835 \scriptstyle{\pm 0.024}$ & $0.753 \scriptstyle{\pm 0.037}$ & 
        $0.839 \scriptstyle{\pm 0.020}$ & $0.664 \scriptstyle{\pm 0.075}$\\
        % -------------------------------------------------------------- %
        BESO  & 
        $0.705 \scriptstyle{\pm 0.044}$ & $0.579 \scriptstyle{\pm 0.066}$ & 
        $0.820 \scriptstyle{\pm 0.023}$ & $0.712 \scriptstyle{\pm 0.029}$ & 
        $0.836 \scriptstyle{\pm 0.010}$ & $0.761 \scriptstyle{\pm 0.044}$ &
        $0.861 \scriptstyle{\pm 0.016}$ & $0.711 \scriptstyle{\pm 0.030}$\\
        % -------------------------------------------------------------- %
        ACT & 
        $0.668 \scriptstyle{\pm 0.112}$ & $0.049 \scriptstyle{\pm 0.031}$ & 
        $0.892 \scriptstyle{\pm 0.028}$ & $0.089 \scriptstyle{\pm 0.023}$ & 
        $0.899 \scriptstyle{\pm 0.026}$ & $0.140 \scriptstyle{\pm 0.023}$ &
        $0.891 \scriptstyle{\pm 0.022}$ & $0.025 \scriptstyle{\pm 0.012}$\\
        % -------------------------------------------------------------- %
        DiffusionPolicy & 
        $0.711 \scriptstyle{\pm 0.027}$ & $0.650 \scriptstyle{\pm 0.020}$ & 
        $0.831 \scriptstyle{\pm 0.013}$ & $0.666 \scriptstyle{\pm 0.067}$ & 
        $0.848 \scriptstyle{\pm 0.025}$ & $0.715 \scriptstyle{\pm 0.068}$ &
        $0.849 \scriptstyle{\pm 0.023}$ & $0.749 \scriptstyle{\pm 0.041}$\\
        % -------------------------------------------------------------- %
        
	\bottomrule
\end{tabular}

}
\vskip -0.15in
\end{table}

% \begin{table}[hbtp]
% \centering
%  \caption{Ablation study on the size of dataset for Block Push}\label{t:2}
% \resizebox{\textwidth}{!}{  

% \begin{tabular}{l|cc|cc|cc|cc}
% 	\toprule 
%             & \multicolumn{2}{c|}{25\% dataset} & \multicolumn{2}{c|}{50\% dataset} & \multicolumn{2}{c}{75\% dataset} & \multicolumn{2}{c}{100\% dataset} \\

%         \midrule

%                  & Success Rate & entropy & Success Rate & entropy & Success Rate & entropy \\

% 	\midrule

%         CVAE  & 
%         $0 \scriptstyle{\pm 0}$ & $0 \scriptstyle{\pm 0}$ & 
%         $0 \scriptstyle{\pm 0}$ & $0 \scriptstyle{\pm 0}$ & 
%         0 & 0 \\
%         % -------------------------------------------------------------- %
%         DDPM & 
%         0 & 0 & 
%         0 & 0 & 
%         0 & 0\\
%         % -------------------------------------------------------------- %
%         BeT & 
%         $0 \scriptstyle{\pm 0}$ & $0 \scriptstyle{\pm 0}$ & 
%         $0 \scriptstyle{\pm 0}$ & $0 \scriptstyle{\pm 0}$ & 
%         0 & 0\\
%         % -------------------------------------------------------------- %
%         DDPM-GPT & 
%         $0 \scriptstyle{\pm 0}$ & $0 \scriptstyle{\pm 0}$ & 
%         $0 \scriptstyle{\pm 0}$ & $0 \scriptstyle{\pm 0}$ & 
%         0 & 0\\
%         % -------------------------------------------------------------- %
%         BESO  & 
%         0 & 0 & 
%         0 & 0 & 
%         0 & 0\\
        
% 	\bottomrule
% \end{tabular}

% }
% \vskip -0.15in
% \end{table}

\begin{table}[hbtp]
\centering
 \caption{Ablation study with DDPM-GPT policy selection standards}\label{image_table}
\resizebox{\textwidth}{!}{  

\begin{tabular}{l|cc|cc|cc}
	\toprule 
            & \multicolumn{2}{c|}{Robot Push} & \multicolumn{2}{c|}{Sorting 4 Boxes} & \multicolumn{2}{c}{Image-based Sorting 4 boxes}  \\
            
        \midrule

          & Success Rate & Entropy & Success Rate & Entropy & Success Rate & Entropy \\

	\midrule

        MSE loss  & 
        $0. \scriptstyle{\pm 0.}$ & $0. \scriptstyle{\pm 0.}$ & 
        $0. \scriptstyle{\pm 0.}$ & $0. \scriptstyle{\pm 0.}$ & 
        $0. \scriptstyle{\pm 0.}$ & $0. \scriptstyle{\pm 0.}$ \\
        % -------------------------------------------------------------- %
        
        ELBO & 
        $0.839 \scriptstyle{\pm 0.016}$ & $0.775 \scriptstyle{\pm 0.061}$ &
        $0.340 \scriptstyle{\pm 0.064}$ & $0.392 \scriptstyle{\pm 0.067}$ & 
        $0. \scriptstyle{\pm 0.}$ & $0. \scriptstyle{\pm 0.}$\\
        % -------------------------------------------------------------- %
        
        Last checkpoint & 
        $0. \scriptstyle{\pm 0.}$ & $0. \scriptstyle{\pm 0.}$ &
        $0.491 \scriptstyle{\pm 0.071}$ & $0.430 \scriptstyle{\pm 0.049}$ & 
        $0. \scriptstyle{\pm 0.}$ & $0. \scriptstyle{\pm 0.}$  
        \\
        % -------------------------------------------------------------- %
        
        Simulation performance & 
        $0. \scriptstyle{\pm 0.}$ & $0. \scriptstyle{\pm 0.}$ &
        $0. \scriptstyle{\pm 0.}$ & $0. \scriptstyle{\pm 0.}$ & 
        $0.770 \scriptstyle{\pm 0.022}$ & $0.270 \scriptstyle{\pm 0.033}$ 
        \\

        
	\bottomrule
\end{tabular}

}
\vskip -0.15in
\end{table}

==> sections/methods_copy.tex <==
% \section{Multi-modal robot learning tasks}
\section{Datasets with Diverse Demonstrations
for Imitation Learning}
% \begin{figure*}[t]
%         \centering
%         \subfigure[Obstacle Avoidance]{
%         \begin{minipage}[t!]{0.3\textwidth}
%             \centering 
%             \includegraphics[width=\textwidth]{figures/tasks2/oa.png}
%         \end{minipage}
%         }
%         \hfill
%         \subfigure[Block Push]{
%         \begin{minipage}[t!]{0.3\textwidth}
%             \centering 
%             \includegraphics[width=\textwidth]{figures/tasks2/bp.png}
%         \end{minipage}
%         }
%          \hfill
%          \subfigure[Box Alignment]{
%         \begin{minipage}[t!]{0.3\textwidth}
%             \centering 
%             \includegraphics[width=\textwidth]{figures/tasks2/rp.png}
%         \end{minipage}
%         }
        
%          \hfill
%         \subfigure[Sorting]{
%          \begin{minipage}[t!]{0.32\textwidth}
%             \centering 
%             \includegraphics[width=\textwidth]{figures/tasks2/sorting.png}
%         \end{minipage}
%         }
%         \hfill
%         \subfigure[CubeStacking]{
%         \begin{minipage}[t!]{0.32\textwidth}
%             \centering 
%             \includegraphics[width=\textwidth]{figures/tasks2/cube_stacking.png}
%         \end{minipage}
%         }
%         \hfill
%         \caption[ ]
%         {\small \textbf{Environments.} We created 5 tasks in this paper, including one toy task Obstacle Avoidance and 4 robot manipulation tasks. For each task, we collected a large amount of human demonstrations with diverse behaviors. }
%         \label{fig:environments}
% \end{figure*}

% \begin{table}[hbtp]
% \centering
%  \caption{Dataset description}\label{t:2}
% % \resizebox{\textwidth}{!}{  

% \begin{tabular}{l|cccc}
% 	\toprule 
            
%          Tasks &  Modes & Training &  Evaluation & KL \\

% 	\midrule

%         Obstacle Avoidance  & 
%         24 & 96 & 
%         0 & 0  \\
%         % -------------------------------------------------------------- %
%         Block Push  & 
%         4 & 1800 & 
%         200 & 0  \\
%         % -------------------------------------------------------------- %
%         Box Alignment & 
%         2 & 900 & 
%         100 & 0 \\
%         % -------------------------------------------------------------- %
%         Sorting 2 & 
%         2 & 540 & 
%         60 & 0 \\
%         % -------------------------------------------------------------- %
%         Sorting 4 & 
%         6 & 0 & 
%         0 & 0 \\
%         % -------------------------------------------------------------- %
%         Sorting 6 & 
%         0 & 0 & 
%         0 & 0 \\
%         % -------------------------------------------------------------- %  
%         Cube Stacking & 
%         6 & 0 & 
%         0 & 0 \\
% 	\bottomrule
% \end{tabular}

% % }
% \vskip -0.15in
% \end{table}

% \textcolor{red}{
% \subsection{Quantifying Multimodality}
% \begin{enumerate}
%     \item Mention that multimodality refers to a multimodal action distribution for a given state
%     \item Hard to quantify on a state level
%     \item We therefore design our tasks such that we can compute auxiliary metrics that are highly correlated with multimodality on a state level. 
%     \item Mention that we are using the word \textit{mode} interchangeably for both metrics  
%     \item examples
% \end{enumerate}
% }
% \textbf{All tasks consist of a human-recorded dataset for training and a simulator for evaluation.}

In this section, we present a novel suite of tasks known as D3IL - Datasets with Diverse Demonstrations for Imitation Learning. We first introduce metrics for the quantification of diverse behavior (refer to Section \ref{section:quant}). Subsequently, we delve into the design principles underlying our tasks, which are subsequently introduced at the end of this section.

\subsection{Quantifying Diverse Behavior}
\label{section:quant}
% For simplicity, we restrict the following discussion to Markovian policies $\pi(\act|\state)$, but can straightforwardly be generalized to policies with history $h$, prediction horizon $k$, or both. Define Action and Observation space.
Let $\mathcal{D} = \{(\act_n, \state_n)\}_{n=1}^N$ be a human-recorded demonstration dataset with actions $\act \in \mathcal{A}$ and states $\state \in \mathcal{S}$. Further, let $p(\act|\state)$ be the underlying state-conditional action distribution. The goal of imitation learning is to learn a policy $\pi(\act|\state) \approx p(\act|\state)$. Diversity is characterized by a multimodal action distribution $p(\act|\state)$, meaning that there are multiple distinct actions that are likely for a given state $\state$. We refer to this as multimodality on a \textit{state-level}. However, this multimodality is hard to quantify in most scenarios as we do not have access to $p(\act|\state)$. Instead, we look at the multimodality on a \textit{behavior-level} to define an auxiliary metric that reflects if a model is capable of imitating diverse behaviors. To define behavior-level multi-modality, we introduce a behavior distribution $p(\beta)$ which is a categorical distribution over discrete behavior descriptors $\beta \in \mathcal{B}$, for example, which box has been chosen to be pushed first. %In this work, we define behavior as a sequence of actions that lead to a successful task completion. 
The space $\mathcal{B}$ of behaviour descriptors and its demonstration distribution $p(\beta)$ are thus task-specific and are discussed in Section \ref{section:task_data}.

To evaluate the ability of a trained policy $\pi(\act|\state)$ to capture multi-modality, we utilize simulations in the task environment to compute the agents'  distribution $\pi(\beta)$ over its achieved behaviors. Subsequently, we assess the policy by measuring the similarity between the agents' behavior distribution $\pi(\beta)$ and the demonstrated behavior distribution $p(\beta)$. This evaluation is achieved through the Kullback-Leibler (KL) divergence, i.e.,
\begin{equation*}
    D_{\text{KL}}\big(\pi(\beta)\|p(\beta)\big) = \sum_{\beta \in \mathcal{B}} \pi(\beta) \log \frac{\pi(\beta)}{p(\beta)}.
\end{equation*}
 In practice, we collect data such that the distribution over behaviors is approximately uniform, i.e., $p(\beta) \approx 1/|\mathcal{B}|$. Consequently, we can replace the KL divergence with the behavior entropy, that is,
\begin{equation}
\label{eq:ent}
    \mathcal{H}\big(\pi(\beta)\big) = -  \sum_{\beta \in \mathcal{B}} 
    \pi(\beta) \log_{|\mathcal{B}|} {\pi(\beta)},
\end{equation}
to quantify diverse behaviors. Please note that we employ the logarithm with a base of $|\mathcal{B}|$ to ensure that $\mathcal{H}\big(\pi(\beta)\big) \in [0,1]$. This choice of base facilitates a straightforward interpretation of the metric: An entropy value of $0$ signifies a policy that consistently executes the same behavior, while an entropy value of $1$ represents a diverse policy that executes all behaviors with equal probability, that is, $\pi(\beta) \approx 1/|\mathcal{B}|$  and hence matches the true behavior distribution by the design of the data collection process. Yet, a high behaviour entropy can also be achieved by following different behaviors in different initial states in a deterministic manner, and hence, this behaviour entropy can be a poor metric for behavior diversity. Hence, we evaluate the expected entropy of the behavior conditioned on the initial state $\state_0$. If, for the same initial state, all behaviors can be achieved, the conditional behavior entropy is high, while if for the same initial state always the same behavior is executed, this entropy is 0. We define the conditional behavior entropy as
%
%To ensure that deterministic policies are quantified as having zero diversity, certain tasks necessitate the definition of a context-dependent behavior distribution denoted as $p(\beta|\con)$, where $\con$ is drawn from a context distribution $p(\con)$ within the context space $\con \in \mathcal{C}$. Analogously to the derivation of Eq. \ref{eq:ent}, we introduce the expected contextual entropy metric
\begin{equation}
\label{eq:c_ent}
    \mathbb{E}_{\state_0 \sim p(\state_0)}\left[\mathcal{H}\big(\pi(\beta|\state_0)\big)\right] \approx - \frac{1}{S_0}\sum_{\state_0 \sim p(\state_0)} \sum_{\beta \in \mathcal{B}} 
    \pi(\beta|\state_0) \log_{|\mathcal{B}|} {\pi(\beta|\state_0)},
\end{equation}
where the expectation is approximated using a Monte Carlo estimate. Here, $S_0$ denotes the number of samples from the initial state distribution $p(\state_0)$. 

% In human demonstrations, multi-modality refers to a multi-modal action distribution for a given state, which is $p(a|s)$. Since the state space is infinite, it is hard to quantify the multi-modality on a state level. We therefore consider auxiliary metrics that are highly correlated with multi-modality on the state level. Considering that the different actions on a specific state could lead to different solutions for a task, we try to evaluate the multi-modality on the task level. Given a human dataset, we define $p_m^*$ as the mode distribution, which describes the probability for different solutions. 

% Imitation learning model aims to learn a policy $\pi(a|s)$ which can match the data distribution $p(a|s)$. We expect the model to solve the task with $m$ solutions and ideally, the mode distribution should match the data distribution $p_m^*$.
% During the evaluation, we rollout the policy for multiple times and calculate the mode density $p_m$. Comparing the distance between $p_m^*$ and $p_m$, we can approximate how good the model learns the multi-modality.


% A classic example is reaching task, where the robot can choose multiple ways to reach the goal. 

% \textbf{Non-Markovian Data.} \textcolor{red}{Remove. Change to closed loop feedback/sensory.} In addition to variable trajectory lengths, our dataset includes non-Markovian data. This means that actions at a given time step depend not only on the current state but also on a more extensive history of observations and actions. This design principle introduces complexity and tests our models' ability to capture long-term dependencies and correlations within the data, which is often crucial for understanding diverse human behaviors.

\subsection{Task Design Principles}
\label{section:design}
We build D3IL based on the following key principles:
\textbf{i) Diverse Behavior.} 
Diversity is the central aspect of our task design. We intentionally design our tasks to encompass multiple viable approaches to successful task completion. To quantify the behavior diversity, we explicitly specify these distinct behaviors, each representing a legitimate solution. %This allows us to establish tractable metrics for quantifying a model's capacity to replicate diverse human behavior as discussed in Section \ref{section:quant}. 
\textbf{ii.) Multiple Human Demonstrators.} To reflect the natural variability in human behavior and to obtain a richer dataset, we have collected demonstration data from multiple human demonstrators. This diversity in data sources introduces variations in the quality and style of demonstrations.
\textbf{iii.) Variable Trajectory Lengths.}
Our tasks incorporate variable trajectory lengths, replicating real-world scenarios where demonstrations may differ in duration. This design choice challenges our learning agents to handle non-uniform data sequences effectively. By accommodating varying trajectory lengths, our approach must learn to adapt and generalize to different time horizons, a critical property for real-world applications.
\textbf{iv.) Task Variations and Closed-Loop Feedback.} For most tasks, agents need to rely on sensory feedback  to achieve a good performance which considerably increases the complexity of the learning task in comparison to learning open-loop trajectories.  We achieve this by introducing task variations in every execution. For example, in every execution, the initial position of the objects will be different and the agent needs to adapt its behaviour accordingly. 

%This feedback loop, which encompasses visual, proprioceptive, or other sensory inputs, enables the agents to perceive the consequences of their actions and make necessary adjustments to achieve task objectives. By incorporating sensory feedback as a fundamental element of our task design, we create learning environments that closely emulate real-world situations.

\subsection{Task Description and Data Collection}
\label{section:task_data}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
We simulate all tasks (\textbf{T1}-\textbf{T5}) using the Mujoco physics engine (\cite{todorov2012mujoco}). The simulation environment consists of a 7DoF Franka Emika Panda robot and various objects. For \textbf{T1}-\textbf{T4}, the robot is equipped
with a cylindrical end effector to perform object manipulations. The corresponding demonstrations
are recorded by using an Xbox game-pad which sends commands to an inverse kinematics (IK) controller. In \textbf{T5}, the robot has a parallel gripper and uses an augmented reality setup for
controlling the end effector, allowing for more dexterous manipulations. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{SCfigure}[50][ht]
    \centering
    \includegraphics[width=0.25\linewidth]{figures/tasks2/oa.png} 
             \caption{\textbf{Avoiding (T1).} The Avoiding task requires the robot to reach the green finish line from a fixed initial position without colliding with one of the six obstacles. The task does not require object manipulation and is designed to test a model's ability to capture diversity.
There are $24$ different ways of successfully completing the task and thus $|\mathcal{B}|=24$. The dataset contains 96 demonstrations in total, comprising 24 solutions with 4 trajectories for each solution.}
\vspace{-0.5cm}
\end{SCfigure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% , and hence $p(\beta) = 1/|\mathcal{B}|$. 
% 
% of successful task completions alongside the success rate, i.e., the percentage of successful task completions. 
% The human demonstrations are recorded by using an Xbox controller and the robot is controlled by using an inverse kinematics (IK) controller. The dataset contains 96 demonstrations in total, comprising 24 solutions with 4 trajectories for each solution, and hence $p(\beta) = 1/|\mathcal{B}|$.


% The obstacle avoidance task is a robot learning environment to evaluate the model's multi-modality. This environment has 6 obstacles and the robot's goal is to reach the green line without colliding with any of those objects. The human demonstrations are recorded by using the Xbox controller and the robot is controlled by using an inverse kinematics controller. The dataset contains 96 demonstrations in total, comprising 24 solutions with 4 trajectories for each solution. For each imitation learning method, the inputs $x$ include the robot's desired cartesian position and current cartesian position. The targets $y$ include the robot's desired cartesian velocity.

\begin{SCfigure}[50][ht]
    \centering
    \includegraphics[width=0.25\linewidth]{figures/tasks2/rp.png} 
             \caption{\textbf{Aligning (T2).} The Aligning task requires the robot to push a hollow box to a predefined target position and orientation. The task can be completed by either pushing the box from outside or inside and thus $|\mathcal{B}|=2$. It requires less diversity than T1 but involves complex object manipulation. The dataset contains $1\text{k}$ demonstrations, $500$ for each behavior with uniformly sampled initial states.}
             
\vspace{-0.5cm}
\end{SCfigure}

\begin{SCfigure}[50][ht]
    \centering
    \vspace{-0.5cm}
    \includegraphics[width=0.25\linewidth]{figures/tasks2/bp.png} 
             \caption{\textbf{Pushing (T3).} This task requires the robot to push two blocks to fixed target zones. Having two blocks and two target zones results in $|\mathcal{B}|= 4$ behaviors. The task has more diversity than T2 and involves complex object manipulations. Additionally, the task has high variation in trajectory length caused by multiple human demonstrators with different experience levels. The dataset contains $2\text{k}$ demonstrations, $500$ for each behavior with uniformly sampled initial block positions.}
\end{SCfigure}

%
% The block push task is similar to the block-pusing environment used by Implicit Behavioral Cloning (IBC) \cite{florence2022implicit}. This task contains two stage: pushing one block to a target area; coming back and pushing another block to another target area. From the IBC environment, it has two solutions for this task. The robot can either push the red block to the red target first or push the green block to the green target first. They use a scripted policy to collect demonstrations. In this paper, we add two more modes: the robot can also push the red block to the green area and push the green block to the red area. We collect 500 human demonstrations for each mode, for a total of 2000 demonstrations across four modes. 
% The inputs $x$ contains robot's desired cartesian position, current cartesian position and two blocks' positions and orientation. 




\begin{SCfigure}[50][ht]
    \centering
    \includegraphics[width=0.25\linewidth]{figures/tasks2/sorting.png} 
             \caption{\textbf{Sorting-}$\text{X}$\textbf{ (T4).} This task requires the robot to sort red and blue blocks to their color-matching target box. The `X' refers to the number of blocks. In this work, we test three difficulty levels, i.e., $\text{X} \in \{2,4,6\}$. The number of behaviors $|\mathcal{B}|$ is determined by the sorting order. For $\text{X}=6$, the task has many objects, is highly diverse ($|\mathcal{B}|=20$), requires complex manipulations,  has high variation in trajectory length, and is thus more challenging than T1-T3. The dataset contains $1.6$k demonstrations for $X=6$ and an approximately equal number of trajectories for each sorting order.}
             \vspace{-0.5cm}
\end{SCfigure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{SCfigure}[50][hbt!]
    \centering
    \includegraphics[width=0.25\linewidth]{figures/tasks2/cube_stacking.png} 
            \caption{\textbf{Stacking-}$\text{X}$\textbf{ (T5).} This task requires the robot to stack blocks with different colors in a (yellow) target zone. The number of behaviors $|\mathcal{B}|$ is given by the stacking order. Having three different blocks results in six different combinations for stacking the blocks and hence $|\mathcal{B}|=6$. This task additionally requires dexterous manipulations since the blue box has the be stacked upright and is thus considered to be the most challenging out of all five tasks. Here, `X' does not refer to the difficulty but rather to the evaluation protocol: For Stacking-X with $\text{X}\in \{1,2,3\}$ we compute the performance metrics of the models that are capable of stacking X blocks. The $\approx 1\text{k}$ trajectories were recorded using augmented reality (AR) such that each stacking order is equally often present.}
             % \caption{\textbf{Stacking (T5).} This  task requires the robot to stack blocks with different colors in a (yellow) target zone. The number of behaviors $|\mathcal{B}|$ is given by the stacking order. Having three different blocks results in six different combinations for stacking the blocks and hence $|\mathcal{B}|=6$. This task additionally requires dexterous manipulations since the blue box has the be stacked upright and is thus considered to be the most challenging out of all five tasks. The $\approx 1\text{k}$ trajectories were recorded using augmented reality (AR) such that each stacking order is equally often present.}
             \vspace{-0.5cm}
\end{SCfigure}

\captionsetup[figure]{labelformat=default}%
\setcounter{figure}{0} 
% ($p(\beta) \approx 1/|\mathcal{B}|$). \textcolor{red}{Mention contextual entropy with context c.}


% Explain setup here (AR collected data + high dimensional action space + Dexterous Manipulation + Multimodality)
% %
% In this task, there are three boxes with different colors, two of which are cubes and one is a rectangular box. The goal is to stack the three boxes together. For the red and green cubes, it is straightforward to pick and place them. To stack the blue box, the robot need to firstly pick it and rotate the box to make it stand upright. The different behaviors for three boxes make this task rather complex. The robot can stack the three boxes in different orders which give 6 solutions for the task. We record 1095 human demonstrations using Augmented Reality. 

% \subsection{Dataset Collection}
% For obstacle avoidance, box alignment, block push and sorting tasks, the height and orientation of the end effector of the robot are fixed. These tasks are named as 2d tasks, because the action space only contains $x$ and $y$ axis. In these tasks, the robot is controlled by an inverse kinematics controller. We use a Xbox controller to record the human demonstrations. 

% For the CubeStacking task, the robot need to rotate and stack the cubes. We directly use a joint position controller. In this task, we developed an intuitive AR system to control the robot. The virtual robot in the simulation needs to follow the moves of the real robot. Then we get all the trajectories from the simulation logs.

% \subsection{Diverse behaviors}
% In order to better characterize the multi-modality of each task, we further analyze the different solutions. Generally, different trajectories can be represented as different modes. For obstacle avoidance, it is straightforward to illustrate the different solutions \ref{fig:environments}. For box alignment, pushing from inside or outside of the box can lead to different actions. Imitation learning aims to learn a policy $\pi(a|s)$ which can match the data distribution $p(a|s)$. Fig. \ref{fig:environments} shows the action distribution for two modes of box alignment task. Note that the two different modes mainly exist before the robot pushing the box. The pushing behavior is actually similar for two modes.

% For environments with multiple boxes, different manipulation orders can end up with different trajectories. We define 4 modes for block push task. As to the sorting task, we increase the number of mode by adding more boxes. For cubestacking task, we add a rectangular box to make it more complex.

% In this task, the robot's action is the velocity of $x$ and $y$ axis. 
